On discretization of continuous-time LPV control solutions

In recent years, the Linear Parameter-Varying (LPV) framework has become increasingly useful for analysis and control of time-varying systems. Generally, LPV control synthesis is performed in the continuous-time (CT) domain due to significantly more intuitive performance shaping methods in CT. However, the main complication of CT synthesis approaches is the successive implementation of the resulting CT control solutions on physical hardware. In the literature, several discretization methods have been developed for LPV systems. However, most of these approaches necessitate heavy nonlinear operations introduced by the discretization of these time-varying matrices or can introduce significant approximation error, thereby severely limiting implementation capabilities of CT LPV control solutions. Alternatively, the $w'$ discretization approach has been introduced in the LTI case to allow for preservation of the CT control. Based on these observations, this paper aims at extending the $w'$ discretization approach to LPV systems, such that implementation of CT LPV control solutions on physical hardware is simplified.

==> MyBib.tex <==
\Sort{
  Mode{on}
  Collation{mixed}
  SortTypeOrder{pattern,key,name}
  NameOrder{ascending}
  Key{{author,editor},\year{year,note}}
  KeyOrder{descending,nulls first}
  Pattern{author+editor: "doron"}
  PatternOrder{first}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{whitbeck1978digital,
  title={Digital control law synthesis in the w'domain},
  author={Whitbeck, RF and Hofmannf, LG},
  journal={Journal of Guidance and Control},
  volume={1},
  number={5},
  pages={319--326},
  year={1978}
}

@book{zhou1998essentials,
  title={Essentials of robust control},
  author={Zhou, Kemin and Doyle, John Comstock},
  volume={104},
  year={1998},
  publisher={Prentice hall Upper Saddle River, NJ}
}

 @book{sysidToolbox,
  title={System Identification Toolbox: User's guide},
  author={Ljung, L.},
  year={2019},
  publisher={MathWorks}
 }
 
 
@manual{agilentDatasheet,
    organization  = "Agilent Laser and Optics",
    title         = "User’s Manual, Volume I",
    number        = "05517-90086",
    year          =  2007
}

@manual{agilentDatasheet,
    organization  = "Agilent Laser and Optics",
    title         = "User’s Manual, Volume I",
    number        = "05517-90086",
    year          =  2007
}

@MANUAL{ansysSoftware,
title = { ANSYS Academic Research Mechanical, Release 17.1},
organization = {ANSYS Inc.},
}

@manual{agilentDatasheetFull,
    organization  = "Keysight Technologies",
    title         = "Optics and Laser Heads for Laser-Interferometer Positioning Systems",
    number        = "5964-6190E",
    year          =  2017
}


 @misc{ refPhotoGovernor,
   author = "{Wikimedia Commons}",
   title = "File:Centrifugal governor.svg --- Wikimedia Commons{,} the free media repository",
   year = "2017",
   url = "https://commons.wikimedia.org/w/index.php?title=File:Centrifugal_governor.svg&oldid=234951643",
 }

@misc{refAppleChip,
author  = "{Apple press release}",
title = {{Apple introduces iPhone XR}},
  howpublished = {\url{https://www.apple.com/newsroom/2018/09/apple-introduces-iphone-xr/}},
   year={2018}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@book{Pintelonbook,
  title={System identification: a frequency domain approach},
  author={Pintelon, Rik and Schoukens, Johan},
  year={2012},
  publisher={John Wiley \& Sons}
}

@article{LeeU,
  title={U-statistics: Theory and Practice},
  author={Lee, Justin},
  year={1990},
  publisher={CRC Press}
}

@book{Rozanov,
  title={Probability theory: a concise course},
  author={Rozanov, IU},
  year={1977},
  publisher={Courier Dover Publications}
}

@book{Friedland,
  title={Control system design: an introduction to state-space methods},
  author={Friedland, Bernard},
  year={2012},
  publisher={Courier Dover Publications}
}

@book{SchererRobustBook,
  title={Theory of robust control},
  author={Scherer, C.},
  publisher={Delft University of Technology},
  year={2001}  
}

@book{ProakisBook,
  title={Digital signal processing: principles algorithms and applications},
  author={Proakis, J. G.},
  year={2001},
  publisher={Pearson Education India}
}

@book{CarlinBook,
  title={Bayes and empirical Bayes methods for data analysis},
  author={Carlin, B. P. and Louis, T. A.},
  year={2010},
  publisher={Chapman and Hall/CRC}
}

@book{Beck,
  title={Parameter estimation in engineering and science},
  author={Beck, James Vere and Arnold, Kenneth J},
  year={1977},
  publisher={John Wiley \& Sons Inc}
}

@book{RughBook,
  title={Linear system theory},
  author={Rugh, W. J.},
  volume={2},
  year={1996},
  publisher={prentice hall Upper Saddle River, NJ}
}

@book{GriffithsBook,
  title={Introduction to electrodynamics},
  author={Griffiths, D. J.},
  year={1999},
  publisher={Prentice Hall}
}

@book{NealBook,
  title={Bayesian learning for neural networks},
  author={Neal, R.M.},
  volume={118},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@book{Rasmussen,
 author = {Rasmussen, C. E. and Williams, C. K. I.},
 title = {Gaussian Processes for Machine Learning (Adaptive Computation and Machine Learning)},
 year = {2005},
 publisher = {MIT Press}
} 

   @BOOK{VerhaegenBook,
   author = "Verhaegen, M. and Verdult, V.",
   title= "Filtering and System Identification. A Least Squares Approach",
   publisher = "Cambridge University Press",
   year = 2011 }

   @BOOK{Katayama,
   author = "Tohru Katayama",
   title= "Subspace Methods for System Identification",
   publisher = "Springer",
   year = 2005 }
   
      @BOOK{VanOverscheeMoorBook,
   author = "van Overschee, P. and de Moor, B.",
   title= "Subspace Identification for Linear Systems",
   publisher = "Kluwer Academic Publishers",
   year = 1996 }
 
 @book{LjungMatlab,
    author = {Ljung, L.},
    citeulike-article-id = {3853201},
    keywords = {phd},
    posted-at = {2009-01-06 11:06:00},
    priority = {4},
    publisher = {The MathWorks, Inc.},
    title = {System Identification Toolbox for Use with {MATLAB}},
    year = {2007}
}

@article{Scherer-lmi-book,
  title={Linear matrix inequalities in control},
  author={Scherer, C. and Weiland, S.},
  journal={Lecture Notes, Dutch Institute for Systems and Control, Delft, The Netherlands},
  volume={3},
  number={2},
  year={2000}
}
  
  
  @book{DekkingBook,
  title={A Modern Introduction to Probability and Statistics: Understanding why and how},
  author={Dekking, F. M. and Kraaikamp, C. and Lopuha{\"a}, H. P. and Meester, L. E.},
  year={2005},
  publisher={Springer Science \& Business Media}
}


  @book{LjungBook,
  title={System identification - Theory for the User},
  author={Ljung, L.},
  year={1999},
  publisher={Prentice-Hall}
}

  @book{Golub,
  title={Matrix Computations, Fourth Edition},
  author={G.H. Golub and C.F. van Loan},
  year={2013},
  publisher={The Johns Hopkins University Press}
}
@book{Boyd,
  title={Convex optimization},
  author={Boyd, Stephen P and Vandenberghe, Lieven},
  year={2004},
  publisher={Cambridge university press}
}

@book{AstromBook,
 author = {{\AA}str\"{o}m, K. J. and Wittenmark, B.},
 title = {Computer-controlled Systems (3rd Ed.)},
 year = {1997},
 isbn = {0-13-314899-8},
 publisher = {Prentice-Hall, Inc.},
 address = {Upper Saddle River, NJ, USA},
}


@book{AndersonBook,
  title={Optimal filtering},
  author={Anderson, B. D. O. and Moore, J. B.},
  year={2012},
  publisher={Courier Dover Publications}
}

@book{VanDenHof,
  title={Course SC4110: System Identification},
  author={van den Hof, P. M. J.},
  year={2006},
  publisher={Delft University of Technology}
}

@book{Papoulis,
  title={Probability, random variables, and stochastic processes},
  author={Papoulis, Athanasios and Pillai, S Unnikrishna},
  year={2002},
  publisher={Tata McGraw-Hill Education}
}

@book{Tothbook,
  title={Modeling and identification of linear parameter-varying systems},
  author={T{\'o}th, R.},
  volume={403},
  year={2010},
  publisher={Springer}
}

@book{Furlani,
  title={Permanent magnet and electromechanical devices: materials, analysis, and applications},
  author={Furlani, E. P.},
  year={2001},
  publisher={Academic Press}
}

@book{Skogestad,
  title={Multivariable feedback control: analysis and design},
  author={Skogestad, Sigurd and Postlethwaite, Ian},
  volume={2},
  year={2007},
  publisher={Wiley New York}
}


@book{Craig,
  title={Introduction to robotics: mechanics and control},
  author={Craig, J. J.},
  volume={3},
  year={2005},
  publisher={Pearson Prentice Hall Upper Saddle River}
}

@book{Murray-book,
  title={A mathematical introduction to robotic manipulation},
  author={Murray, R. M. and Li, Z. and Sastry, S. S.},
  year={1994},
  publisher={CRC press}
}

@book{YoungBook,
  title={An introduction to Hilbert space},
  author={Young, N.},
  year={1988},
  publisher={Cambridge university press}
}


@book{Spong,
  title={Robot modeling and control},
  author={Spong, M. W. and Hutchinson, S. and Vidyasagar, M.},
  volume={3},
  year={2006},
  publisher={Wiley New York}
}

@book{Harrison,
  title={Advanced engineering dynamics},
  author={Harrison, H.R.N.T. and Nettleton, T.},
  year={1997},
  publisher={Butterworth-Heinemann}
}

@book{Gawronski,
  title={Advanced structural dynamics and active control of structures},
  author={Gawronski, W.},
  year={2004},
  publisher={Springer Science \& Business Media}
}


@book{Rao-book,
  title={Mechanical vibrations},
  author={Rao, S. S. and Yap, F. F.},
  volume={4},
  year={1995},
  publisher={Addison-Wesley New York}
}

@book{Franklin,
  title={Feedback control of dynamic systems},
  author={Franklin, Gene F and Powell, J David and Emami-Naeini, Abbas and Powell, J David},
  volume={2},
  year={1994},
  publisher={Addison-Wesley Reading}
}

@book{Hutton-book,
  title={Fundamentals of finite element analysis},
  author={Hutton, David},
  year={2004},
  publisher={McGraw-Hill,}
}

@book{Zienkiewicz-book,
  title={The finite element method: its basis and fundamentals},
  author={Zienkiewicz, O. C. and Taylor, R. L. and Zhu, J. Z.},
  year={2005},
  publisher={Elsevier}
}

@book{Preumont,
  title={Vibration control of active structures},
  author={Preumont, Andr{\'e}},
  volume={2},
  year={1997},
  publisher={Springer}
}


@book{CraigBook,
  title={Fundamentals of structural dynamics},
  author={Craig, R. R. and Kurdila, A. J.},
  year={2006},
  publisher={John Wiley \& Sons}
}

@book{ZhouBook,
 author = {Zhou, K. and Doyle, J. C. and Glover, K.},
 title = {Robust and Optimal Control},
 year = {1996},
 isbn = {0-13-456567-3},
 publisher = {Prentice-Hall, Inc.},
 address = {Upper Saddle River, NJ, USA}
} 

@book{OppenheimBook,
 author = {Oppenheim, A. V. and Schafer, R. W. and Buck, J. R.},
 title = {Discrete-time Signal Processing (2Nd Ed.)},
 year = {1999},
 isbn = {0-13-754920-2},
 publisher = {Prentice-Hall, Inc.},
 address = {Upper Saddle River, NJ, USA}
} 

@book{MackBook,
  title={Field guide to optical lithography},
  author={Mack, C. A.},
  volume={6},
  year={2006},
  publisher={SPIE Press Bellingham, WA}
}

@book{LojekBook,
  title={History of semiconductor engineering},
  author={Lojek, B.},
  year={2007},
  publisher={Springer}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%		Patents			%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@misc{PatentTrumper1,
  title={Magnetic arrays},
  author={Trumper, D.L. and Kim, W. and Williams, M.E.},
  year={1997},
  month=may # "~20",
  note={US Patent 5,631,618}
}

@misc{PatentFrissen,
  title={Contactless lifting of an object by an inverted planar motor},
  author= {Frissen, P.C.M. and Compter, J.C.},
 year={2009},
 note={WO Patent 2,009,083,889}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%		Techincal report			%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@techreport{TRVerkerk,
  title={NAPAS dSpace Sensor Acquisition (technical report)},
     author = {Verkerk, Koen},
     group = {Control Systems},
     year = {2016},
     institution = {Eindhoven University of Technology},
}

@techreport{TRVerkerk1,
  title={NAPAS dSpace Control (technical report)},
     author = {Verkerk, Koen},
     group = {Control Systems},
     year = {2016},
     institution = {Eindhoven University of Technology},
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%		THESES				%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% THESES and PHD PROJECTS
 	@mastersthesis{Koster,
 	author = "S.E. Koster",
 	title = "Development of a novel subspace identification method: a backward-time approach",
 	school = "Delft University of Technology",
 	year = 2013 }
 	
 		@mastersthesis{Felici,
 	author = "Federico Felici",
 	title = "Subspace Identification of {LPV} systems: A novel approach",
 	school = "Delft University of Technology",
 	year = 2005 }
 
 
 @book{Verdult-phd,
  title={Non linear system identification: a state-space approach},
  author={Verdult, Vincent},
  year={2002},
  publisher={Twente University Press}
}	

@phdthesis{JW-phd,
  title={Control of wind turbines with 'Smart' rotors: proof of concept \& {LPV} subspace identification},
  author={van Wingerden, Jan-Willem},
  school={Delft University of Technology},
  year={2008}
}

@phdthesis{Rovers-phd,
  title={Multiphysical modeling of high-precision electromechanical devices},
  author={Rovers, J. M. M.},
    school={Eindhoven University of Technology},
  year={2013}
}

@phdthesis{Jansen-phd,
  title={Magnetically levitated planar actuator with moving magnets: Electromechanical analysis and design {I}},
  author={Jansen, J. W.},
  school={Eindhoven University of Technology},
  year={2007}
}

@phdthesis{Lierop-phd,
  title={Magnetically levitated planar actuator with moving magnets: Electromechanical analysis and design II},
  author={van Lierop, C. M. M.},
  school={Eindhoven University of Technology},
  year={2007}
}

@phdthesis{Dorosti-phd,
  title={Reduced-order Model Updating for Prediction of Performance Variables in Mechanical Structures},
  author={Dorosti, M.},
  school={Eindhoven University of Technology},
  year={2017}
}

@phdthesis{Cox-phd,
  title={Towards efficient identification of linear parameter-varying state-space models},
  author={Cox, Pepijn B},
  year={2018},
  publisher = "Technische Universiteit Eindhoven",
 school= {Eindhoven University of Technology},
}

@phdthesis{Darwish-phd,
title = "Bayesian identification of linear dynamic systems: synthesis of kernels in the LTI case and beyond",
author = "M.A.H. Darwish",
year = "2017",
month = "10",
day = "10",
language = "English",
isbn = "978-90-386-4352-6",
 school= {Eindhoven University of Technology}
}


@phdthesis{Custers-phd,
title = "Overactuated magnetically levitated systems: flexible modes and eddy current phenomena in high-precision bearingless planar motors",
author = "Custers, C.",
year = "2019",
day = "24",
language = "English",
isbn = "978-90-386-4800-2",
publisher = "Technische Universiteit Eindhoven",
 school= {Eindhoven University of Technology}
}

@phdthesis{Verkerk-phd,
title = "Improved accuracy of flexible systems by state estimation : applied to high-precision motion systems",
author = "K.W. Verkerk",
year = "2018",
month = "1",
day = "17",
language = "English",
isbn = "978-90-386-4411-0",
publisher = "Technische Universiteit Eindhoven",
 school= {Eindhoven University of Technology}
}


@phdthesis{Proimadis-phd,
title = "Nanometer-accurate motion control of moving-magnet planar motors",
author = "Ioannis Proimadis",
year = "2020",
day = "30",
language = "English",
isbn = "978-90-386-5026-5",
publisher = "Technische Universiteit Eindhoven",
school = "Department of Electrical Engineering"
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%		Papers			%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
@inproceedings{3Gebraad,
  title={{LPV} subspace identification using a novel nuclear norm regularization method},
  author={Gebraad, PMO and van Wingerden, JW and van der Veen, GJ and Verhaegen, M},
  booktitle={American Control Conference (ACC), 2011},
  pages={165--170},
  year={2011},
  organization={IEEE}
}

@article{4Sadigh,
  title={Robust Subspace System Identification via Weighted Nuclear Norm Optimization},
  author={Sadigh, Dorsa and Ohlsson, Henrik and Sastry, S Shankar and Seshia, Sanjit A},
  journal={arXiv preprint arXiv:1312.2132},
  year={2013}
}

@article{5Veen,
  title={Global Identification of Wind Turbines Using a Hammerstein Identification Method},
  author={van der Veen, G. and van Wingerden, J. W. and Verhaegen, M.},
  journal={IEEE Transactions on Control Systems Technology},
  number={99},
  pages={1--1},
  year={2012},
  publisher={IEEE}
}

 @article{7Ljung,
  title={Subspace identification from closed loop data},
  author={Ljung, L. and McKelvey, T.},
  journal={Signal Processing},
  volume={52},
  number={2},
  pages={209--215},
  year={1996},
  publisher={Elsevier}
}


@article{9Veen,
  title={Closed-loop subspace identification methods: an overview},
  author={van der Veen, G. and van Wingerden, J. W. and Bergamasco, M. and Lovera, M. and Verhaegen, M.},
  journal={IET Control Theory \& Applications},
  volume={7},
  number={10},
  pages={1339--1358},
  year={2013},
  publisher={IET Digital Library}
}

	
@inproceedings{10Qin,
  title={Parallel {QR} implementation of subspace identification with parsimonious models},
  author={Qin, S.J. and Ljung, L.},
  booktitle={Proceedings of the 13th IFAC SYSID Symposium},
  pages={1631--1636},
  year={2003}
}
 	
@inproceedings{11Qin,
  title={Closed-loop subspace identification with innovation estimation},
  author={Qin, S.J. and Ljung, L.},
  booktitle={Proceedings of the 13th IFAC SYSID Symposium},
  pages={887--892},
  year={2003}
}

@article{12Chiuso,
title = "Consistency analysis of some closed-loop subspace identification methods ",
journal = "Automatica ",
volume = "41",
number = "3",
pages = "377 - 391",
year = "2005",
note = "Data-Based Modelling and System Identification ",
issn = "0005-1098",
doi = "http://dx.doi.org/10.1016/j.automatica.2004.10.015",
author = "Alessandro Chiuso and Giorgio Picci",
keywords = "Subspace identification",
keywords = "Exogenous inputs",
keywords = "Stochastic realization",
keywords = "Statistical analysis",
keywords = "Stochastic state-space identification "
}

 	@article{13Forssell,
title = "Closed-loop identification revisited ",
journal = "Automatica ",
volume = "35",
number = "7",
pages = "1215 - 1241",
year = "1999",
note = "",
issn = "0005-1098",
doi = "http://dx.doi.org/10.1016/S0005-1098(99)00022-9",
author = "Urban Forssell and Lennart Ljung",
keywords = "System identification",
keywords = "Closed-loop identification",
keywords = "Prediction error methods",
keywords = "Modelling",
keywords = "Statistical analysis "
}


@inproceedings{14Lin,
title = "Comparison of subspace identification methods for systems operating on closed-loop ",
  author={Lin, Weilu and Qin, S Joe and Ljung, Lennart},
  booktitle={Proceedings of the 16th IFAC World Congress},
  pages={494--499},
  year={2005}
}


@article{16Qin,
title = "An overview of subspace identification ",
journal = "Computers \& Chemical Engineering ",
volume = "30",
number = "10–12",
pages = "1502 - 1513",
year = "2006",
note = "Papers form Chemical Process Control \{VII\} \{CPC\} \{VII\} Seventh international conference in the Series ",
issn = "0098-1354",
doi = "http://dx.doi.org/10.1016/j.compchemeng.2006.05.045",
author = "S. Joe Qin",
keywords = "Subspace identification",
keywords = "Closed-loop identification",
keywords = "Overview",
keywords = "State space models",
keywords = "Causal model",
keywords = "Practice "
}

@article{17Schon,
  title={System identification of nonlinear state-space models},
  author={Sch{\"o}n, Thomas B and Wills, Adrian and Ninness, Brett},
  journal={Automatica},
  volume={47},
  number={1},
  pages={39--49},
  year={2011},
  publisher={Elsevier}
}

@article{21Ljung,
  title={Approaches to identification of nonlinear systems},
  author={Ljung, Lennart},
  year={2010}
}

@article{22Ljung,
  title={Four encounters with system identification},
  author={Ljung, L. and Hjalmarsson, H. and Ohlsson, H.},
  journal={European Journal of Control},
  volume={17},
  number={5},
  pages={449--471},
  year={2011},
  publisher={Elsevier}
}

@inproceedings{27Kantas,
  title={An overview of sequential Monte Carlo methods for parameter estimation in general state-space models},
  author={Kantas, Nicholas and Doucet, Arnaud and Singh, Sumeetpal Sindhu and Maciejowski, Jan Marian},
  booktitle={15th IFAC Symposium on System Identification (SYSID), Saint-Malo, France.(invited paper)},
  volume={102},
  pages={117},
  year={2009}
}

 	@article{28VanOverschee,
title = "N4SID: Subspace algorithms for the identification of combined deterministic-stochastic systems ",
journal = "Automatica ",
volume = "30",
number = "1",
pages = "75 - 93",
year = "1994",
note = "Special issue on statistical signal processing and control ",
issn = "0005-1098",
doi = "http://dx.doi.org/10.1016/0005-1098(94)90230-5",
url = "http://www.sciencedirect.com/science/article/pii/0005109894902305",
author = "van Overschee, P. and de Moor, B.",
keywords = "System identification",
keywords = "Kalman filters",
keywords = "difference equations",
keywords = "\{QR\} and singular value decomposition",
keywords = "multivariable systems",
keywords = "state space methods "
}

@article{29VanOverschee,
title = "A unifying theorem for three subspace system identification algorithms ",
journal = "Automatica ",
volume = "31",
number = "12",
pages = "1853 - 1864",
year = "1995",
note = "Trends in System Identification ",
issn = "0005-1098",
doi = "http://dx.doi.org/10.1016/0005-1098(95)00072-0",
url = "http://www.sciencedirect.com/science/article/pii/0005109895000720",
author = "Peter van Overschee and Bart de Moor",
keywords = "System identification",
keywords = "subspace methods",
keywords = "multivariable systems",
keywords = "state-space methods",
keywords = "linear algebra",
keywords = "Kalman filters",
keywords = "difference equations",
keywords = "stochastic systems "
}


@INPROCEEDINGS{30Larimore, 
author={Larimore, W.E.}, 
booktitle={Decision and Control, 1990., Proceedings of the 29th IEEE Conference on}, 
title={Canonical variate analysis in identification, filtering, and adaptive control}, 
year={1990}, 
month={Dec}, 
pages={596-604 vol.2}, 
keywords={Markov processes;adaptive control;filtering and prediction theory;identification;statistical analysis;abruptly changing systems;adaptive control;canonical variate analysis;filtering;identification;nonlinear systems;optimal Akaike information criterion procedure;past/future Markov property;reduced-order prediction problem;singular value decomposition;state order selection;state-space model estimation;time-varying systems;Adaptive control;Adaptive filters;Filtering;Predictive control;Predictive models;Singular value decomposition;State estimation;Stochastic processes;System identification;Time varying systems}, 
doi={10.1109/CDC.1990.203665},}

@article{31Verhaegen,
title = "Identification of the deterministic part of {MIMO} state space models given in innovations form from input-output data ",
journal = "Automatica ",
volume = "30",
number = "1",
pages = "61 - 74",
year = "1994",
note = "Special issue on statistical signal processing and control ",
issn = "0005-1098",
doi = "http://dx.doi.org/10.1016/0005-1098(94)90229-1",
author = "Michel Verhaegen",
keywords = "State space",
keywords = "system identification",
keywords = "linear systems",
keywords = "linear algebra "
}

@article{32McKelvey,
  title={Frequency Domain System Identification with IV Based Subspace Algorithm},
  author={McKelvey, Tomas},
  year={1995},
  publisher={Citeseer}
}

@inproceedings{38Veen,
  title={Closed-loop MOESP subspace model identification with parametrisable disturbances},
  author={van der Veen, Gijs and van Wingerden, J and Verhaegen, Michel},
  booktitle={Decision and Control (CDC), 2010 49th IEEE Conference on},
  pages={2813--2818},
  year={2010},
  organization={IEEE}
}

@inproceedings{39Ruscio,
  title={Subspace system identification of the Kalman filter: open and closed loop systems},
  author={Di Ruscio, David},
  booktitle={Proc. Intl. Multi-Conf. on Engineering and Technological Innovation},
  year={2008}
}

@article{40Ruscio,
  title={{Closed and Open Loop Subspace System Identification of the Kalman Filter}},
  author={Di Ruscio, David},
  journal={Modeling, Identification and Control},
  volume={30},
  number={2},
  pages={71--86},
  year={2009},
  doi={10.4173/mic.2009.2.3},
  publisher={Norwegian Society of Automatic Control}
}

@article{41Chiuso,
  title={The role of vector autoregressive modeling in predictor-based subspace identification},
  author={Chiuso, Alessandro},
  journal={Automatica},
  volume={43},
  number={6},
  pages={1034--1048},
  year={2007},
  publisher={Elsevier}
}

@article{42Verdult,
  title={Subspace identification of multivariable linear parameter-varying systems},
  author={Verdult, V. and Verhaegen, M.},
  journal={Automatica},
  volume={38},
  number={5},
  pages={805--814},
  year={2002},
  publisher={Elsevier}
}

@article{43Felici,
  title={Subspace identification of MIMO LPV systems using a periodic scheduling sequence},
  author={Felici, F. and van Wingerden, J. W. and Verhaegen, M.},
  journal={Automatica},
  volume={43},
  number={10},
  pages={1684--1697},
  year={2007},
  publisher={Elsevier}
}

@article{44Wingerden,
  title={Subspace identification of bilinear and {LPV} systems for open-and closed-loop data},
  author={van Wingerden, J. W. and Verhaegen, M.},
  journal={Automatica},
  volume={45},
  number={2},
  pages={372--381},
  year={2009},
  publisher={Elsevier}
}

@INPROCEEDINGS{45Lee, 
author={Lee, L.H. and Poolla, K.}, 
booktitle={Decision and Control, 1996., Proceedings of the 35th IEEE Conference on}, 
title={Identification of linear parameter-varying systems via LFTs}, 
year={1996}, 
month={Dec}, 
volume={2}, 
pages={1545-1550 vol.2}, 
keywords={Hessian matrices;minimisation;nonlinear programming;parameter estimation;Hessian-based nonlinear optimization algorithms;LFT;LPV;cost function minimization;gradient-based nonlinear optimization algorithms;identifiability;identification;initialization;linear parameter-varying systems;linear-fractional parameter dependence;prediction error method;1f noise;Aircraft;Cost function;Linear systems;Mechanical engineering;Missiles;Noise measurement;Noise reduction;Parameter estimation;Time varying systems}, 
doi={10.1109/CDC.1996.572742}, 
ISSN={0191-2216},}

@article{46Verdult,
title = "Kernel methods for subspace identification of multivariable \{LPV\} and bilinear systems ",
journal = "Automatica ",
volume = "41",
number = "9",
pages = "1557 - 1565",
year = "2005",
note = "",
issn = "0005-1098",
doi = "http://dx.doi.org/10.1016/j.automatica.2005.03.027",
author = "Verdult, V. and Verhaegen, M.",
keywords = "System identification",
keywords = "Subspace methods",
keywords = "State-space methods",
keywords = "Linear parameter-varying systems",
keywords = "Bilinear systems "
}

@inproceedings{47Verdult,
  title={Identification of fully parameterized linear and nonlinear state-space systems by projected gradient search},
  author={Verdult, Vincent and Bergboer, Niek and Verhaegen, Michel},
  booktitle={Proceedings of the 13th IFAC Symposium on System Identification, The Netherlands},
  year={2003}
}

@inproceedings{48Verdult,
  title={Least squares support vector machines for kernel CCA in nonlinear state-space identification},
  author={Verdult, Vincent and Suykens, Johan AK and Boets, Jeroen and Goethals, Ivan and de Moor, Bart},
  booktitle={Proceedings of the 16th international symposium on Mathematical Theory of Networks and Systems (MTNS2004), Leuven, Belgium},
  year={2004}
}

@inproceedings{49Wingerden,
  title={Subspace identification of {MIMO} LPV systems: The PBSID approach},
  author={van Wingerden, J. W. and Verhaegen, M.},
  booktitle={Decision and Control, 2008. CDC 2008. 47th IEEE Conference on},
  pages={4516--4521},
  year={2008},
  organization={IEEE}
}

@inproceedings{50Wingerden,
  title={Subspace identification of multivariable LPV systems: a novel approach},
  author={van Wingerden, J. W. and Verhaegen, M.},
  booktitle={Computer-Aided Control Systems, 2008. CACSD 2008. IEEE International Conference on},
  pages={840--845},
  year={2008},
  organization={IEEE}
}

@inproceedings{52Wingerden,
  title={Subspace identification of bilinear systems using a dedicated input sequence},
  author={van Wingerden, J. W. and Verhaegen, M.},
  booktitle={Decision and Control, 2007 46th IEEE Conference on},
  pages={4962--4967},
  year={2007},
  organization={IEEE}
}

@inproceedings{53Rajaoarisoa,
  title={Subspace technique for identification of hybrid complex systems.},
  author={Rajaoarisoa, Lala H and M'sirdi, Nacer K and Boukas, E-K and Naamane, Aziz},
  booktitle={Control and Automation, 2008 16th Mediterranean Conference on},
  pages={89--94},
  year={2008},
  organization={IEEE}
}

@inproceedings{54Wingerden,
  title={The asymptotic variance of the PBSIDopt algorithm},
  author={van Wingerden, Jan-Willem},
  booktitle={System Identification},
  volume={16},
  number={1},
  pages={1167--1172},
  year={2012}
}

@inproceedings{55Lygeros,
  title={Lecture notes on hybrid systems},
  author={Lygeros, J.},
  booktitle={Notes for an ENSIETA workshop},
  year={2004}
}

@article{56Paoletti,
  title={Identification of Hybrid Systems A Tutorial},
  author={Paoletti, Simone and Juloski, Aleksandar Lj and Ferrari-Trecate, Giancarlo and Vidal, Ren{\'e}},
  journal={European journal of control},
  volume={13},
  number={2},
  pages={242--260},
  year={2007},
  publisher={Elsevier}
}

@inproceedings{57Verdult,
  title={Subspace identification of piecewise linear systems},
  author={Verdult, V. and Verhaegen, M.},
  booktitle={Decision and Control, 2004. CDC. 43rd IEEE Conference on},
  volume={4},
  pages={3838--3843},
  year={2004},
  organization={IEEE}
}

@inproceedings{58Borges,
  title={Iterative subspace identificatino of piecewise linear systems},
  author={Borges, J. and Verdult, V. and Verhaegen, M.},
  booktitle={Proceedings of the 14th IFAC SYSID Symposium},
  pages={368--373},
  year={2006}
}

@incollection{59Juloski,
  title={Comparison of four procedures for the identification of hybrid systems},
  author={Juloski, Aleksandar Lj and Heemels, WPMH and Ferrari-Trecate, Giancarlo and Vidal, Ren{\'e} and Paoletti, Simone and Niessen, JHG},
  booktitle={Hybrid systems: computation and control},
  pages={354--369},
  year={2005},
  publisher={Springer}
}

@inproceedings{60Borges,
  title={A switching detection method based on projected subspace classification},
  author={Borges, J. and Verdult, V. and Verhaegen, M. and Botto, M. A.},
  booktitle={Decision and Control, 2005 and 2005 European Control Conference. CDC-ECC'05. 44th IEEE Conference on},
  pages={344--349},
  year={2005},
  organization={IEEE}
}

@article{61Verhaegen,
  title={Subspace model identification part 3. Analysis of the ordinary output-error state-space model identification algorithm},
  author={Verhaegen, M.},
  journal={International Journal of control},
  volume={58},
  number={3},
  pages={555--586},
  year={1993},
  publisher={Taylor \& Francis}
}

@INPROCEEDINGS{62Lopes, 
author={Vilela Lopes, R. and Araujo Borges, G. and Yoshiyuki Ishihara, J.}, 
booktitle={American Control Conference (ACC), 2013}, 
title={New algorithm for identification of discrete-time switched linear systems}, 
year={2013}, 
month={June}, 
pages={6219-6224}, 
keywords={MIMO systems;discrete time systems;identification;linear systems;matrix algebra;pattern classification;pattern clustering;state-space methods;time-varying systems;data classification;data clustering;discrete-time switched linear MIMO state space system identification;numerical simulation;submodel matrix representation;subspace identification techniques;Clustering algorithms;Data models;Heuristic algorithms;Markov processes;Robustness;Switches;Vectors}, 
ISSN={0743-1619},}

@INPROCEEDINGS{63Huang, 
author={Kun Huang and Wagner, A. and Yi Ma}, 
booktitle={Decision and Control, 2004. CDC. 43rd IEEE Conference on}, 
title={Identification of hybrid linear time-invariant systems via subspace embedding and segmentation (SES)}, 
year={2004}, 
month={Dec}, 
volume={3}, 
pages={3227-3234 Vol.3}, 
keywords={linear systems;observability;principal component analysis;state-space methods;time-varying systems;generalized principal component analysis;hybrid linear time-invariant systems;state-space models;subspace embedding;subspace segmentation;Biomedical informatics;Bismuth;Filtering;Linear systems;Noise robustness;Principal component analysis;System identification;Upper bound}, 
doi={10.1109/CDC.2004.1428971}, 
ISSN={0191-2216},}

@article{64Vidal,
  title={Generalized principal component analysis (GPCA)},
  author={Vidal, Rene and Ma, Yi and Sastry, Shankar},
  journal={Pattern Analysis and Machine Intelligence, IEEE Transactions on},
  volume={27},
  number={12},
  pages={1945--1959},
  year={2005},
  publisher={IEEE}
}


@INPROCEEDINGS{65Pekpe, 
author={Pekpe, K.M. and Mourot, G. and Gasso, K. and Ragot, J.}, 
booktitle={Decision and Control, 2004. CDC. 43rd IEEE Conference on}, 
title={Identification of switching systems using change detection technique in the subspace framework}, 
year={2004}, 
month={Dec}, 
volume={4}, 
pages={3720-3725 Vol.4}, 
keywords={Markov processes;parameter estimation;time-varying systems;Markov parameters;abrupt model changes;change detection technique;identification technique;local models;subspace framework;subspace method;switching systems;Control system analysis;Convergence;Delay estimation;Merging;Nonlinear control systems;Nonlinear systems;Parameter estimation;State-space methods;Switching systems;Testing}, 
doi={10.1109/CDC.2004.1429317}, 
ISSN={0191-2216},}


@inproceedings{66Bako,
  title={Identification of MIMO switched state-space models},
  author={Bako, Laurent and Le, van Luong and Lauer, Fabien and Bloch, Gerard},
  booktitle={American Control Conference (ACC), 2013},
  pages={71--76},
  year={2013},
  organization={IEEE}
}


@incollection{67Wingerden,
  title={Subspace Identification of Hammerstein--Wiener Systems Operating in Closed-loop},
  author={van Wingerden, J.W. and Verhaegen, M.},
  booktitle={Block-oriented Nonlinear System Identification},
  pages={229--239},
  year={2010},
  publisher={Springer}
}

@inproceedings{68Wingerden,
  title={Closed-loop subspace identification of Hammerstein-Wiener models},
  author={van Wingerden, J. W. and Verhaegen, M.},
  booktitle={Decision and Control, 2009 held jointly with the 2009 28th Chinese Control Conference. CDC/CCC 2009. Proceedings of the 48th IEEE Conference on},
  pages={3637--3642},
  year={2009},
  organization={IEEE}
}

@inproceedings{69Wingerden,
  title={Closed loop identification of MIMO Hammerstein models using LS-SVM},
  author={van Wingerden, J. W. and Verhaegen, M.},
  booktitle={System Identification},
  volume={15},
  number={1},
  pages={1650--1655},
  year={2009}
}

@article{70Goethals,
  title={Identification of MIMO Hammerstein models using least squares support vector machines},
  author={Goethals, Ivan and Pelckmans, Kristiaan and Suykens, Johan AK and de Moor, Bart},
  journal={Automatica},
  volume={41},
  number={7},
  pages={1263--1272},
  year={2005},
  publisher={Elsevier}
}

@article{71Goethals,
  title={Subspace identification of Hammerstein systems using least squares support vector machines},
  author={Goethals, Ivan and Pelckmans, Kristiaan and Suykens, Johan AK and de Moor, Bart},
  journal={Automatic Control, IEEE Transactions on},
  volume={50},
  number={10},
  pages={1509--1519},
  year={2005},
  publisher={IEEE}
}

@inproceedings{72Verdult,
  title={A kernel method for subspace identification of multivariable bilinear systems},
  author={Verdult, V. and Verhaegen, M.},
  booktitle={Decision and Control, 2003. Proceedings. 42nd IEEE Conference on},
  volume={4},
  pages={3972--3977},
  year={2003},
  organization={IEEE}
}

@article{73Suykens,
  title={Least squares support vector machine classifiers},
  author={Suykens, Johan AK and Vandewalle, Joos},
  journal={Neural processing letters},
  volume={9},
  number={3},
  pages={293--300},
  year={1999},
  publisher={Springer}
}

@inproceedings{74Goethals,
  title={Subspace intersection identification of Hammerstein-Wiener systems},
  author={Goethals, Ivan and Pelckmans, Kristiaan and Hoegaerts, Luc and Suykens, JAK and de Moor, BLR},
  booktitle={IEEE CONFERENCE ON DECISION AND CONTROL},
  volume={44},
  number={7},
  pages={7108},
  year={2005},
  organization={IEEE; 1998}
}

@article{75Visser,
title = "A new approach to linear regression with multivariate splines ",
journal = "Automatica ",
volume = "45",
number = "12",
pages = "2903 - 2909",
year = "2009",
note = "",
issn = "0005-1098",
doi = "http://dx.doi.org/10.1016/j.automatica.2009.09.017",
author = "C.C. de Visser and Q.P. Chu and J.A. Mulder",
keywords = "Splines",
keywords = "Parameter estimation",
keywords = "Scattered data",
keywords = "Function approximation",
keywords = "Estimators "
}

@article{76Moonen,
  title={On-and off-line identification of linear state-space models},
  author={Moonen, M. and de Moor, B. and Vandenberghe, L. and Vandewalle, J.},
  journal={International Journal of Control},
  volume={49},
  number={1},
  pages={219--232},
  year={1989},
  publisher={Taylor \& Francis}
}


@inproceedings{78Ljung,
  title={What Can Regularization Offer for Estimation of Dynamical Systems?},
  author={Ljung, L. and Chen, T.},
  booktitle={Adaptation and Learning in Control and Signal Processing},
  volume={11},
  number={1},
  pages={1--8},
  year={2013}
}

@article{79Chen,
  title= {{On the estimation of transfer functions, regularizations and Gaussian processes - Revisited}},
  author={Chen, T. and Ohlsson, H. and Ljung, L.},
  journal={Automatica},
  volume={48},
  number={8},
  pages={1525--1535},
  year={2012},
  publisher={Elsevier}
}

@article{80Schon,
  title={An explanation of the expectation maximization algorithm},
  author={Sch{\"o}n, Thomas},
  year={2009}
}

@article{82Ljung,
  title={Perspectives on system identification},
  author={Ljung, L.},
  journal={Annual Reviews in Control},
  volume={34},
  number={1},
  pages={1--12},
  year={2010},
  publisher={Elsevier}
}

@article{83Astrom,
  title={Maximum likelihood and prediction error methods},
  author={{\AA}str{\"o}m, Karl Johan},
  journal={Automatica},
  volume={16},
  number={5},
  pages={551--574},
  year={1980},
  publisher={Elsevier}
}

@article{84Gibson,
  title={Robust maximum-likelihood estimation of multivariable dynamic systems},
  author={Gibson, Stuart and Ninness, Brett},
  journal={Automatica},
  volume={41},
  number={10},
  pages={1667--1682},
  year={2005},
  publisher={Elsevier}
}

@article{85Gibson,
  title={Maximum-likelihood parameter estimation of bilinear systems},
  author={Gibson, Stuart and Wills, Adrian and Ninness, Brett},
  journal={Automatic Control, IEEE Transactions on},
  volume={50},
  number={10},
  pages={1581--1596},
  year={2005},
  publisher={IEEE}
}

@inproceedings{86Deisenroth,
 author = {Deisenroth, Marc Peter and Huber, Marco F. and Hanebeck, Uwe D.},
 title = {Analytic Moment-based Gaussian Process Filtering},
 booktitle = {Proceedings of the 26th Annual International Conference on Machine Learning},
 series = {ICML '09},
 year = {2009},
 isbn = {978-1-60558-516-1},
 location = {Montreal, Quebec, Canada},
 pages = {225--232},
 numpages = {8},
 doi = {10.1145/1553374.1553403},
 acmid = {1553403},
 publisher = {ACM},
 address = {New York, NY, USA}
} 

@inproceedings{87Turner,
  title={State-space inference and learning with Gaussian processes},
  author={Turner, Ryan D and Deisenroth, Marc P and Rasmussen, Carl E},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={868--875},
  year={2010}
}

@article{88Pillonetto,
title = "Kernel methods in system identification, machine learning and function estimation: A survey ",
journal = "Automatica ",
volume = "50",
number = "3",
pages = "657 - 682",
year = "2014",
note = "",
issn = "0005-1098",
doi = "http://dx.doi.org/10.1016/j.automatica.2014.01.001",
author = "Pillonetto, G. and Dinuzzo, F. and Chen, T. and de Nicolao, G. and Ljung, L.",
keywords = "Linear system identification",
keywords = "Prediction error methods",
keywords = "Model complexity selection",
keywords = "Bias-variance trade-off",
keywords = "Kernel-based regularization",
keywords = "Inverse problems",
keywords = "Reproducing kernel Hilbert spaces",
keywords = "Gaussian processes "
}


    @article{89Ljung,
     jstor_articletype = {research-article},
     title = {Asymptotic Properties of the Least-Squares Method for Estimating Transfer Functions and Disturbance Spectra},
     author = {Ljung, L. and Wahlberg, B.},
     journal = {Advances in Applied Probability},
     jstor_issuetitle = {},
     volume = {24},
     number = {2},
     jstor_formatteddate = {Jun., 1992},
     pages = {pp. 412-440},
    ISSN = {00018678},
     abstract = {The problem of estimating the transfer function of a linear system, together with the spectral density of an additive disturbance, is considered. The set of models used consists of linear rational transfer functions and the spectral densities are estimated from a finite-order autoregressive disturbance description. The true system and disturbance spectrum are, however, not necessarily of finite order. We investigate the properties of the estimates obtained as the number of observations tends to ∞ at the same time as the model order employed tends to ∞ . It is shown that the estimates are strongly consistent and asymptotically normal, and an expression for the asymptotic variances is also given. The variance of the transfer function estimate at a certain frequency is related to the signal/noise ratio at that frequency and the model orders used, as well as the number of observations. The variance of the noise spectral estimate relates in a similar way to the squared value of the true spectrum.},
     language = {English},
     year = {1992},
     publisher = {Applied Probability Trust},
     copyright = {Copyright © 1992 Applied Probability Trust},
    }
    
@article{90Rivals,
  title={Black-box modeling with state-space neural networks},
  author={Rivals, Isabelle and Personnaz, L{\'e}on},
  journal={Neural Adaptive Control Technology},
  volume={15},
  pages={237},
  year={1996},
  publisher={World Scientific}
}    

@article{91Akaike,
  title={Stochastic theory of minimal realization},
  author={Akaike, Hirotugu},
  journal={Automatic Control, IEEE Transactions on},
  volume={19},
  number={6},
  pages={667--674},
  year={1974},
  publisher={IEEE}
}

@inproceedings{92Pillonetto,
  title={Predictor estimation via Gaussian regression},
  author={Pillonetto, G. and Chiuso, A. and de Nicolao, G.},
  booktitle={Decision and Control, 2008. CDC 2008. 47th IEEE Conference on},
  pages={744--749},
  year={2008},
  organization={IEEE},
  month = {}
}

@article{93Pillonetto,
  title={A new kernel-based approach for linear system identification},
  author={Pillonetto, G. and de Nicolao, G.},
  journal={Automatica},
  volume={46},
  number={1},
  pages={81--93},
  year={2010},
  publisher={Elsevier}
}

@INPROCEEDINGS{94Chiuso,
author={Chiuso, A. and Pillonetto, G. and de Nicolao, G.}, 
booktitle={Decision and Control, 2008. CDC 2008. 47th IEEE Conference on}, 
title={Subspace identification using predictor estimation via Gaussian regression}, 
year={2008}, 
month={Dec}, 
pages={3299-3304}, 
}


@article{96Pillonetto,
  title={Prediction error identification of linear systems: a nonparametric Gaussian regression approach},
  author={Pillonetto, G. and Chiuso, A. and de Nicolao, G.},
  journal={Automatica},
  volume={47},
  number={2},
  pages={291--305},
  year={2011},
  publisher={Elsevier}
}

@article{97Markovsky,
  title={Overview of total least-squares methods},
  author={Markovsky, Ivan and van Huffel, Sabine},
  journal={Signal processing},
  volume={87},
  number={10},
  pages={2283--2302},
  year={2007},
  publisher={Elsevier}
}

@article{98Ibragimov,
  title={Some limit theorems for stationary processes},
  author={Ibragimov, Ildar A},
  journal={Theory of Probability \& Its Applications},
  volume={7},
  number={4},
  pages={349--382},
  year={1962},
  publisher={SIAM}
}

@article{99Withers,
  title={Central limit theorems for dependent variables. I},
  author={Withers, Christopher Stroude},
  journal={Zeitschrift f{\"u}r Wahrscheinlichkeitstheorie und verwandte Gebiete},
  volume={57},
  number={4},
  pages={509--534},
  year={1981},
  publisher={Springer}
}

@article{100Paige,
  title={Covariance matrix representation in linear filtering},
  author={Paige, Christopher C},
  journal={Special Issue of Contemporary Mathematics on Linear Algebra and its Role in Systems Theory, AMS},
  year={1985}
}

@inproceedings{101Aravkin,
  title={On the estimation of hyperparameters for empirical bayes estimators: Maximum marginal likelihood vs minimum MSE},
  author={Aravkin, Aleksandr and Burke, James V and Chiuso, Alessandro and Pillonetto, Gianluigi},
  booktitle={16th IFAC Symposium on System Identification},
  volume={16},
  number={1},
  pages={125--130},
  year={2012}
}

@inproceedings{102Carli,
  title={{On the estimation of hyperparameters for Bayesian system identification with exponentially decaying kernels.}},
  author={Carli, R. and Chen, T. and Chiuso, A. and Ljung, L. and Pillonetto, G.},
  booktitle={51st IEEE Conference on Decision and Control},
  pages={5260--5265},
  year={2012}
}

@article{103Houtzager,
  title={Predictor-based subspace identification toolbox version 0.4, 2010},
  author={Houtzager, I and van Wingerden, JW and Verhaegen, M},
  journal={URL http://www. dcsc. tudelft. nl/\~{} datadriven/pbsid}
}

@inproceedings{104Toth,
  title={Discrete time {LPV} {I/O} and state space representations, differences of behavior and pitfalls of interpolation},
  author={T{\'o}th, R. and Felici, F. and Heuberger, P. S. C. and van den Hof, P. M. J.},
  booktitle={Proc. of the European control conf},
  pages={5418--5425},
  year={2007}
}

@article{105Chen,
  title={Implementation of algorithms for tuning parameters in regularized least squares problems in system identification},
  author={Chen, T. and Ljung, L.},
  journal={Automatica},
  volume={49},
  number={7},
  pages={2213--2220},
  year={2013},
  publisher={Elsevier}
}

@inproceedings{106Carli,
  title={Efficient algorithms for large scale linear system identification using stable spline estimators},
  author={Carli, Francesca Paola and Chiuso, Alessandro and Pillonetto, Gianluigi},
  booktitle={System Identification},
  volume={16},
  number={1},
  pages={119--124},
  year={2012}
}

@inproceedings{107Chen,
  title={Rank-1 kernels for regularized system identification},
  author={Chen, Tianshi and Chiuso, Alessandro and Pillonetto, Gianluigi and Ljung, Lennart},
  booktitle={Decision and Control (CDC), 2013 IEEE 52nd Annual Conference on},
  pages={5162--5167},
  year={2013},
  organization={IEEE}
}

@inproceedings{108Pillonetto,
  title={Kernel selection in linear system identification Part I: A Gaussian process perspective},
  author={Pillonetto, G. and de Nicolao, G.},
  booktitle={Decision and Control and European Control Conference (CDC-ECC), 2011 50th IEEE Conference on},
  pages={4318--4325},
  year={2011},
  organization={IEEE}
}

@inproceedings{109Chen,
  title={Kernel selection in linear system identification part II: A classical perspective},
  author={Chen, T. and Ohlsson, H. and Goodwin, G.C. and Ljung, L.},
  booktitle={Decision and Control and European Control Conference (CDC-ECC), 2011 50th IEEE Conference on},
  pages={4326--4331},
  year={2011},
  organization={IEEE}
}

@article{113Pillonetto,
author={G. {Pillonetto} and A. {Aravkin}},
booktitle={2014 IEEE International Workshop on Machine Learning for Signal Processing (MLSP)},
title={A new kernel-based approach for identification of time-varying linear systems},
year={2014},
volume={},
number={},
pages={1-6},
doi={10.1109/MLSP.2014.6958894},
ISSN={1551-2541},
month={Sep.}
}


@article{110Bauer,
  title={Order estimation for subspace methods},
  author={Bauer, Dietmar},
  journal={Automatica},
  volume={37},
  number={10},
  pages={1561--1573},
  year={2001},
  publisher={Elsevier}
}

@ARTICLE{114Chen, 
author={Tianshi Chen and Andersen, M.S. and Ljung, L. and Chiuso, A. and Pillonetto, G.}, 
journal={Automatic Control, IEEE Transactions on}, 
title={System Identification Via Sparse Multiple Kernel-Based Regularization Using Sequential Convex Optimization Techniques}, 
year={2014}, 
month={Nov}, 
volume={59}, 
number={11}, 
pages={2933-2945}, }

@article{115Carli,
  title={Maximum Entropy Kernels for System Identification},
  author={Carli, Francesca Paola and Chen, Tianshi and Ljung, Lennart},
  journal={arXiv preprint arXiv:1411.5620},
  year={2014}
}

@inproceedings{116Golabi,
  title={{A Bayesian Approach for Estimation of Linear-Regression LPV Models}},
  author={Golabi, A. and Meskin, N. and T{\'o}th, R. and Mohammadpour, J.},
  booktitle={Decision and Control (CDC), 2014 53th IEEE Conference on},
  pages={2555-2560},
  year={2014},
  organization={IEEE}
}

@article{118Bachnas,
title = "A review on data-driven linear parameter-varying modeling approaches: A high-purity distillation column case study ",
journal = "Journal of Process Control ",
volume = "24",
number = "4",
pages = "272 - 285",
year = "2014",
note = "",
issn = "0959-1524",
author = "A.A. Bachnas and R. T\'{o}th and J.H.A. Ludlage and A. Mesbah"
}

@article{121Toth,
  title={On the state-space realization of {LPV} input-output models: Practical approaches},
  author={T{\'o}th, R. and Abbas, H.S. and Werner, H.},
  journal={Control Systems Technology, IEEE Transactions on},
  volume={20},
  number={1},
  pages={139--153},
  year={2012},
  publisher={IEEE}
}

@article{122Toth,
  title={The behavioral approach to linear parameter-varying systems},
  author={T{\'o}th, R. and Willems, J. C. and Heuberger, P. S. C. and van den Hof, P. M. J.},
  journal={Automatic Control, IEEE Transactions on},
  volume={56},
  number={11},
  pages={2499--2514},
  year={2011},
  publisher={IEEE}
}\\

@article{123Goodwin,
  title={Quantifying the error in estimated transfer functions with application to model order selection},
  author={Goodwin, G.C. and Gevers, M. and Ninness, B.},
  journal={Automatic Control, IEEE Transactions on},
  volume={37},
  number={7},
  pages={913--928},
  year={1992},
  publisher={IEEE}
}

@inproceedings{124Lovera,
  title={Identification for gain-scheduling: a balanced subspace approach},
  author={Lovera, M. and Merc{\`e}re, G.},
  booktitle={American Control Conference 2007, ACC'07},
  pages={CDROM},
  year={2007}
}

@inproceedings{125Chen,
  title={Constructive state space model induced kernels for regularized system identification⋆},
  author={Chen, Tianshi and Ljung, Lennart},
  booktitle={Proceedings of the 19th IFAC World Congress},
  year={2014}
}

@article{127Dinuzzo,
  title={Kernels for linear time invariant system identification},
  author={Dinuzzo, F.},
  journal={arXiv preprint arXiv:1203.4930},
  year={2012}
}

@article{128Aronszajn,
  title={Theory of reproducing kernels},
  author={Aronszajn, N.},
  journal={Transactions of the American mathematical society},
  pages={337--404},
  year={1950},
  publisher={JSTOR}
}

@inproceedings{129Scholkopf,
  title={A generalized representer theorem},
  author={Sch{\"o}lkopf, B. and Herbrich, R. and Smola, A. J.},
  booktitle={Computational learning theory},
  pages={416--426},
  year={2001},
  organization={Springer}
}


@incollection{132Lovera,
  title={{LPV} modelling and identification: An overview},
  author={Lovera, M. and Bergamasco, M. and Casella, F.},
  booktitle={Robust Control and Linear Parameter Varying Approaches},
  pages={3--24},
  year={2013},
  publisher={Springer}
}

@book{133Verdult,
  title={Non linear system identification: a state-space approach},
  author={Verdult, Vincent},
  year={2002},
  publisher={Twente University Press}
}

@book{134Wingerden,
  title={Control of wind turbines with'Smart'rotors: proof of concept \& {LPV} subspace identification},
  author={van Wingerden, J. W.},
  year={2008},
  publisher={TU Delft, Delft University of Technology}
}

@inproceedings{136Toth,
  title={Model structure learning: A support vector machine approach for {LPV} linear-regression models},
  author={T{\'o}th, R. and Laurain, V. and Zheng, W. X. and Poolla, K.},
  booktitle={Decision and Control and European Control Conference (CDC-ECC), 2011 50th IEEE Conference on},
  pages={3192--3197},
  year={2011},
  organization={IEEE}
}

@article{137Rasmussen,
  title={Occam's razor},
  author={Rasmussen, C. E. and Ghahramani, Z.},
  journal={Advances in neural information processing systems},
  pages={294--300},
  year={2001},
  publisher={MIT; 1998}
}

@book{138Mohammadpour,
  title={Control of linear parameter varying systems with applications},
  author={Mohammadpour, J. and Scherer, C.},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@article{139Leith,
  title={Survey of gain-scheduling analysis and design},
  author={Leith, D. J. and Leithead, W. E.},
  journal={International journal of control},
  volume={73},
  number={11},
  pages={1001--1025},
  year={2000},
  publisher={Taylor \& Francis}
}

@article{140Rugh,
title = "Research on gain scheduling ",
journal = "Automatica ",
volume = "36",
number = "10",
pages = "1401 - 1425",
year = "2000",
author = "Rugh, W. J. and Shamma, J. S."
}

@misc{141Orr,
  title={Introduction to radial basis function networks},
  author={Orr, M. J. L.},
  year={1996},
  publisher={Technical Report, Center for Cognitive Science, University of Edinburgh}
}

@article{142Golub,
author = {Golub, Gene H. and Heath, Michael and Wahba, Grace},
title = {Generalized Cross-Validation as a Method for Choosing a Good Ridge Parameter},
journal = {Technometrics},
volume = {21},
number = {2},
pages = {215-223},
year = {1979},
doi = {10.1080/00401706.1979.10489751}
}

@book{143Wahba,
  title={Spline models for observational data},
  author={Wahba, Grace},
  volume={59},
  year={1990},
  publisher={Siam}
}

@article{144Rasmussen,
  title={{Gaussian processes for machine learning (GPML) toolbox}},
  author={Rasmussen, C. E. and Nickisch, H.},
  journal={The Journal of Machine Learning Research},
  volume={11},
  pages={3011--3015},
  year={2010},
  publisher={JMLR. org}
}

@misc{145Houtzager,
  title={Predictor-based Subspace Identification Toolbox Version 0. 4},
  author={Houtzager, I. and Gebraad, P. and van Wingerden, J. W. and Verhaegen, M.},
  year={2010}
}

@article{146Stoica,
  title={On biased estimators and the unbiased Cram{\'e}r-Rao lower bound},
  author={Stoica, Petre and Moses, Randolph L},
  journal={Signal Processing},
  volume={21},
  number={4},
  pages={349--350},
  year={1990},
  publisher={Elsevier}
}

@inproceedings{147Pillonetto,
  title={Pitfalls of the Parametric Approaches Exploiting Cross-Validation for Model Order Selection},
  author={Pillonetto, Gianluigi and de Nicolao, Giuseppe},
  booktitle={System Identification},
  volume={16},
  number={1},
  pages={215--220},
  year={2012}
}

@inproceedings{148Chiuso,
  title={Regularization strategies for nonparametric system identification},
  author={Chiuso, Alessandro and Chen, Tianshi and Ljung, Lennart and Pillonetto, Gianluigi},
  booktitle={Decision and Control (CDC), 2013 IEEE 52nd Annual Conference on},
  pages={6013--6018},
  year={2013},
  organization={IEEE}
}

@inproceedings{149Aravkin,
  title={Convex vs nonconvex approaches for sparse estimation: Lasso, Multiple Kernel Learning and Hyperparameter Lasso},
  author={Aravkin, Aleksander and Burke, James V and Chiuso, Alessandro and Pillonetto, Gianluigi},
  booktitle={Decision and Control and European Control Conference (CDC-ECC), 2011 50th IEEE Conference on},
  pages={156--161},
  year={2011},
  organization={IEEE}
}

@article{150Houtzager,
  title={Recursive predictor-based subspace identification with application to the real-time closed-loop tracking of flutter},
  author={Houtzager, I. and van Wingerden, J. W. and Verhaegen, M.},
  journal={Control Systems Technology, IEEE Transactions on},
  volume={20},
  number={4},
  pages={934--949},
  year={2012},
  publisher={IEEE}
}

@article{151Lovera,
  title={Recursive subspace identification of linear and non-linear Wiener state-space models},
  author={Lovera, M. and Gustafsson, T. and Verhaegen, M.},
  journal={Automatica},
  volume={36},
  number={11},
  pages={1639--1650},
  year={2000},
  publisher={Elsevier}
}

@INPROCEEDINGS{152Huber, 
author={Huber, M.F.}, 
booktitle={Acoustics, Speech and Signal Processing (ICASSP), 2013 IEEE International Conference on}, 
title={{Recursive Gaussian process regression}}, 
year={2013}, 
month={May}, 
pages={3362-3366}, 
ISSN={1520-6149},}

@article{153Merriman,
  title={On the history of the method of least squares},
  author={Merriman, Mansfield},
  journal={The Analyst},
  pages={33--36},
  year={1877},
  publisher={JSTOR}
}

@article{154Freeth,
  title={Decoding the ancient Greek astronomical calculator known as the Antikythera Mechanism},
  author={Freeth, T. and Bitsakis, Y. and Moussas, X. and Seiradakis, J.H. and Tselikas, A. and Mangou, .H and Zafeiropoulou, M. and Hadland, R. and Bate, D. and Ramsey, A.},
  journal={Nature},
  volume={444},
  number={7119},
  pages={587--591},
  year={2006},
  publisher={Nature Publishing Group}
}

@book{155Scholkopf,
  title={Learning with kernels: Support vector machines, regularization, optimization, and beyond},
  author={Sch{\"o}lkopf, B. and Smola, A. J.},
  year={2002},
  publisher={MIT Press}
}

@article{160Jansen,
  title={Magnetically levitated planar actuator with moving magnets},
  author={Jansen, J. W. and van Lierop, C. M. M. and Lomonova, E. A. and Vandenput, A. J. A.},
  journal={IEEE Transactions on Industry Applications},
  volume={44},
  number={4},
  pages={1108--1115},
  year={2008},
  publisher={IEEE}
}

@inproceedings{161Darwish,
  title={Bayesian Identification of {LPV} Box-Jenkins Models},
  author={Darwish, M. and Cox, P. and Pillonetto, G. and T\'{o}th, R.},
  booktitle={Proceedings of the 54th IEEE Conference on Decision and Control (CDC), Osaka, Japan},
  year={2015},
  organization={IEEE}
}

@inproceedings{162Proimadis,
  title={A kernel based approach for {LPV} subspace identification},
  author={Proimadis, Ioannis and Bijl, Hildo and van Wingerden, Jan Willem},
  booktitle={Proceedings of the 1st IFAC Workshop on Linear Parameter Varying Systems, Grenoble, France},
  year={2015},
}

@article{163Golabi, 
author={A. {Golabi} and N. {Meskin} and R. {T{\'o}th} and J. {Mohammadpour}}, 
booktitle={53rd IEEE Conference on Decision and Control}, 
title={{A Bayesian approach for estimation of linear-regression LPV models}}, 
year={2014}, 
volume={}, 
number={}, 
pages={2555-2560}, 
doi={10.1109/CDC.2014.7039779}, 
ISSN={0191-2216}, 
month={Dec}
}

@article{166Akoun,
  title={{3D} analytical calculation of the forces exerted between two cuboidal magnets},
  author={Akoun, G. and Yonnet, J. P.},
  journal={Magnetics, IEEE Transactions on},
  volume={20},
  number={5},
  pages={1962--1964},
  year={1984},
  publisher={IEEE}
}

@article{167Jansen,
  title={Analytical calculation of interaction force between orthogonally magnetized permanent magnets},
  author={Jansen, J. L. G. and Paulides, J. J. H. and Lomonova, E. A. and B{\"o}l{\"o}ni, F. and Tounzi, A. and Piriou, F.},
  journal={Sensor letters},
  volume={7},
  number={3},
  pages={442--445},
  year={2009},
  publisher={American Scientific Publishers}
}

@article{168Rovers,
  title={Calculation of the static forces among the permanent magnets in a {Halbach} array},
  author={Rovers, J. M. M. and Jansen, J. W. and Lomonova, E. A. and Ronde, M. J. C.},
  journal={IEEE Transactions on Magnetics},
  volume={45},
  number={10},
  pages={4372--4375},
  year={2009},
  publisher={IEEE}
}

@article{169Rovers,
  title={Analytical calculation of the force between a rectangular coil and a cuboidal permanent magnet},
  author={Rovers, J. M. M. and Jansen, J. W. and Lomonova, E. A.},
  journal={Magnetics, IEEE Transactions on},
  volume={46},
  number={6},
  pages={1656--1659},
  year={2010},
  publisher={IEEE}
}

@article{171Jansen,
  title={Modeling of magnetically levitated planar actuators with moving magnets},
  author={Jansen, J. W. and van Lierop, C. M. M. and Lomonova, E. A. and Vandenput, A. J. A.},
  journal={Magnetics, IEEE Transactions on},
  volume={43},
  number={1},
  pages={15--25},
  year={2007},
  publisher={IEEE}
}

@article{172Compter,
  title={Electro-dynamic planar motor},
  author={Compter, J. C.},
  journal={Precision Engineering},
  volume={28},
  number={2},
  pages={171--180},
  year={2004},
  publisher={Elsevier}
}

@article{173Rovers,
  title={Analysis method of the dynamic force and torque distribution in the magnet array of a commutated magnetically levitated planar actuator},
  author={Rovers, J. M. M. and Jansen, J. W. and Compter, J. C. and Lomonova, E. A.},
  journal={IEEE Transactions on Industrial Electronics},
  volume={59},
  number={5},
  pages={2157--2166},
  year={2012},
  publisher={IEEE}
}

@article{174Jansen,
  title={Overview of analytical models for the design of linear and planar motors},
  author={Jansen, J. W. and Smeets, J. P. C. and Overboom, T. T. and Rovers, J. M. M. and Lomonova, E. A.},
  journal={IEEE Transactions on Magnetics},
  volume={50},
  number={11},
  pages={1--7},
  year={2014},
  publisher={IEEE}
}


@article{175Wassink,
  title={{LPV} control for a wafer stage: beyond the theoretical solution},
  author={Wassink, M. G. and van de Wal, M. and Scherer, C. and Bosgra, O.},
  journal={Control Engineering Practice},
  volume={13},
  number={2},
  pages={231--245},
  year={2005},
  publisher={Elsevier}
}

@article{176Butler,
  title={Position control in lithographic equipment},
  author={Butler, H.},
  journal={IEEE Control Systems Magazine},
  volume={31},
  number={5},
  pages={28--47},
  year={2011}
}

@article{177Rovers,
title = "The deformation of the moving magnet plate of a commutated magnetically levitated planar actuator ",
journal = "Mechatronics ",
volume = "23",
number = "2",
pages = "233 - 239",
year = "2013",
note = "Special Issue on Linear Drives ",
issn = "0957-4158",
doi = "http://dx.doi.org/10.1016/j.mechatronics.2012.01.011",
author = "Rovers, J.M.M. and Achterberg, J. and Ronde, M.J.C. and  Jansen, J.W. and Compter, J.C. and Lomonova, E.A. and van Lierop, C.M.M. and  van den Molengraft, M.J.G.",
}

@inproceedings{179Verkerk,
  title={Modal observer design for a flexible motion system with state dependent sensor positions},
  author={Verkerk, K. W. and Achterberg, J. and van Lierop, C. M. M. and Weiland, S.},
  booktitle={Decision and Control (CDC), 2012 IEEE 51st Annual Conference on},
  pages={4498--4504},
  year={2012},
  organization={IEEE}
}

@inproceedings{180Verkerk,
  title={State estimator synthesis for position dependent flexible systems with position independent error convergence},
  author={Verkerk, K.W. and Kasemsinsup, Y. and Butler, H. and Weiland, S.},
  booktitle={Control and Automation (MED), 2015 23th Mediterranean Conference on},
  pages={1065--1070},
  year={2015},
  organization={IEEE}
}

@MastersThesis{181Kasemsinsup,
  title={Position-dependent state observer design for a planar motor wafer stage},
  author={Kasemsinsup, Y.},
  year={2013},
  school={Department of Electrical Engineering, Control Systems Group, Eindhoven University of Tehcnology}
    }
    
@article{183Pillonetto,
  title={A new kernel-based approach for nonlinear system identification},
  author={Pillonetto, G. and Quang, M. H. and Chiuso, A.},
  journal={Automatic Control, IEEE Transactions on},
  volume={56},
  number={12},
  pages={2825--2840},
  year={2011},
  publisher={IEEE}
}


@article{184Jeltsema,
  title={Multidomain modeling of nonlinear networks and systems},
  author={Jeltsema, D. and Scherpen, J.M.A.},
  journal={IEEE Control Systems},
  volume={29},
  number={4},
  pages={28--59},
  year={2009},
  publisher={IEEE}
}

@article{185Wal,
  title={Multivariable $\mathcal{H}_\infty$/$\mu$ feedback control design for high-precision wafer stage motion},
  author={van de Wal, M. and van Baars, G. and Sperling, F. and Bosgra, O.},
  journal={Control Engineering Practice},
  volume={10},
  number={7},
  pages={739--755},
  year={2002},
  publisher={Elsevier}
}

@article{187Wal,
  title={Experimentally validated multivariable $\mu$ feedback controller design for a high-precision wafer stage},
  author={van de Wal, M. and van Baars, G. and Sperling, F. and Bosgra, O.},
  booktitle={Decision and Control, 2001. Proceedings of the 40th IEEE Conference on},
  volume={2},
  pages={1583--1588},
  year={2001},
  organization={IEEE}
}

@article{188Hughes,
  title={Space structure vibration modes: How many exist? Which ones are important?},
  author={Hughes, P.},
  journal={IEEE Control Systems Magazine},
  volume={7},
  number={1},
  pages={22--28},
  year={1987},
  publisher={IEEE}
}

@article{189Schneiders, 
author={M. G. E. Schneiders and M. J. G. van de Molengraft and M. Steinbuch}, 
booktitle={Proceedings of the 2004 American Control Conference}, 
title={Benefits of over-actuation in motion systems}, 
year={2004}, 
volume={1}, 
number={}, 
pages={505-510 vol.1}, 
keywords={motion control;vibration control;actuators;feedforward;feedback;control system synthesis;motion control system;feedback controller design;vibration control strategy;disturbance attenuation;feedforward path;Actuators;Resonance;Attenuation;Controllability;Feedback;Tuning;Adaptive control;Vibration control;Bandwidth;Resonant frequency}, 
doi={10.23919/ACC.2004.1383653}, 
ISSN={0743-1619}, 
month={June},}

@inbook{190Steinbuch,
title = "Advanced Motion Control Design",
abstract = "No abstract.",
author = "M. Steinbuch and R.J.E. Merry and M.L.G. Boerlage and M.J.C. Ronde and {Molengraft, van de}, M.J.G.",
year = "2010",
doi = "10.1201/b10382-35",
language = "English",
isbn = "978-1-4200-7360-7",
pages = "27--1/25",
booktitle = "The Control Handbook, Control System Applications, Second edition",
publisher = "CRC Press",

}


@article{191Lierop,
  title={Model-based commutation of a long-stroke magnetically levitated linear actuator},
  author={van Lierop, C. M. M. and Jansen, J. W. and Damen, A. A. H. and Lomonova, E. A. and van Den Bosch, P. P. J. and Vandenput, A. J. A.},
  journal={IEEE Transactions on Industry Applications},
  volume={45},
  number={6},
  pages={1982--1990},
  year={2009},
  publisher={IEEE}
}

@misc{192Moore,
  title={Cramming more components onto integrated circuits},
  author={Moore, G. E.},
  year={1965},
  publisher={McGraw-Hill New York, NY, USA}
}

@inproceedings{193Jong,
  title={Enabling the lithography roadmap: an immersion tool based on a Novel Stage Positioning System},
  author={de Jong, F. and van der Pasch, B. and Castenmiller, T. and Vleeming, B. and Droste, R. and van de Mast, F.},
  booktitle={SPIE Advanced Lithography},
  pages={72741S--72741S},
  year={2009},
  organization={International Society for Optics and Photonics}
}

@article{194Rovers,
title = "Real-time {3D} thermal modeling of a magnetically levitated planar actuator ",
journal = "Mechatronics ",
volume = "23",
number = "2",
pages = "240 - 246",
year = "2013",
note = "Special Issue on Linear Drives ",
issn = "0957-4158",
doi = "http://dx.doi.org/10.1016/j.mechatronics.2012.04.004",
author = "Rovers, J.M.M.  and St{\"o}ck, M.  and  Jansen, J.W. and  van Lierop, C.M.M. and Lomonova,  E.A. and Perriard, Y. "
}

@inproceedings{195Rovers,
  title={Design and measurements of the double layer planar motor},
  author={Rovers, J. M. M. and Jansen, J. W. and Lomonova, E. A.},
  booktitle={Electric Machines \& Drives Conference (IEMDC), 2013 IEEE International},
  pages={204--211},
  year={2013},
  organization={IEEE}
}

@article{196Rovers,
  title={Multiphysical analysis of moving-magnet planar motor topologies},
  author={Rovers, J. M. M. and Jansen, J. W. and Lomonova, E. A.},
  journal={Magnetics, IEEE Transactions on},
  volume={49},
  number={12},
  pages={5730--5741},
  year={2013},
  publisher={IEEE}
}

@inproceedings{197Achterberg,
  title={Performance of a six Degree-of-Freedom controlled moving-magnet planar actuator with a laser interferometer measurement setup},
  author={Achterberg, J. and Rovers, J. M. M. and van Lierop, C. M. M. and Jansen, J. W. and van den Bosch, P. P. J.},
  booktitle={Eighth international symposium on linear drives for industry applications},
  year={2011},
  address = {},
  month = {}
}


@article{198Steinbuch,
title = "Advanced Motion Control: An Industrial Perspective",
journal = "European Journal of Control",
volume = "4",
number = "4",
pages = "278 - 293",
year = "1998",
issn = "0947-3580",
doi = "https://doi.org/10.1016/S0947-3580(98)70121-9",
author = "M. Steinbuch and M.L. Norg",
keywords = "Application, Compact disk, Disturbance rejection, Drives, Hard disk, Model-based control, Motion control, Robust control",
abstract = "Industrial feedback motion controllers are tuned using manual loopshaping, according to certain design rules. This controller tuning serves as a benchmark for robust control research as applied to optical and magnetic disk drive storage systems. The design and implementation of robust controllers for the focus servo of a compact disk and the tracking servo of a hard disk mechanism is investigated. The design objective is to achieve good track-following performance in the presence of disk disturbances. H∞ robust control is used to systematically include disturbance and specification models in the standard plant framework. The control design iteration is based on disturbance identification, including implementation within the design cycle. The industrial relevance of robust control is discussed and areas for academic research in robust control are indicated, as feedback from industry."
}

@inproceedings{199Chen,
  title={{LPV} control design for precision motion systems},
  author={Chen, N. and Wen, J. T.},
  booktitle={2014 American Control Conference},
  pages={4470--4475},
  year={2014},
  organization={IEEE}
}

@inproceedings{205Kasemsinsup,
  title={Exact plant inversion of flexible motion systems with a time-varying state-to-output map},
  author={Kasemsinsup, Y. and Heertjes, M. and Butler, H. and Weiland, S.},
  booktitle={2016 European Control Conference (ECC)},
  pages={2483--2488},
  year={2016},
  organization={IEEE}
}

@INPROCEEDINGS{206Boerlage, 
title={Model-based feedforward for motion systems},
author={M. {Boerlage} and M. {Steinbuch} and P. {Lambrechts} and M. {van de Wal}}, 
booktitle={Proceedings of 2003 IEEE Conference on Control Applications, 2003. CCA 2003.}, 
year={2003}, 
volume={2}, 
number={}, 
pages={1158-1163 vol.2}
}

@article{207Clayton,
  title={A review of feedforward control approaches in nanopositioning for high-speed SPM},
  author={Clayton, G. M. and Tien, S. and Leang, K. K. and Zou, Q. and Devasia, S.},
  journal={Journal of dynamic systems, measurement, and control},
  volume={131},
  number={6},
  pages={061101},
  year={2009},
  publisher={American Society of Mechanical Engineers}
}

@article{208Lambrechts,
  title={Trajectory planning and feedforward design for electromechanical motion systems},
  author={Lambrechts, P. and Boerlage, M. and Steinbuch, M.},
  journal={Control Engineering Practice},
  volume={13},
  number={2},
  pages={145--157},
  year={2005},
  publisher={Elsevier}
}

@article{209Heertjes,
  title={{MIMO} feed-forward design in wafer scanners using a gradient approximation-based algorithm},
  author={Heertjes, M. and Hennekens, D. and Steinbuch, M.},
  journal={Control Engineering Practice},
  volume={18},
  number={5},
  pages={495--506},
  year={2010},
  publisher={Elsevier}
}

@inproceedings{211Steinbuch,
  title={Experimental modelling and {LPV} control of a motion system},
  author={Steinbuch, M. and van de Molengraft, R. and van der Voort, A.},
  booktitle={American Control Conference, 2003. Proceedings of the 2003},
  volume={2},
  pages={1374--1379},
  year={2003},
  organization={IEEE}
}

@article{212Scherer,
  title={{LPV} control and full block multipliers},
  author={Scherer, C.},
  journal={Automatica},
  volume={37},
  number={3},
  pages={361--375},
  year={2001},
  publisher={Elsevier}
}

@article{214Toth,
author={R. {T\'{o}th} and M. {van de Wal} and P. S. C. {Heuberger} and P. M. J. {van den Hof}},
booktitle={Proceedings of the 2011 American Control Conference},
title={{LPV} identification of high performance positioning devices},
year={2011},
volume={},
number={},
pages={151-158},
doi={10.1109/ACC.2011.5990902},
ISSN={2378-5861},
month={June},}

@ARTICLE{221Hoffman,
author={C. {Hoffmann} and H. {Werner}},
journal={IEEE Transactions on Control Systems Technology},
title={A Survey of Linear Parameter-Varying Control Applications Validated by Experiments or High-Fidelity Simulations},
year={2015},
volume={23},
number={2},
pages={416-433},
doi={10.1109/TCST.2014.2327584},
ISSN={1063-6536},
month={March},}


@article{224Shamma,
  title={Gain scheduling: Potential hazards and possible remedies},
  author={Shamma, J. S. and Athans, M.},
  journal={IEEE Control Systems Magazine},
  volume={12},
  number={3},
  pages={101--107},
  year={1992},
  publisher={IEEE}
}

@article{237Gahinet,
author = {Gahinet, P. and Apkarian, P.},
title = {A linear matrix inequality approach to $\mathcal{H}_{\infty}$ control},
journal = {International Journal of Robust and Nonlinear Control},
volume = {4},
number = {4},
pages = {421-448},
keywords = {State-space H∞ control, Linear matrix inequalities, Riccati inequalities, Loop shaping},
doi = {10.1002/rnc.4590040403},
year = {1994}
}


@inproceedings{238Kulcsar,
title = "On the similarity state transformation for linear parameter-varying systems",
abstract = "Abstract: Similarity state transformations between equivalent State-Space (SS) representations of discrete-time Linear Parameter-Varying (LPV) systems are investigated. Based on previous results, it is known that to characterize all equivalent LPV-SS representations, the statetransformation matrix must depend dynamically on the scheduling variable. However, preserving static dependence of a LPV-SS representation, i.e. characterizing all equivalent SS representation with static dependence, has primary importance both in control and identication. Therefore, rst, the state transformation problem is investigated from an algebraic (behavior) point of view, then conditions are developed to guarantee preservation of the static dependence in similarity state transformations. Additional geometric interpretation of the obtained results, together with computational approach to synthesize state-transformations are also developed. An illustrative example is provided to demonstrate the validity of the obtained results.",
author = "B. Kulcsar and R. Toth",
year = "2011",
language = "English",
pages = "4155--4160",
booktitle = "Proceedings of the 18th IFAC World Congress, 28 August-2 September 2011, Milano, Italy",
publisher = "International Federation of Automatic Control",
}

@unpublished{240Zhang,
  TITLE = {{On local LTI model coherence for LPV interpolation}},
  AUTHOR = {Zhang, Q. and Ljung, L. and Pintelon, R.},
  NOTE = {working paper or preprint},
  YEAR = {2018},
  MONTH = Apr,
  PDF = {https://hal.inria.fr/hal-01758337/file/coherence_hal.pdf},
  HAL_ID = {hal-01758337},
  HAL_VERSION = {v1},
}

@article{241Zhang,
title = "From structurally independent local {LTI} models to {LPV} model",
journal = "Automatica",
volume = "84",
pages = "232 - 235",
year = "2017",
issn = "0005-1098",
doi = "https://doi.org/10.1016/j.automatica.2017.06.006",
author = "Qinghua Z. and Lennart L.",
abstract = "The local approach to linear parameter varying (LPV) system identification consists in interpolating individually estimated local linear time invariant (LTI) models corresponding to fixed values of the scheduling variable. It is shown in this paper that, without any global structural assumption of the considered LPV system, individually estimated local state-space LTI models do not contain sufficient information for determining similarity transformations making them coherent. It is possible to estimate these similarity transformations from input–output data under appropriate excitation conditions."
}

@ARTICLE{242Shamma, 
author={J. S. {Shamma} and M. {Athans}}, 
journal={IEEE Transactions on Automatic Control}, 
title={Analysis of gain scheduled control for nonlinear plants}, 
year={1990}, 
volume={35}, 
number={8}, 
pages={898-907}, 
keywords={control system analysis;nonlinear systems;scheduling;stability;gain scheduled control;nonlinear plants;design;robustness;reference trajectory;stability;nonlinearities;Robust stability;Processor scheduling;Performance gain;Feedback;Design methodology;Acoustical engineering;Design engineering;Performance analysis;Stability analysis;Control systems}, 
doi={10.1109/9.58498}, 
ISSN={0018-9286}, 
month={Aug},}

@article{250Mottershead,
  title={Model updating in structural dynamics: a survey},
  author={Mottershead, J. E. and Friswell, M. I.},
  journal={Journal of sound and vibration},
  volume={167},
  number={2},
  pages={347--375},
  year={1993},
  publisher={Elsevier}
}

@article{251Dorosti,
title = "Iterative pole-zero finite element model updating using generic parameters",
journal = "Mechatronics",
volume = "55",
pages = "180 - 193",
year = "2018",
issn = "0957-4158",
doi = "https://doi.org/10.1016/j.mechatronics.2018.06.012",
author = "M. Dorosti and R.H.B. Fey and M.F. Heertjes and M.M.J. van de Wal and H. Nijmeijer",
keywords = "FE model, Model updating, System identification, Prediction and control, Generic parameters",
abstract = "Prediction and control of unmeasurable performance variables in complex large-scale systems is an important topic in systems and control. The preferred solution to this problem is to have a relatively low-order and accurate standard plant model. A reduced Finite Element (FE) dynamic model may be a good candidate for that purpose apart from the fact that its accuracy is always limited, since it never truly matches the real structure. In this paper, an iterative procedure is proposed to update the FE model using poles and zeros estimated from the measured Frequency Response Functions (FRFs). Assuming the errors in the FE stiffness and/or damping matrix to be dominant over the mass matrix, but the exact physical parameters responsible for these errors to be unknown, the eigenvalues of the (sub)structure stiffness and/or damping matrix may be updated to reduce the differences between the poles and zeros from the model and measured FRFs. The proposed procedure matches poles and zeros sequentially in an iterative manner as to realize convergence to the measured quantities. This procedure, further referred to as Iterative Pole-Zero (IPZ) model updating, facilitates the process of obtaining improved parametric models which can be used for accurate prediction and control of unmeasurable performance variables. The proposed procedure is first illustrated using a mass-spring model and then is validated via a collocated FRF measurement from an experimental beam setup."
}

@article{252Mottershead,
  title={The sensitivity method in finite element model updating: a tutorial},
  author={Mottershead, J. E. and Link, M. and Friswell, M. I.},
  journal={Mechanical systems and signal processing},
  volume={25},
  number={7},
  pages={2275--2296},
  year={2011},
  publisher={Elsevier}
}

@inproceedings{260Lofberg,
address = {Taipei, Taiwan},
author = {L{\"{o}}fberg, J.},
booktitle = {In Proceedings of the CACSD Conference},
title = {{YALMIP : A Toolbox for Modeling and Optimization in MATLAB}},
year = {2004}
}

@article{270Besselink,
  title={A comparison of model reduction techniques from structural dynamics, numerical mathematics and systems and control},
  author={Besselink, B. and Tabak, U. and Lutowska, A. and van de Wouw, N. and Nijmeijer, H. and Rixen, D. J. and Hochstenbach, M. E. and Schilders, W. H. A.},
  journal={Journal of Sound and Vibration},
  volume={332},
  number={19},
  pages={4403--4422},
  year={2013},
  publisher={Elsevier}
}


@inproceedings{271Heertjes,
author={M. {Heertjes} and D. {Hennekens} and A. {van Engelen} and M. {Steinbuch}},
booktitle={Proceedings of the 48h IEEE Conference on Decision and Control (CDC) held jointly with 2009 28th Chinese Control Conference},
title={Dynamic decoupling in motion systems using a gradient approximation-based algorithm},
year={2009}
}

@article{272Meulen,
  title={Fixed structure feedforward controller design exploiting iterative trials: Application to a wafer stage and a desktop printer},
  author={van der Meulen, Stan H and Tousain, Rob L and Bosgra, Okko H},
  journal={Journal of Dynamic Systems, Measurement, and Control},
  volume={130},
  number={5},
  pages={051006},
  year={2008},
  publisher={American Society of Mechanical Engineers}
}

@article{274Arora,
  title={Comparative study of finite element model updating methods},
  author={Arora, V.},
  journal={Journal of Vibration and Control},
  volume={17},
  number={13},
  pages={2023--2039},
  year={2011},
  publisher={Sage Publications Sage UK: London, England}
}



@article{275Dorosti,
title = "Finite Element Model Reduction and Model Updating of structures for Control",
journal = "IFAC Proceedings Volumes",
volume = "47",
number = "3",
pages = "4517 - 4522",
year = "2014",
note = "19th IFAC World Congress",
issn = "1474-6670",
doi = "https://doi.org/10.3182/20140824-6-ZA-1003.01644",
author = "Dorosti, M. and Fey, R. and Heertjes, M. and van de Wal, M. and Nijmeijer, H.",
keywords = "Model updating, model reduction, finite element model, identification, model-based control"
}

@INPROCEEDINGS{276Dorosti, 
author={M. Dorosti and F. J. M. Heck and R. H. B. Fey and M. F. Heertjes and M. M. J. van de Wal and H. Nijmeijer}, 
booktitle={2016 American Control Conference (ACC)}, 
title={Frequency Response Sensitivity model updating using generic parameters}, 
year={2016}, 
volume={}, 
number={}, 
pages={6215-6220}, 
keywords={damping;eigenvalues and eigenfunctions;elastic constants;finite element analysis;frequency response;matrix algebra;2D pinned-sliding beam system;FE dynamic models;FE model updating algorithm;FRS model;damping matrix;eigenvalues;finite element dynamic models;frequency response sensitivity model;generic parameters;high-precision system;stiffness matrix;unmeasured performance variables;Computational modeling;Damping;Eigenvalues and eigenfunctions;Mathematical model;Matrix decomposition;Semiconductor device modeling;Zinc}, 
doi={10.1109/ACC.2016.7526646}, 
ISSN={}, 
month={July},}

@article{277Balas,
  title={Active control of flexible systems},
  author={Balas, M. J.},
  journal={Journal of Optimization theory and Applications},
  volume={25},
  number={3},
  pages={415--436},
  year={1978},
  publisher={Springer}
}

@article{278Rozario,
  title={Global feedforward control of spatio-temporal mechanical systems: with application to a prototype wafer stage},
  author={de Rozario, R. and Voorhoeve, R. and Aangenent, W. and Oomen, T.},
  journal={IFAC-PapersOnLine},
  volume={50},
  number={1},
  pages={14575--14580},
  year={2017},
  publisher={Elsevier}
}

@article{280Schneiders,
  title={Introduction to an integrated design for motion systems using over-actuation},
  author={Schneiders, M.G.E. and van de Molengraft, M.J.G. and Steinbuch, M.},
  booktitle={European Control Conference (ECC), 2003},
  pages={3249--3254},
  year={2003},
  organization={IEEE}
}

@inproceedings{282Galvan, 
author={S. D. Galvan and M. Heertjes and R. Dunand}, 
booktitle={2012 American Control Conference (ACC)}, 
title={Plant enhancements in motion systems by modal control}, 
year={2012}
}

@article{283Herpen,
title = "Exploiting additional actuators and sensors for nano-positioning robust motion control",
journal = "Mechatronics",
volume = "24",
number = "6",
pages = "619 - 631",
year = "2014",
issn = "0957-4158",
doi = "https://doi.org/10.1016/j.mechatronics.2014.03.008",
author = "van Herpen, R. and Oomen, T. and Kikken, E. and van de Wal, M. and Aangenent, W. and Steinbuch, M.",
keywords = "Mechatronic systems, Performance limitations, Robust control, System identification, Input–output selection"
}

@article{285Vizer,
  title={$\mathcal{H}_\infty$-norm-based optimization for the identification of gray-box {LTI} state-space model parameters},
  author={Vizer, D. and Merc{\`e}re, G. and Prot, O. and Laroche, E.},
  journal={Systems \& Control Letters},
  volume={92},
  pages={34--41},
  year={2016},
  publisher={Elsevier}
}

@article{286Bergamasco,
  title={State space model identification: from unstructured to structured models with an $\mathcal{H}_\infty$ approach},
  author={Bergamasco, M. and Lovera, M.},
  journal={IFAC Proceedings Volumes},
  volume={46},
  number={2},
  pages={202--207},
  year={2013},
  publisher={Elsevier}
}

@article{289Marcos,
  title={Development of linear-parameter-varying models for aircraft},
  author={Marcos, A. and Balas, G. J.},
  journal={Journal of Guidance, Control, and Dynamics},
  volume={27},
  number={2},
  pages={218--228},
  year={2004}
}

@ARTICLE{300Bristow, 
author={D. A. Bristow and M. Tharayil and A. G. Alleyne}, 
journal={IEEE Control Systems}, 
title={A survey of iterative learning control}, 
year={2006}, 
volume={26}, 
number={3}, 
pages={96-114}, 
keywords={adaptive control;control system analysis;control system synthesis;feedback;feedforward;iterative methods;learning systems;robust control;design techniques;feedback control;feedforward control;iterative learning control;learning algorithms;learning transient behavior;robotics;stability;Adaptive control;Chemical industry;Control systems;Error correction;Iterative methods;Learning systems;Motion control;Muscles;Open loop systems;Radio control}, 
doi={10.1109/MCS.2006.1636313}, 
ISSN={1066-033X}, 
month={June}
}

@article{284Oomen,
  title={Connecting system identification and robust control for next-generation motion control of a wafer stage},
  author={Oomen, T. and van Herpen, R. and Quist, S. and van de Wal, M. and Bosgra, O. and Steinbuch, M.},
  journal={IEEE Transactions on Control Systems Technology},
  volume={22},
  number={1},
  pages={102--118},
  year={2014},
  publisher={IEEE}
}

@article{287Taamallah,
  title={{LPV} modelling with affine dependence: A local $\mathcal{H}_{\infty}$ approach},
  author={Taamallah, S. and Bombois, X. and T{\'o}th, R. and van den Hof, P. M. J.},
  journal={International Journal of RObust and Nonlinear Control},
  pages={1--19},
  year={2016},
  publisher={John Wiley and Sons, Ltd.},
  year={2016}
}

@INPROCEEDINGS{288Taamallah,
author={S. {Taamallah} and X. {Bombois} and P. M. J. {van den Hof}},
booktitle={52nd IEEE Conference on Decision and Control},
title={Affine {LPV} modeling: An $\mathcal{H}_{\infty}$ based approach},
year={2013},
volume={},
number={},
pages={2726-2733},
doi={10.1109/CDC.2013.6760295},
ISSN={0191-2216},
month={Dec},}

@article{301Mishra,
  title={Precision positioning of wafer scanners segmented iterative learning control for nonrepetitive disturbances [applications of control]},
  author={Mishra, S. and Coaplen, J. and Tomizuka, M.},
  journal={IEEE control systems},
  volume={27},
  number={4},
  pages={20--25},
  year={2007},
  publisher={IEEE}
}

@ARTICLE{302Bolder, 
author={J. Bolder and T. Oomen}, 
journal={IEEE Transactions on Control Systems Technology}, 
title={Rational Basis Functions in Iterative Learning Control - With Experimental Verification on a Motion System}, 
year={2015}, 
volume={23}, 
number={2}, 
pages={722-729}, 
keywords={extrapolation;iterative learning control;optimisation;ILC approaches;complex optimization problem;exogenous signals;experimental verification;extrapolation properties;iterative learning control;iterative optimization algorithm;motion system;rational basis functions;setpoint variations;single-input single-output systems;Convolution;Extrapolation;Feedforward neural networks;Finite impulse response filters;Optimization;Polynomials;Vectors;Basis functions;iterative learning control (ILC);optimal control;optimal control.}, 
doi={10.1109/TCST.2014.2327578}, 
ISSN={1063-6536}, 
month={March}
}


@article{303Butler,
title = "Magnetic disturbance compensation for a reticle stage in a lithographic tool",
journal = "Mechatronics",
volume = "23",
number = "6",
pages = "559 - 565",
year = "2013",
issn = "0957-4158",
doi = "https://doi.org/10.1016/j.mechatronics.2013.04.011",
author = "Butler, H.",
keywords = "Reticle stage, Lithography, Feedforward, Magnetic interaction"
}

@article{309Hof,
  title={Closed-loop issues in system identification},
  author={van den Hof, P. M. J.},
  journal={Annual reviews in control},
  volume={22},
  pages={173--186},
  year={1998},
  publisher={Elsevier}
}



@article{310Darwish,
title = "Prediction-error identification of {LPV} systems: A nonparametric {Gaussian} regression approach",
journal = "Automatica",
volume = "97",
pages = "92 - 103",
year = "2018",
issn = "0005-1098",
doi = "https://doi.org/10.1016/j.automatica.2018.07.032",
author = "M.A.H. Darwish and P.B. Cox and I. Proimadis and G. Pillonetto and R. T{\'o}th"
}

@inproceedings{313Callafon,
author={R. A. {de Callafon} and D. {de Roover} and P. M. J. {van den Hof}},
title={Multivariable least squares frequency domain identification using polynomial matrix fraction descriptions},
booktitle={Proceedings of 35th IEEE Conference on Decision and Control},
year={1996}
}

@article{316Voorhoeve,
  author={Voorhoeve, R. and {de Rozario}, R. and Aangenent, W. and Oomen, T.},
  title={Identifying Position-Dependent Mechanical Systems: A Modal Approach with Applications to Wafer Stage Control},
  journal={{arXiv preprint arXiv:1807.06942}},
  year={2018}
}


@ARTICLE{317Mercere,
author={G. {Merc{\`e}re} and O. {Prot} and J. A. {Ramos}},
journal={IEEE Transactions on Automatic Control},
title={Identification of Parameterized Gray-Box State-Space Systems: From a Black-Box Linear Time-Invariant Representation to a Structured One},
year={2014},
volume={59},
number={11},
pages={2873-2885},
ISSN={0018-9286},
month={Nov}
}

@inproceedings{321Vizer,
  title={A local approach framework for black-box and gray-box {LPV} system identification},
  author={Vizer, D. and Merc{\`e}re, G. and Prot, O. and Ramos, J.},
  booktitle={2013 European Control Conference (ECC)},
  pages={1916--1921},
  year={2013},
  organization={IEEE}
}

@inproceedings{322Vizer,
author={D. {Vizer} and G. {Merc{\`e}re}},
booktitle={2014 European Control Conference (ECC)},
title={$\mathcal{H}_{\infty}$-based {LPV} model identification from local experiments with a gap metric-based operating point selection},
year={2014}
}


@incollection{323Vizer,
  TITLE = {{Linear fractional LPV model identification from local experiments using an $\mathcal{H}_\infty$-based glocal approach}},
  AUTHOR = {Vizer, D. and Merc{\`e}re, G. and Laroche, E. and Prot, O.},
  BOOKTITLE = {{Control-oriented modelling and identification : theory and practice}},
  EDITOR = {M. Lovera},
  PUBLISHER = {{The Institution of Engineering and Technology}},
  PAGES = {189-213},
  YEAR = {2015},
  DOI = {10.1049/PBCE080E\_ch9 },
  HAL_ID = {hal-01313923},
  HAL_VERSION = {v1},
}

@article{325Lu,
title = "{6D} direct-drive technology for planar motion stages",
journal = "CIRP Annals",
volume = "61",
number = "1",
pages = "359 - 362",
year = "2012",
issn = "0007-8506",
doi = "https://doi.org/10.1016/j.cirp.2012.03.145",
author = "Xiaodong, L. and Usman, I. ",
keywords = "Actuator, Mechatronic, Magnetic bearing",
abstract = "Achieving 6D direct drive motion control over long planar strokes on a single mover can greatly improve machine performance. Existing solutions are either limited to small-stroke applications (a fraction of the stage size) or require a large number of coils with enormous control complexity. This paper presents a novel 6D direct drive technology for planar stages with many advantages: (1) stroke can be on the order of several meters; (2) the number of coils increases linearly with motion range; (3) no end effects or force coupling between axes; and (4) ease of control and superior force linearity."
}

@article{326Caigny,
  title={Interpolated modeling of {LPV} systems based on observability and controllability},
  author={Caigny, J and Pintelon, Rik and Camino, Juan F and Swevers, Jan},
  journal={IFAC Proceedings Volumes},
  volume={45},
  number={16},
  pages={1773--1778},
  year={2012},
  publisher={Elsevier}
}

@article{327Caigny,
  title={Interpolated modeling of {LPV} systems},
  author={de Caigny, J. and Pintelon, R. and Camino, J. F. and Swevers, J.},
  journal={IEEE Transactions on Control Systems Technology},
  volume={22},
  number={6},
  pages={2232--2246},
  year={2014},
  publisher={IEEE}
}

@article{328Schmidt,
  title={Distilling free-form natural laws from experimental data},
  author={Schmidt, M. and Lipson, H.},
  journal={science},
  volume={324},
  number={5923},
  pages={81--85},
  year={2009},
  publisher={American Association for the Advancement of Science}
}
@InProceedings{329Duvenaud,
  title = 	 {Structure Discovery in Nonparametric Regression through Compositional Kernel Search},
  author = 	 {Duvenaud, D. and Lloyd, J.R. and Grosse, R. and Tenenbaum, J. and Ghahramani, Z.},
  booktitle = 	 {Proceedings of the 30th International Conference on Machine Learning},
  pages = 	 {1166--1174},
  year = 	 {2013},
  volume = 	 {28},
  number =       {3},
  series = 	 {Proceedings of Machine Learning Research},
  address = 	 {Atlanta, Georgia, USA},
  month = 	 {17--19 Jun},
  publisher = 	 {PMLR}
}

@article{330Prot,
title = "Initialization of Gradient-based Optimization Algorithms for the Identification of Structured State-Space Models",
journal = "IFAC Proceedings Volumes",
volume = "44",
number = "1",
pages = "10782 - 10787",
year = "2011",
note = "18th IFAC World Congress",
issn = "1474-6670",
doi = "https://doi.org/10.3182/20110828-6-IT-1002.02879",
author = "Prot, O. and Merc{\`e}re, G.",
keywords = "System identification, Convex optimization, Iterative methods, Parameterization"
}


@inproceedings{331Petersson,
  author={Petersson, D. and L{\"o}fberg, J.},
  title={Optimization based {LPV}-approximation of multi-model systems},
  booktitle={2009 European Control Conference (ECC)},
  year={2009},
  pages={3172--3177},  
  organization={IEEE}
}

@inproceedings{332Xie,
	author={Xie, L.L. and Ljung, L.},
  	title={Estimate physical parameters by black box modeling},
  	booktitle={Proceedings of the 21st Chinese Control Conference},
  	year={2002}
}


@article{333Mercere,
author={Merc{\`e}re, G. and Laroche, E. and Prot, O.},
title = "Analytical Modelling and Grey-box Identification of a Flexible Arm using a Linear Parameter-varying Model",
journal = "IFAC Proceedings Volumes",
volume = "45",
number = "16",
pages = "1251 - 1256",
year = "2012",
note = "16th IFAC Symposium on System Identification",
issn = "1474-6670"
}

@inproceedings{334Paijmans,
author={B. {Paijmans} and W. {Symens} and H. {van Brussel} and J. {Swevers}},
title={A gain-scheduling-control technique for mechatronic systems with position-dependent dynamics},
booktitle={2006 American Control Conference},
year={2006}
}

@ARTICLE{335Callafon,
author={R. A. {de Callafon} and P. M. J. {van den Hof}},
journal={IEEE Transactions on Control Systems Technology},
title={Multivariable feedback relevant system identification of a wafer stepper system},
year={2001},
volume={9},
number={2},
pages={381-390},
ISSN={1063-6536},
month={March},}

@article{336Maas,
  title={Accurate FRF identification of LPV systems: nD-LPM with application to a medical X-ray system},
  author={van der Maas, R. and van der Maas, A. and Voorhoeve, R. and Oomen, T.},
  journal={IEEE Transactions on Control Systems Technology},
  volume={25},
  number={5},
  pages={1724--1735},
  year={2016},
  publisher={IEEE}
}

@article{337Voorhoeve,
  title={Non-parametric identification of multivariable systems: A local rational modeling approach with application to a vibration isolation benchmark},
  author={Voorhoeve, R. and van der Maas, A. and Oomen, T.},
  journal={Mechanical Systems and Signal Processing},
  volume={105},
  pages={129--152},
  year={2018},
  publisher={Elsevier}
}



@ARTICLE{340Dobrowiecki,
author={T. P. {Dobrowiecki} and J. {Schoukens} and P. {Guillaume}},
journal={IEEE Transactions on Instrumentation and Measurement},
title={Optimized Excitation Signals for {MIMO} Frequency Response Function Measurements},
year={2006},
volume={55},
number={6},
pages={2072-2079},
doi={10.1109/TIM.2006.887036},
ISSN={0018-9456},
month={Dec},}

@article{344Boeij,
  title={Contactless planar actuator with manipulator: A motion system without cables and physical contact between the mover and the fixed world},
  author={de Boeij, J. and Lomonova, E. and Duarte, J.},
  journal={IEEE Transactions on Industry Applications},
  volume={45},
  number={6},
  pages={1930--1938},
  year={2009},
  publisher={IEEE}
}


@ARTICLE{345Balakrishnan, 
author={V. {Balakrishnan} and L. {Vandenberghe}}, 
journal={IEEE Transactions on Automatic Control}, 
title={Semidefinite programming duality and linear time-invariant systems}, 
year={2003}, 
volume={48}, 
number={1}, 
pages={30-41}, 
keywords={eigenvalues and eigenfunctions;linear matrix inequalities;time-varying systems;linear systems;convex programming;semidefinite programming duality;linear time-invariant systems;linear matrix inequality constraints;convex optimization duality;dual optimization problems;system theoretic terms;Linear programming;Linear matrix inequalities;Application software;Control theory;Control systems;Control system synthesis;Riccati equations;Qualifications;Controllability;Constraint theory}, 
doi={10.1109/TAC.2002.806652}, 
ISSN={0018-9286}, 
month={Jan},}


@article{348Caughey,
  title={Classical normal modes in damped linear dynamic systems},
  author={O'Kelly, M. E. J. and Caughey, T. K.},
  journal={Journal of Applied Mechanics},
  volume={32},
  number={3},
  pages={583--588},
  year={1965}
}

@article{349Li,
  title={Thermal-error modeling for complex physical systems: the-state-of-arts review},
  author={Li, J.W. and Zhang, W.J. and Yang, G.S. and Tu, S.D. and Chen, X.B.},
  journal={The International Journal of Advanced Manufacturing Technology},
  volume={42},
  number={1-2},
  pages={168},
  year={2009},
  publisher={Springer}
}



@inproceedings{350Boerlage,
  title={Jerk derivative feedforward control for motion systems},
  author={Boerlage, M. and Tousain, R. and Steinbuch, M.},
  booktitle={Proceedings of the 2004 American Control Conference},
  volume={5},
  pages={4843--4848},
  year={2004},
  organization={IEEE}
}

@inproceedings{351Zou,
  title={Preview-based stable-inversion for output tracking},
  author={Zou, Q. and Devasia, S.},
  booktitle={Proceedings of the 1999 American Control Conference (Cat. No. 99CH36251)},
  volume={5},
  pages={3544--3548},
  year={1999},
  organization={IEEE}
}

@ARTICLE{352Devasia, 
author={S. {Devasia} and B. {Paden}}, 
journal={IEEE Transactions on Automatic Control}, 
title={Stable inversion for nonlinear nonminimum-phase time-varying systems}, 
year={1998}, 
volume={43}, 
number={2}, 
pages={283-288},
ISSN={0018-9286}, 
month={Feb}
}

@inproceedings{353Bloemers,
  title={Parameter-dependent feedforward strategies for motion systems},
  author={Bloemers, T.A.H. and Proimadis, I. and Kasemsinsup, Y. and T{\'o}th, R.},
  booktitle={2018 Annual American Control Conference (ACC)},
  pages={2017--2022},
  year={2018},
  organization={IEEE}
}



@article{354Bristow,
  title={A survey of iterative learning control},
  author={Bristow, D. A. and Tharayil, M. and Alleyne, A. G.},
  journal={IEEE control systems magazine},
  volume={26},
  number={3},
  pages={96--114},
  year={2006},
  publisher={IEEE}
}

@inproceedings{355Stearns,
  title={A comparative study of feedforward tuning methods for wafer scanning systems},
  author={Stearns, H. and Yu, S. and Fine, B. and Mishra, S. and Tomizuka, M.},
  booktitle={ASME 2008 Dynamic Systems and Control Conference},
  pages={669--676},
  year={2008},
  organization={American Society of Mechanical Engineers}
}

@inproceedings{356Theis,
  title={Linear parameter-varying feedforward control: A missile autopilot design},
  author={Theis, J. and Pfifer, H. and Knoblach, A. and Saupe, F. and Werner, H.},
  booktitle={AIAA Guidance, Navigation, and Control Conference},
  pages={2001},
  year={2015}
}

@article{357Mayne,
author={D. Q. {Mayne}},
journal={Proceedings of the Institution of Electrical Engineers},
title={Sequential design of linear multivariable systems},
year={1979},
volume={126},
number={6},
pages={568-572},
doi={10.1049/piee.1979.0135},
ISSN={0020-3270},
month={June}
}

@article{358Custers,
author = {C.H.H.M. Custers and J.W. Jansen and M.C. van Beurden and E.A. Lomonova},
title = {3{D} harmonic modeling of eddy currents in segmented conducting structures},
journal = {COMPEL - The international journal for computation and mathematics in electrical and electronic engineering},
volume = {38},
number = {1},
pages = {2-23},
year = {2019},
doi = {10.1108/COMPEL-02-2018-0070}
}

@INPROCEEDINGS{359Custers, 
author={C. H. H. M. {Custers} and J. W. {Jansen} and E. A. {Lomonova}}, 
booktitle={2017 IEEE International Electric Machines and Drives Conference (IEMDC)}, 
title={Static decoupling of force and torque components in a moving-magnet planar motor}, 
year={2017}, 
volume={}, 
number={}, 
pages={1-8}, 
doi={10.1109/IEMDC.2017.8002065}, 
ISSN={}, 
month={May}
}




@article{365Freeth,
  title={Decoding the ancient Greek astronomical calculator known as the Antikythera Mechanism},
  author={Freeth, T. and Bitsakis, Y. and Moussas, X. and Seiradakis, J. H. and Tselikas, A. and Mangou, H. and Zafeiropoulou, M. and Hadland, R. and Bate, D. and Ramsey, A. and others},
  journal={Nature},
  volume={444},
  number={7119},
  pages={587},
  year={2006},
  publisher={Nature Publishing Group}
}

@book{366Hobsbawm,
  title={Age of revolution: 1789-1848},
  author={Hobsbawm, E.},
  year={2010},
  publisher={Hachette UK}
}

@ARTICLE{367Kang, 
author={C. {Kang}}, 
journal={IEEE Control Systems Magazine}, 
title={{Origin of Stability Analysis: ``On Governors'' by J.C. Maxwell [Historical Perspectives]}}, 
year={2016}, 
volume={36}, 
number={5}, 
pages={77-88}, 
keywords={History;Stability criteria;Differential equations;Water clocks;Brakes}, 
doi={10.1109/MCS.2016.2584358}, 
ISSN={1066-033X}, 
month={Oct},}

@article{368Mayr,
  title={The origins of feedback control},
  author={Mayr, O.},
  journal={Scientific American},
  volume={223},
  number={4},
  pages={110--119},
  year={1970},
  publisher={JSTOR}
}

@misc{369Sawyer,
  title={Magnetic positioning device},
  author={Sawyer, B. A.},
  year={1968},
  month=apr # "~2",
  publisher={Google Patents},
  note={US Patent 3,376,578}
}

@ARTICLE{370Cho, 
author={ Cho, H.S. and Im, C. H. and Jung, H. K.}, 
journal={IEEE Transactions on Magnetics}, 
title={Magnetic field analysis of 2-D permanent magnet array for planar motor}, 
year={2001}, 
volume={37}, 
number={5}, 
pages={3762-3766}, 
keywords={magnetic fields;permanent magnet motors;magnetic flux;synchronous motors;magnetic field analysis;2D permanent magnet array;planar motor;flux density distribution;scalar magnetic potential equation;Magnetic fields;Magnetic analysis;Planar motors;Magnetic flux;Synchronous motors;Permanent magnet motors;Stators;Equations;Coils;Laboratories}, 
doi={10.1109/20.952708}, 
ISSN={0018-9464}, 
month={Sep.},}

@article{371Kim,
title = "High-precision magnetic levitation stage for photolithography",
journal = "Precision Engineering",
volume = "22",
number = "2",
pages = "66 - 77",
year = "1998",
issn = "0141-6359",
doi = "https://doi.org/10.1016/S0141-6359(98)00009-9",
author = "Kim, W.  and Trumper, D.L. ",
keywords = "precision motion control, photolithography, magnetic levitation, mechatronics",
abstract = "In this paper, we present a high-precision magnetic levitation (maglev) stage for photolithography in semiconductor manufacturing. This stage is the world’s first maglev stage that provides fine six-degree-of-freedom motion controls and realizes large (50 mm × 50 mm) planar motions with only a single magnetically levitated moving part. The key element of this stage is a linear motor capable of providing forces in both suspension and translation without contact. The advantage of such a stage is that the mechanical design is far simpler than competing conventional approaches and, thus, promises faster dynamic response and higher mechanical reliability. The stage operates with a positioning noise as low as 5 nm rms in x and y, and acceleration capabilities in excess of 1 g (10 m/s2). We demonstrate the utility of this stage for next-generation photolithography or in other high-precision motion control applications."
}

@INPROCEEDINGS{372Boerj, 
	author={J. {de Boeij} and E. {Lomonova} and J. {Duarte}},
		title={Contactless Planar Actuator with Manipulator: a Motion System without Cables and Physical Contact between the Mover and the Fixed World}, 
		 booktitle={2008 IEEE Industry Applications Society Annual Meeting}, 
	year={2008}
} 

@phdthesis{373Roover,
  title={Motion control of a wafer stage},
  author={de Roover, D.},
  school={Delft University of Technology},
  year={1997}
}

@article{374Ronde,
  title={Data-based spatial feedforward for over-actuated motion systems},
  author={Ronde, M.J.C. and Leenknegt, G.A.L. and van de Molengraft, M.J.G. and Steinbuch, M.},
  journal={Mechatronics},
  volume={24},
  number={6},
  pages={679--690},
  year={2014},
  publisher={Elsevier}
}

@article{375Halbach,
title = "Design of permanent multipole magnets with oriented rare earth cobalt material",
journal = "Nuclear Instruments and Methods",
volume = "169",
number = "1",
pages = "1 - 10",
year = "1980",
issn = "0029-554X",
doi = "https://doi.org/10.1016/0029-554X(80)90094-4",
author = "K. Halbach"
}

@article{376Ronde,
title = "Model-based spatial feedforward for over-actuated motion systems",
journal = "Mechatronics",
volume = "24",
number = "4",
pages = "307 - 317",
year = "2014",
note = "Vibration control systems",
issn = "0957-4158",
doi = "https://doi.org/10.1016/j.mechatronics.2013.09.010",
author = "M.J.C. Ronde and M.G.E. Schneiders and E.J.G.J. Kikken and M.J.G. van de Molengraft and M. Steinbuch",
}


@inproceedings{377Baggen,
author={M. {Baggen} and M. {Heertjes} and R. {Kamidi}},
title={Data-based feed-forward control in {MIMO} motion systems},
booktitle={2008 American Control Conference},
year={2008},
pages={3011-3016}
}

@book{378Kocijan,
  title={Modelling and control of dynamic systems using {Gaussian} process models},
  author={Kocijan, J.}},
  year={2016},
  publisher={Springer}
}

@article{380Tibshirani,
  title={Regression shrinkage and selection via the lasso},
  author={Tibshirani, R.},
  journal={Journal of the Royal Statistical Society: Series B (Methodological)},
  volume={58},
  number={1},
  pages={267--288},
  year={1996},
  publisher={Wiley Online Library}
}

@article{381Recht,
  title={Guaranteed minimum-rank solutions of linear matrix equations via nuclear norm minimization},
  author={Recht, B. and Fazel, M. and Parrilo, P. A.},
  journal={SIAM review},
  volume={52},
  number={3},
  pages={471--501},
  year={2010},
  publisher={SIAM}
}

@article{382Kimeldorf,
  title={Some results on Tchebycheffian spline functions},
  author={Kimeldorf, G. and Wahba, G.},
  journal={Journal of mathematical analysis and applications},
  volume={33},
  number={1},
  pages={82--95},
  year={1971},
  publisher={Elsevier}
}

@ARTICLE{383Aravkin, 
author={A. Y. {Aravkin} and B. M. {Bell} and J. V. {Burke} and G. {Pillonetto}}, 
journal={IEEE Transactions on Neural Networks and Learning Systems}, 
title={{The Connection Between Bayesian Estimation of a Gaussian Random Field and RKHS}}, 
year={2015}, 
volume={26}, 
number={7}, 
pages={1518-1524}, 
doi={10.1109/TNNLS.2014.2337939}, 
ISSN={2162-237X}, 
month={July},}


@article{384Mackay,
  title={{Introduction to Gaussian processes}},
  author={MacKay, D. J. C.},
  journal={NATO ASI Series F Computer and Systems Sciences},
  volume={168},
  pages={133--166},
  year={1998},
  publisher={Springer Verlag}
}


@article{385Tresp,
  title={{A Bayesian committee machine}},
  author={Tresp, V.},
  journal={Neural computation},
  volume={12},
  number={11},
  pages={2719--2741},
  year={2000},
  publisher={MIT Press}
}

@INBOOK{386Bottu,
author={L. {Bottou} and O. {Chapelle} and D. {DeCoste} and J. {Weston}},
title={Large-Scale Kernel Machines},
year={2007},
volume={},
number={},
pages={},
keywords={},
doi={},
ISSN={},
publisher={MIT Press},
isbn={9780262255790}
}

@article{387Quinonero,
  title={Approximation methods for Gaussian process regression},
  author={Quinonero-Candela, J. and Rasmussen, C. E. and Williams, C. K. I.},
  journal={Large-scale kernel machines},
  pages={203--224},
  year={2007},
  publisher={MIT Press}
}

@article{389Edwards,
author = {Edwards, C. and Postlethwaite, I.},
title = "Anti-windup and bumpless-transfer schemes",
journal = "Automatica",
volume = "34",
number = "2",
pages = "199 - 210",
year = "1998",
issn = "0005-1098",
doi = "https://doi.org/10.1016/S0005-1098(97)00165-9"
}


@article{390Peng,
author = {Peng, Y. and Vran\v{v}i\'{c}, D. and Hanus, R.},
year = {1996},
month = {09},
pages = {48 - 57},
title = {Antiwindup, Bumpless, and Conditioned Transfer Techniques for PID Controllers},
volume = {16},
journal = {Control Systems, IEEE},
doi = {10.1109/37.526915}
}

@article{391Kowalski,
title = "Implementation of a linear quadratic bumpless transfer method to a magnetically levitated planar actuator with moving magnets",
author = "K.K. Kowalski and J. Achterberg and {Lierop, van}, C.M.M. and {Bosch, van den}, P.P.J.",
year = "2010",
booktitle = "Proceedings of the 2010 IEEE International Conference on Control Applications (CCA 2010), part of the 2010 IEEE Multi-Conference on Systems and Control (MSC 2010), 8-10 September 2010, Yokohama, Japan"
}

@article{392Turner,
title = "Linear quadratic bumpless transfer",
journal = "Automatica",
volume = "36",
number = "8",
pages = "1089 - 1101",
year = "2000",
issn = "0005-1098",
doi = "https://doi.org/10.1016/S0005-1098(00)00021-2",
author = "Turner, M. C. and Walker, D. J.",
}

@article{393Amidror,
  title={Scattered data interpolation methods for electronic imaging systems: a survey},
  author={Amidror, I.},
  journal={Journal of electronic imaging},
  volume={11},
  pages={157--76},
  year={2002}
}


@article{394Englehart,
title = "A four-block problem for $H_{\infty}$ design: Properties and applications",
 author={Englehart, M. J. and Smith, M. C.},
journal = "Automatica",
volume = "27",
number = "5",
pages = "811 - 818",
year = "1991",
issn = "0005-1098",
doi = "https://doi.org/10.1016/0005-1098(91)90035-Z"
}

@mastersthesis{395Bloemers,
title={Nanometer accurate motion control of a magnetically levitated planar actuator},
author={
Bloemers, T.A.H.},
year={2018},
school={Eindhoven University of Technology, Department of Electrical Engineering, Control Systems Group}
}

@inproceedings{396Wortelboer, 
author={P. M. R. {Wortelboer} and O. H. {Bosgra}}, 
title={Frequency weighted closed-loop order reduction in the control design configuration}, 
booktitle={Proceedings of 1994 33rd IEEE Conference on Decision and Control}, 
year={1994}, 
}

@article{397Grosdidier,
title = "Interaction measures for systems under decentralized control",
journal = "Automatica",
volume = "22",
number = "3",
pages = "309 - 319",
year = "1986",
issn = "0005-1098",
doi = "https://doi.org/10.1016/0005-1098(86)90029-4",
author = "Grosdidier, P. and Morari, M."
}

@article{398Heertjes,
title = "Minimizing cross-talk in high-precision motion systems using data-based dynamic decoupling",
journal = "Control Engineering Practice",
volume = "19",
number = "12",
pages = "1423 - 1432",
year = "2011",
issn = "0967-0661",
doi = "https://doi.org/10.1016/j.conengprac.2011.07.016",
author = "Heertjes, M. and van Engelen, A.",
keywords = "Dynamic decoupling, Iterative schemes, Autotuning, Disturbance rejection, Industrial applications of optimal control"
}

@inproceedings{399Vaes,
author={D. {Vaes} and J. {Swevers} and P. {Sas}},
booktitle={Proceedings of the 2004 American Control Conference},
title={Optimal decoupling for {MIMO}-controller design with robust performance},
year={2004}
}

@ARTICLE{400Paattilammi,
author={J. {Paattilammi} and P. M. {Makila}},
journal={IEEE Control Systems Magazine},
title={Fragility and robustness: a case study on paper machine headbox control},
year={2000},
volume={20},
number={1},
pages={13-22},
doi={10.1109/37.823222},
ISSN={},
month={Feb}
}


@inproceedings{401Ravi,
author={R. {Ravi} and J. {Chen} and C. N. {Nett}},
booktitle={Proceedings of the 31st IEEE Conference on Decision and Control},
title={Computing nominal models for uncertain plants},
year={1992}
}

@article{402Devasia,
  title={Should model-based inverse inputs be used as feedforward under plant uncertainty?},
  author={Devasia, Santosh},
  journal={IEEE Transactions on Automatic Control},
  volume={47},
  number={11},
  pages={1865--1871},
  year={2002},
  publisher={IEEE}
}

@article{403Gelder,
  title={Nominal and robust feedforward design with time domain constraints applied to a wafer stage},
  author={de Gelder, E. and van de Wal, M. and Scherer, C. and Hol, C. and Bosgra, O.},
  journal={Journal of dynamic systems, measurement, and control},
  volume={128},
  number={2},
  pages={204--215},
  year={2006},
  publisher={American Society of Mechanical Engineers}
}

@article{404Rozario,
author={R. {de Rozario} and T. {Oomen} and M. {Steinbuch}},
booktitle={2017 American Control Conference (ACC)},
title={Iterative Learning Control and feedforward for LPV systems: Applied to a position-dependent motion system},
year={2017},
volume={},
number={},
pages={3518-3523},
month={May},}

@article{405Pintelon,
  title={Estimation of nonparametric noise and FRF models for multivariable systems—Part I: Theory},
  author={Pintelon, Rik and Schoukens, Johan and Vandersteen, Gerd and Barb{\'e}, Kurt},
  journal={Mechanical Systems and Signal Processing},
  volume={24},
  number={3},
  pages={573--595},
  year={2010},
  publisher={Elsevier}
}
@article{406Wollnack,
title = "Fixed-structure {LPV-IO} controllers: An implicit representation based approach",
journal = "Automatica",
volume = "83",
pages = "282 - 289",
year = "2017",
issn = "0005-1098",
doi = "https://doi.org/10.1016/j.automatica.2017.06.009",
author = "S. Wollnack and H.S. Abbas and R. T{\'o}th and H. Werner",
keywords = "Linear parameter-varying, Fixed-structure, Input–output"
}


@inproceedings{407Wollnack,
author={S. {Wollnack} and H. {Werner}},
booktitle={2016 American Control Conference (ACC)},
title={{LPV-IO controller design: An LMI approach}},
year={2016}
}


@article{409Schaller,
  title={Moore's law: past, present and future},
  author={Schaller, R.},
  journal={IEEE spectrum},
  volume={34},
  number={6},
  pages={52--59},
  year={1997},
  publisher={IEEE}
}

@article{410Kontaras,
title = "Continuous compliance compensation of position-dependent flexible structures",
journal = "IFAC-PapersOnLine",
volume = "49",
number = "13",
pages = "76 - 81",
year = "2016",
note = "12th IFAC Workshop on Adaptation and Learning in Control and Signal Processing ALCOSP 2016",
issn = "2405-8963",
author = "Kontaras, N. and Heertjes, M. and Zwart, H."
}

@article{411Wal,
  title={A review of methods for input/output selection},
  author={van de Wal, M. and de Jager, B.},
  journal={Automatica},
  volume={37},
  number={4},
  pages={487--510},
  year={2001},
  publisher={Elsevier}
}

@article{412Csato,
  title={Sparse on-line Gaussian processes},
  author={Csat{\'o}, L. and Opper, M.},
  journal={Neural computation},
  volume={14},
  number={3},
  pages={641--668},
  year={2002},
  publisher={MIT Press}
}

@inproceedings{413Arehart,
author={A. B. {Arehart} and W. A. {Wolovich}},
booktitle={Proceedings of 35th IEEE Conference on Decision and Control},
title={Bumpless switching controllers},
year={1996}
}

@article{414Pillonetto,
author={G. {Pillonetto} and A. {Chiuso}},
booktitle={2014 European Control Conference (ECC)},
title={Tuning complexity in kernel-based linear system identification: The robustness of the marginal likelihood estimator},
year={2014},
volume={},
number={},
pages={2386-2391},
doi={10.1109/ECC.2014.6862629},
ISSN={null},
month={June}
}

@inproceedings{415Rasmussen,
  author={Rasmussen, C. E. and Ghahramani, Z.},
  title={Occam's razor},
  booktitle={Advances in neural information processing systems},
  year={2001},
  pages={294--300}
}

@article{416Maxwell,
  title={{I. On governors}},
  author={Maxwell, James Clerk},
  journal={Proceedings of the Royal Society of London},
  number={16},
  pages={270--283},
  year={1868},
  publisher={The Royal Society London},
  address = {}
}

@article{417Schmidt,
  title={Ultra-precision engineering in lithographic exposure equipment for the semiconductor industry},
  author={Schmidt, Robert-H Munnig},
  journal={Philosophical Transactions of the Royal Society A: Mathematical, Physical and Engineering Sciences},
  volume={370},
  number={1973},
  pages={3950--3972},
  year={2012},
  publisher={The Royal Society Publishing}
}

@inproceedings{418Custers,
  title={Active Compensation of the Deformation of a Magnetically Levitated Mover of a Planar Motor},
  author={Custers, CHHM and Proimadis, Ioannis and Jansen, JW and Butler, Hans and Toth, Roland and Lomonova, EA and van den Hof, PMJ},
  booktitle={2019 IEEE International Electric Machines \& Drives Conference (IEMDC)},
  pages={854--861},
  year={2019},
  organization={IEEE}
}

@article{419Lierop,
  title={Commutation of a magnetically levitated planar actuator with moving-magnets},
  author={Jansen, J.W. and Lomonova, E.A. and Damen, A.A.H. and van den Bosch, P.P.J. and Vandenput, A.J.A.},
  journal={IEEJ Transactions on Industry Applications},
  volume={128},
  number={12},
  pages={1333--1338},
  year={2008},
  publisher={The Institute of Electrical Engineers of Japan}
}


==> YorickBroens_BeneluxConference2022_Final (1)/MyBib.tex <==
\Sort{
  Mode{on}
  Collation{mixed}
  SortTypeOrder{pattern,key,name}
  NameOrder{ascending}
  Key{{author,editor},\year{year,note}}
  KeyOrder{descending,nulls first}
  Pattern{author+editor: "doron"}
  PatternOrder{first}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{whitbeck1978digital,
  title={Digital control law synthesis in the w'domain},
  author={Whitbeck, RF and Hofmannf, LG},
  journal={Journal of Guidance and Control},
  volume={1},
  number={5},
  pages={319--326},
  year={1978}
}

@book{zhou1998essentials,
  title={Essentials of robust control},
  author={Zhou, Kemin and Doyle, John Comstock},
  volume={104},
  year={1998},
  publisher={Prentice hall Upper Saddle River, NJ}
}

 @book{sysidToolbox,
  title={System Identification Toolbox: User's guide},
  author={Ljung, L.},
  year={2019},
  publisher={MathWorks}
 }
 
 
@manual{agilentDatasheet,
    organization  = "Agilent Laser and Optics",
    title         = "User’s Manual, Volume I",
    number        = "05517-90086",
    year          =  2007
}

@manual{agilentDatasheet,
    organization  = "Agilent Laser and Optics",
    title         = "User’s Manual, Volume I",
    number        = "05517-90086",
    year          =  2007
}

@MANUAL{ansysSoftware,
title = { ANSYS Academic Research Mechanical, Release 17.1},
organization = {ANSYS Inc.},
}

@manual{agilentDatasheetFull,
    organization  = "Keysight Technologies",
    title         = "Optics and Laser Heads for Laser-Interferometer Positioning Systems",
    number        = "5964-6190E",
    year          =  2017
}


 @misc{ refPhotoGovernor,
   author = "{Wikimedia Commons}",
   title = "File:Centrifugal governor.svg --- Wikimedia Commons{,} the free media repository",
   year = "2017",
   url = "https://commons.wikimedia.org/w/index.php?title=File:Centrifugal_governor.svg&oldid=234951643",
 }

@misc{refAppleChip,
author  = "{Apple press release}",
title = {{Apple introduces iPhone XR}},
  howpublished = {\url{https://www.apple.com/newsroom/2018/09/apple-introduces-iphone-xr/}},
   year={2018}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@book{Pintelonbook,
  title={System identification: a frequency domain approach},
  author={Pintelon, Rik and Schoukens, Johan},
  year={2012},
  publisher={John Wiley \& Sons}
}

@article{LeeU,
  title={U-statistics: Theory and Practice},
  author={Lee, Justin},
  year={1990},
  publisher={CRC Press}
}

@book{Rozanov,
  title={Probability theory: a concise course},
  author={Rozanov, IU},
  year={1977},
  publisher={Courier Dover Publications}
}

@book{Friedland,
  title={Control system design: an introduction to state-space methods},
  author={Friedland, Bernard},
  year={2012},
  publisher={Courier Dover Publications}
}

@book{SchererRobustBook,
  title={Theory of robust control},
  author={Scherer, C.},
  publisher={Delft University of Technology},
  year={2001}  
}

@book{ProakisBook,
  title={Digital signal processing: principles algorithms and applications},
  author={Proakis, J. G.},
  year={2001},
  publisher={Pearson Education India}
}

@book{CarlinBook,
  title={Bayes and empirical Bayes methods for data analysis},
  author={Carlin, B. P. and Louis, T. A.},
  year={2010},
  publisher={Chapman and Hall/CRC}
}

@book{Beck,
  title={Parameter estimation in engineering and science},
  author={Beck, James Vere and Arnold, Kenneth J},
  year={1977},
  publisher={John Wiley \& Sons Inc}
}

@book{RughBook,
  title={Linear system theory},
  author={Rugh, W. J.},
  volume={2},
  year={1996},
  publisher={prentice hall Upper Saddle River, NJ}
}

@book{GriffithsBook,
  title={Introduction to electrodynamics},
  author={Griffiths, D. J.},
  year={1999},
  publisher={Prentice Hall}
}

@book{NealBook,
  title={Bayesian learning for neural networks},
  author={Neal, R.M.},
  volume={118},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@book{Rasmussen,
 author = {Rasmussen, C. E. and Williams, C. K. I.},
 title = {Gaussian Processes for Machine Learning (Adaptive Computation and Machine Learning)},
 year = {2005},
 publisher = {MIT Press}
} 

   @BOOK{VerhaegenBook,
   author = "Verhaegen, M. and Verdult, V.",
   title= "Filtering and System Identification. A Least Squares Approach",
   publisher = "Cambridge University Press",
   year = 2011 }

   @BOOK{Katayama,
   author = "Tohru Katayama",
   title= "Subspace Methods for System Identification",
   publisher = "Springer",
   year = 2005 }
   
      @BOOK{VanOverscheeMoorBook,
   author = "van Overschee, P. and de Moor, B.",
   title= "Subspace Identification for Linear Systems",
   publisher = "Kluwer Academic Publishers",
   year = 1996 }
 
 @book{LjungMatlab,
    author = {Ljung, L.},
    citeulike-article-id = {3853201},
    keywords = {phd},
    posted-at = {2009-01-06 11:06:00},
    priority = {4},
    publisher = {The MathWorks, Inc.},
    title = {System Identification Toolbox for Use with {MATLAB}},
    year = {2007}
}

@article{Scherer-lmi-book,
  title={Linear matrix inequalities in control},
  author={Scherer, C. and Weiland, S.},
  journal={Lecture Notes, Dutch Institute for Systems and Control, Delft, The Netherlands},
  volume={3},
  number={2},
  year={2000}
}
  
  
  @book{DekkingBook,
  title={A Modern Introduction to Probability and Statistics: Understanding why and how},
  author={Dekking, F. M. and Kraaikamp, C. and Lopuha{\"a}, H. P. and Meester, L. E.},
  year={2005},
  publisher={Springer Science \& Business Media}
}


  @book{LjungBook,
  title={System identification - Theory for the User},
  author={Ljung, L.},
  year={1999},
  publisher={Prentice-Hall}
}

  @book{Golub,
  title={Matrix Computations, Fourth Edition},
  author={G.H. Golub and C.F. van Loan},
  year={2013},
  publisher={The Johns Hopkins University Press}
}
@book{Boyd,
  title={Convex optimization},
  author={Boyd, Stephen P and Vandenberghe, Lieven},
  year={2004},
  publisher={Cambridge university press}
}

@book{AstromBook,
 author = {{\AA}str\"{o}m, K. J. and Wittenmark, B.},
 title = {Computer-controlled Systems (3rd Ed.)},
 year = {1997},
 isbn = {0-13-314899-8},
 publisher = {Prentice-Hall, Inc.},
 address = {Upper Saddle River, NJ, USA},
}


@book{AndersonBook,
  title={Optimal filtering},
  author={Anderson, B. D. O. and Moore, J. B.},
  year={2012},
  publisher={Courier Dover Publications}
}

@book{VanDenHof,
  title={Course SC4110: System Identification},
  author={van den Hof, P. M. J.},
  year={2006},
  publisher={Delft University of Technology}
}

@book{Papoulis,
  title={Probability, random variables, and stochastic processes},
  author={Papoulis, Athanasios and Pillai, S Unnikrishna},
  year={2002},
  publisher={Tata McGraw-Hill Education}
}

@book{Tothbook,
  title={Modeling and identification of linear parameter-varying systems},
  author={T{\'o}th, R.},
  volume={403},
  year={2010},
  publisher={Springer}
}

@book{Furlani,
  title={Permanent magnet and electromechanical devices: materials, analysis, and applications},
  author={Furlani, E. P.},
  year={2001},
  publisher={Academic Press}
}

@book{Skogestad,
  title={Multivariable feedback control: analysis and design},
  author={Skogestad, Sigurd and Postlethwaite, Ian},
  volume={2},
  year={2007},
  publisher={Wiley New York}
}


@book{Craig,
  title={Introduction to robotics: mechanics and control},
  author={Craig, J. J.},
  volume={3},
  year={2005},
  publisher={Pearson Prentice Hall Upper Saddle River}
}

@book{Murray-book,
  title={A mathematical introduction to robotic manipulation},
  author={Murray, R. M. and Li, Z. and Sastry, S. S.},
  year={1994},
  publisher={CRC press}
}

@book{YoungBook,
  title={An introduction to Hilbert space},
  author={Young, N.},
  year={1988},
  publisher={Cambridge university press}
}


@book{Spong,
  title={Robot modeling and control},
  author={Spong, M. W. and Hutchinson, S. and Vidyasagar, M.},
  volume={3},
  year={2006},
  publisher={Wiley New York}
}

@book{Harrison,
  title={Advanced engineering dynamics},
  author={Harrison, H.R.N.T. and Nettleton, T.},
  year={1997},
  publisher={Butterworth-Heinemann}
}

@book{Gawronski,
  title={Advanced structural dynamics and active control of structures},
  author={Gawronski, W.},
  year={2004},
  publisher={Springer Science \& Business Media}
}


@book{Rao-book,
  title={Mechanical vibrations},
  author={Rao, S. S. and Yap, F. F.},
  volume={4},
  year={1995},
  publisher={Addison-Wesley New York}
}

@book{Franklin,
  title={Feedback control of dynamic systems},
  author={Franklin, Gene F and Powell, J David and Emami-Naeini, Abbas and Powell, J David},
  volume={2},
  year={1994},
  publisher={Addison-Wesley Reading}
}

@book{Hutton-book,
  title={Fundamentals of finite element analysis},
  author={Hutton, David},
  year={2004},
  publisher={McGraw-Hill,}
}

@book{Zienkiewicz-book,
  title={The finite element method: its basis and fundamentals},
  author={Zienkiewicz, O. C. and Taylor, R. L. and Zhu, J. Z.},
  year={2005},
  publisher={Elsevier}
}

@book{Preumont,
  title={Vibration control of active structures},
  author={Preumont, Andr{\'e}},
  volume={2},
  year={1997},
  publisher={Springer}
}


@book{CraigBook,
  title={Fundamentals of structural dynamics},
  author={Craig, R. R. and Kurdila, A. J.},
  year={2006},
  publisher={John Wiley \& Sons}
}

@book{ZhouBook,
 author = {Zhou, K. and Doyle, J. C. and Glover, K.},
 title = {Robust and Optimal Control},
 year = {1996},
 isbn = {0-13-456567-3},
 publisher = {Prentice-Hall, Inc.},
 address = {Upper Saddle River, NJ, USA}
} 

@book{OppenheimBook,
 author = {Oppenheim, A. V. and Schafer, R. W. and Buck, J. R.},
 title = {Discrete-time Signal Processing (2Nd Ed.)},
 year = {1999},
 isbn = {0-13-754920-2},
 publisher = {Prentice-Hall, Inc.},
 address = {Upper Saddle River, NJ, USA}
} 

@book{MackBook,
  title={Field guide to optical lithography},
  author={Mack, C. A.},
  volume={6},
  year={2006},
  publisher={SPIE Press Bellingham, WA}
}

@book{LojekBook,
  title={History of semiconductor engineering},
  author={Lojek, B.},
  year={2007},
  publisher={Springer}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%		Patents			%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@misc{PatentTrumper1,
  title={Magnetic arrays},
  author={Trumper, D.L. and Kim, W. and Williams, M.E.},
  year={1997},
  month=may # "~20",
  note={US Patent 5,631,618}
}

@misc{PatentFrissen,
  title={Contactless lifting of an object by an inverted planar motor},
  author= {Frissen, P.C.M. and Compter, J.C.},
 year={2009},
 note={WO Patent 2,009,083,889}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%		Techincal report			%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@techreport{TRVerkerk,
  title={NAPAS dSpace Sensor Acquisition (technical report)},
     author = {Verkerk, Koen},
     group = {Control Systems},
     year = {2016},
     institution = {Eindhoven University of Technology},
}

@techreport{TRVerkerk1,
  title={NAPAS dSpace Control (technical report)},
     author = {Verkerk, Koen},
     group = {Control Systems},
     year = {2016},
     institution = {Eindhoven University of Technology},
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%		THESES				%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% THESES and PHD PROJECTS
 	@mastersthesis{Koster,
 	author = "S.E. Koster",
 	title = "Development of a novel subspace identification method: a backward-time approach",
 	school = "Delft University of Technology",
 	year = 2013 }
 	
 		@mastersthesis{Felici,
 	author = "Federico Felici",
 	title = "Subspace Identification of {LPV} systems: A novel approach",
 	school = "Delft University of Technology",
 	year = 2005 }
 
 
 @book{Verdult-phd,
  title={Non linear system identification: a state-space approach},
  author={Verdult, Vincent},
  year={2002},
  publisher={Twente University Press}
}	

@phdthesis{JW-phd,
  title={Control of wind turbines with 'Smart' rotors: proof of concept \& {LPV} subspace identification},
  author={van Wingerden, Jan-Willem},
  school={Delft University of Technology},
  year={2008}
}

@phdthesis{Rovers-phd,
  title={Multiphysical modeling of high-precision electromechanical devices},
  author={Rovers, J. M. M.},
    school={Eindhoven University of Technology},
  year={2013}
}

@phdthesis{Jansen-phd,
  title={Magnetically levitated planar actuator with moving magnets: Electromechanical analysis and design {I}},
  author={Jansen, J. W.},
  school={Eindhoven University of Technology},
  year={2007}
}

@phdthesis{Lierop-phd,
  title={Magnetically levitated planar actuator with moving magnets: Electromechanical analysis and design II},
  author={van Lierop, C. M. M.},
  school={Eindhoven University of Technology},
  year={2007}
}

@phdthesis{Dorosti-phd,
  title={Reduced-order Model Updating for Prediction of Performance Variables in Mechanical Structures},
  author={Dorosti, M.},
  school={Eindhoven University of Technology},
  year={2017}
}

@phdthesis{Cox-phd,
  title={Towards efficient identification of linear parameter-varying state-space models},
  author={Cox, Pepijn B},
  year={2018},
  publisher = "Technische Universiteit Eindhoven",
 school= {Eindhoven University of Technology},
}

@phdthesis{Darwish-phd,
title = "Bayesian identification of linear dynamic systems: synthesis of kernels in the LTI case and beyond",
author = "M.A.H. Darwish",
year = "2017",
month = "10",
day = "10",
language = "English",
isbn = "978-90-386-4352-6",
 school= {Eindhoven University of Technology}
}


@phdthesis{Custers-phd,
title = "Overactuated magnetically levitated systems: flexible modes and eddy current phenomena in high-precision bearingless planar motors",
author = "Custers, C.",
year = "2019",
day = "24",
language = "English",
isbn = "978-90-386-4800-2",
publisher = "Technische Universiteit Eindhoven",
 school= {Eindhoven University of Technology}
}

@phdthesis{Verkerk-phd,
title = "Improved accuracy of flexible systems by state estimation : applied to high-precision motion systems",
author = "K.W. Verkerk",
year = "2018",
month = "1",
day = "17",
language = "English",
isbn = "978-90-386-4411-0",
publisher = "Technische Universiteit Eindhoven",
 school= {Eindhoven University of Technology}
}


@phdthesis{Proimadis-phd,
title = "Nanometer-accurate motion control of moving-magnet planar motors",
author = "Ioannis Proimadis",
year = "2020",
day = "30",
language = "English",
isbn = "978-90-386-5026-5",
publisher = "Technische Universiteit Eindhoven",
school = "Department of Electrical Engineering"
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%		Papers			%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
@inproceedings{3Gebraad,
  title={{LPV} subspace identification using a novel nuclear norm regularization method},
  author={Gebraad, PMO and van Wingerden, JW and van der Veen, GJ and Verhaegen, M},
  booktitle={American Control Conference (ACC), 2011},
  pages={165--170},
  year={2011},
  organization={IEEE}
}

@article{4Sadigh,
  title={Robust Subspace System Identification via Weighted Nuclear Norm Optimization},
  author={Sadigh, Dorsa and Ohlsson, Henrik and Sastry, S Shankar and Seshia, Sanjit A},
  journal={arXiv preprint arXiv:1312.2132},
  year={2013}
}

@article{5Veen,
  title={Global Identification of Wind Turbines Using a Hammerstein Identification Method},
  author={van der Veen, G. and van Wingerden, J. W. and Verhaegen, M.},
  journal={IEEE Transactions on Control Systems Technology},
  number={99},
  pages={1--1},
  year={2012},
  publisher={IEEE}
}

 @article{7Ljung,
  title={Subspace identification from closed loop data},
  author={Ljung, L. and McKelvey, T.},
  journal={Signal Processing},
  volume={52},
  number={2},
  pages={209--215},
  year={1996},
  publisher={Elsevier}
}


@article{9Veen,
  title={Closed-loop subspace identification methods: an overview},
  author={van der Veen, G. and van Wingerden, J. W. and Bergamasco, M. and Lovera, M. and Verhaegen, M.},
  journal={IET Control Theory \& Applications},
  volume={7},
  number={10},
  pages={1339--1358},
  year={2013},
  publisher={IET Digital Library}
}

	
@inproceedings{10Qin,
  title={Parallel {QR} implementation of subspace identification with parsimonious models},
  author={Qin, S.J. and Ljung, L.},
  booktitle={Proceedings of the 13th IFAC SYSID Symposium},
  pages={1631--1636},
  year={2003}
}
 	
@inproceedings{11Qin,
  title={Closed-loop subspace identification with innovation estimation},
  author={Qin, S.J. and Ljung, L.},
  booktitle={Proceedings of the 13th IFAC SYSID Symposium},
  pages={887--892},
  year={2003}
}

@article{12Chiuso,
title = "Consistency analysis of some closed-loop subspace identification methods ",
journal = "Automatica ",
volume = "41",
number = "3",
pages = "377 - 391",
year = "2005",
note = "Data-Based Modelling and System Identification ",
issn = "0005-1098",
doi = "http://dx.doi.org/10.1016/j.automatica.2004.10.015",
author = "Alessandro Chiuso and Giorgio Picci",
keywords = "Subspace identification",
keywords = "Exogenous inputs",
keywords = "Stochastic realization",
keywords = "Statistical analysis",
keywords = "Stochastic state-space identification "
}

 	@article{13Forssell,
title = "Closed-loop identification revisited ",
journal = "Automatica ",
volume = "35",
number = "7",
pages = "1215 - 1241",
year = "1999",
note = "",
issn = "0005-1098",
doi = "http://dx.doi.org/10.1016/S0005-1098(99)00022-9",
author = "Urban Forssell and Lennart Ljung",
keywords = "System identification",
keywords = "Closed-loop identification",
keywords = "Prediction error methods",
keywords = "Modelling",
keywords = "Statistical analysis "
}


@inproceedings{14Lin,
title = "Comparison of subspace identification methods for systems operating on closed-loop ",
  author={Lin, Weilu and Qin, S Joe and Ljung, Lennart},
  booktitle={Proceedings of the 16th IFAC World Congress},
  pages={494--499},
  year={2005}
}


@article{16Qin,
title = "An overview of subspace identification ",
journal = "Computers \& Chemical Engineering ",
volume = "30",
number = "10–12",
pages = "1502 - 1513",
year = "2006",
note = "Papers form Chemical Process Control \{VII\} \{CPC\} \{VII\} Seventh international conference in the Series ",
issn = "0098-1354",
doi = "http://dx.doi.org/10.1016/j.compchemeng.2006.05.045",
author = "S. Joe Qin",
keywords = "Subspace identification",
keywords = "Closed-loop identification",
keywords = "Overview",
keywords = "State space models",
keywords = "Causal model",
keywords = "Practice "
}

@article{17Schon,
  title={System identification of nonlinear state-space models},
  author={Sch{\"o}n, Thomas B and Wills, Adrian and Ninness, Brett},
  journal={Automatica},
  volume={47},
  number={1},
  pages={39--49},
  year={2011},
  publisher={Elsevier}
}

@article{21Ljung,
  title={Approaches to identification of nonlinear systems},
  author={Ljung, Lennart},
  year={2010}
}

@article{22Ljung,
  title={Four encounters with system identification},
  author={Ljung, L. and Hjalmarsson, H. and Ohlsson, H.},
  journal={European Journal of Control},
  volume={17},
  number={5},
  pages={449--471},
  year={2011},
  publisher={Elsevier}
}

@inproceedings{27Kantas,
  title={An overview of sequential Monte Carlo methods for parameter estimation in general state-space models},
  author={Kantas, Nicholas and Doucet, Arnaud and Singh, Sumeetpal Sindhu and Maciejowski, Jan Marian},
  booktitle={15th IFAC Symposium on System Identification (SYSID), Saint-Malo, France.(invited paper)},
  volume={102},
  pages={117},
  year={2009}
}

 	@article{28VanOverschee,
title = "N4SID: Subspace algorithms for the identification of combined deterministic-stochastic systems ",
journal = "Automatica ",
volume = "30",
number = "1",
pages = "75 - 93",
year = "1994",
note = "Special issue on statistical signal processing and control ",
issn = "0005-1098",
doi = "http://dx.doi.org/10.1016/0005-1098(94)90230-5",
url = "http://www.sciencedirect.com/science/article/pii/0005109894902305",
author = "van Overschee, P. and de Moor, B.",
keywords = "System identification",
keywords = "Kalman filters",
keywords = "difference equations",
keywords = "\{QR\} and singular value decomposition",
keywords = "multivariable systems",
keywords = "state space methods "
}

@article{29VanOverschee,
title = "A unifying theorem for three subspace system identification algorithms ",
journal = "Automatica ",
volume = "31",
number = "12",
pages = "1853 - 1864",
year = "1995",
note = "Trends in System Identification ",
issn = "0005-1098",
doi = "http://dx.doi.org/10.1016/0005-1098(95)00072-0",
url = "http://www.sciencedirect.com/science/article/pii/0005109895000720",
author = "Peter van Overschee and Bart de Moor",
keywords = "System identification",
keywords = "subspace methods",
keywords = "multivariable systems",
keywords = "state-space methods",
keywords = "linear algebra",
keywords = "Kalman filters",
keywords = "difference equations",
keywords = "stochastic systems "
}


@INPROCEEDINGS{30Larimore, 
author={Larimore, W.E.}, 
booktitle={Decision and Control, 1990., Proceedings of the 29th IEEE Conference on}, 
title={Canonical variate analysis in identification, filtering, and adaptive control}, 
year={1990}, 
month={Dec}, 
pages={596-604 vol.2}, 
keywords={Markov processes;adaptive control;filtering and prediction theory;identification;statistical analysis;abruptly changing systems;adaptive control;canonical variate analysis;filtering;identification;nonlinear systems;optimal Akaike information criterion procedure;past/future Markov property;reduced-order prediction problem;singular value decomposition;state order selection;state-space model estimation;time-varying systems;Adaptive control;Adaptive filters;Filtering;Predictive control;Predictive models;Singular value decomposition;State estimation;Stochastic processes;System identification;Time varying systems}, 
doi={10.1109/CDC.1990.203665},}

@article{31Verhaegen,
title = "Identification of the deterministic part of {MIMO} state space models given in innovations form from input-output data ",
journal = "Automatica ",
volume = "30",
number = "1",
pages = "61 - 74",
year = "1994",
note = "Special issue on statistical signal processing and control ",
issn = "0005-1098",
doi = "http://dx.doi.org/10.1016/0005-1098(94)90229-1",
author = "Michel Verhaegen",
keywords = "State space",
keywords = "system identification",
keywords = "linear systems",
keywords = "linear algebra "
}

@article{32McKelvey,
  title={Frequency Domain System Identification with IV Based Subspace Algorithm},
  author={McKelvey, Tomas},
  year={1995},
  publisher={Citeseer}
}

@inproceedings{38Veen,
  title={Closed-loop MOESP subspace model identification with parametrisable disturbances},
  author={van der Veen, Gijs and van Wingerden, J and Verhaegen, Michel},
  booktitle={Decision and Control (CDC), 2010 49th IEEE Conference on},
  pages={2813--2818},
  year={2010},
  organization={IEEE}
}

@inproceedings{39Ruscio,
  title={Subspace system identification of the Kalman filter: open and closed loop systems},
  author={Di Ruscio, David},
  booktitle={Proc. Intl. Multi-Conf. on Engineering and Technological Innovation},
  year={2008}
}

@article{40Ruscio,
  title={{Closed and Open Loop Subspace System Identification of the Kalman Filter}},
  author={Di Ruscio, David},
  journal={Modeling, Identification and Control},
  volume={30},
  number={2},
  pages={71--86},
  year={2009},
  doi={10.4173/mic.2009.2.3},
  publisher={Norwegian Society of Automatic Control}
}

@article{41Chiuso,
  title={The role of vector autoregressive modeling in predictor-based subspace identification},
  author={Chiuso, Alessandro},
  journal={Automatica},
  volume={43},
  number={6},
  pages={1034--1048},
  year={2007},
  publisher={Elsevier}
}

@article{42Verdult,
  title={Subspace identification of multivariable linear parameter-varying systems},
  author={Verdult, V. and Verhaegen, M.},
  journal={Automatica},
  volume={38},
  number={5},
  pages={805--814},
  year={2002},
  publisher={Elsevier}
}

@article{43Felici,
  title={Subspace identification of MIMO LPV systems using a periodic scheduling sequence},
  author={Felici, F. and van Wingerden, J. W. and Verhaegen, M.},
  journal={Automatica},
  volume={43},
  number={10},
  pages={1684--1697},
  year={2007},
  publisher={Elsevier}
}

@article{44Wingerden,
  title={Subspace identification of bilinear and {LPV} systems for open-and closed-loop data},
  author={van Wingerden, J. W. and Verhaegen, M.},
  journal={Automatica},
  volume={45},
  number={2},
  pages={372--381},
  year={2009},
  publisher={Elsevier}
}

@INPROCEEDINGS{45Lee, 
author={Lee, L.H. and Poolla, K.}, 
booktitle={Decision and Control, 1996., Proceedings of the 35th IEEE Conference on}, 
title={Identification of linear parameter-varying systems via LFTs}, 
year={1996}, 
month={Dec}, 
volume={2}, 
pages={1545-1550 vol.2}, 
keywords={Hessian matrices;minimisation;nonlinear programming;parameter estimation;Hessian-based nonlinear optimization algorithms;LFT;LPV;cost function minimization;gradient-based nonlinear optimization algorithms;identifiability;identification;initialization;linear parameter-varying systems;linear-fractional parameter dependence;prediction error method;1f noise;Aircraft;Cost function;Linear systems;Mechanical engineering;Missiles;Noise measurement;Noise reduction;Parameter estimation;Time varying systems}, 
doi={10.1109/CDC.1996.572742}, 
ISSN={0191-2216},}

@article{46Verdult,
title = "Kernel methods for subspace identification of multivariable \{LPV\} and bilinear systems ",
journal = "Automatica ",
volume = "41",
number = "9",
pages = "1557 - 1565",
year = "2005",
note = "",
issn = "0005-1098",
doi = "http://dx.doi.org/10.1016/j.automatica.2005.03.027",
author = "Verdult, V. and Verhaegen, M.",
keywords = "System identification",
keywords = "Subspace methods",
keywords = "State-space methods",
keywords = "Linear parameter-varying systems",
keywords = "Bilinear systems "
}

@inproceedings{47Verdult,
  title={Identification of fully parameterized linear and nonlinear state-space systems by projected gradient search},
  author={Verdult, Vincent and Bergboer, Niek and Verhaegen, Michel},
  booktitle={Proceedings of the 13th IFAC Symposium on System Identification, The Netherlands},
  year={2003}
}

@inproceedings{48Verdult,
  title={Least squares support vector machines for kernel CCA in nonlinear state-space identification},
  author={Verdult, Vincent and Suykens, Johan AK and Boets, Jeroen and Goethals, Ivan and de Moor, Bart},
  booktitle={Proceedings of the 16th international symposium on Mathematical Theory of Networks and Systems (MTNS2004), Leuven, Belgium},
  year={2004}
}

@inproceedings{49Wingerden,
  title={Subspace identification of {MIMO} LPV systems: The PBSID approach},
  author={van Wingerden, J. W. and Verhaegen, M.},
  booktitle={Decision and Control, 2008. CDC 2008. 47th IEEE Conference on},
  pages={4516--4521},
  year={2008},
  organization={IEEE}
}

@inproceedings{50Wingerden,
  title={Subspace identification of multivariable LPV systems: a novel approach},
  author={van Wingerden, J. W. and Verhaegen, M.},
  booktitle={Computer-Aided Control Systems, 2008. CACSD 2008. IEEE International Conference on},
  pages={840--845},
  year={2008},
  organization={IEEE}
}

@inproceedings{52Wingerden,
  title={Subspace identification of bilinear systems using a dedicated input sequence},
  author={van Wingerden, J. W. and Verhaegen, M.},
  booktitle={Decision and Control, 2007 46th IEEE Conference on},
  pages={4962--4967},
  year={2007},
  organization={IEEE}
}

@inproceedings{53Rajaoarisoa,
  title={Subspace technique for identification of hybrid complex systems.},
  author={Rajaoarisoa, Lala H and M'sirdi, Nacer K and Boukas, E-K and Naamane, Aziz},
  booktitle={Control and Automation, 2008 16th Mediterranean Conference on},
  pages={89--94},
  year={2008},
  organization={IEEE}
}

@inproceedings{54Wingerden,
  title={The asymptotic variance of the PBSIDopt algorithm},
  author={van Wingerden, Jan-Willem},
  booktitle={System Identification},
  volume={16},
  number={1},
  pages={1167--1172},
  year={2012}
}

@inproceedings{55Lygeros,
  title={Lecture notes on hybrid systems},
  author={Lygeros, J.},
  booktitle={Notes for an ENSIETA workshop},
  year={2004}
}

@article{56Paoletti,
  title={Identification of Hybrid Systems A Tutorial},
  author={Paoletti, Simone and Juloski, Aleksandar Lj and Ferrari-Trecate, Giancarlo and Vidal, Ren{\'e}},
  journal={European journal of control},
  volume={13},
  number={2},
  pages={242--260},
  year={2007},
  publisher={Elsevier}
}

@inproceedings{57Verdult,
  title={Subspace identification of piecewise linear systems},
  author={Verdult, V. and Verhaegen, M.},
  booktitle={Decision and Control, 2004. CDC. 43rd IEEE Conference on},
  volume={4},
  pages={3838--3843},
  year={2004},
  organization={IEEE}
}

@inproceedings{58Borges,
  title={Iterative subspace identificatino of piecewise linear systems},
  author={Borges, J. and Verdult, V. and Verhaegen, M.},
  booktitle={Proceedings of the 14th IFAC SYSID Symposium},
  pages={368--373},
  year={2006}
}

@incollection{59Juloski,
  title={Comparison of four procedures for the identification of hybrid systems},
  author={Juloski, Aleksandar Lj and Heemels, WPMH and Ferrari-Trecate, Giancarlo and Vidal, Ren{\'e} and Paoletti, Simone and Niessen, JHG},
  booktitle={Hybrid systems: computation and control},
  pages={354--369},
  year={2005},
  publisher={Springer}
}

@inproceedings{60Borges,
  title={A switching detection method based on projected subspace classification},
  author={Borges, J. and Verdult, V. and Verhaegen, M. and Botto, M. A.},
  booktitle={Decision and Control, 2005 and 2005 European Control Conference. CDC-ECC'05. 44th IEEE Conference on},
  pages={344--349},
  year={2005},
  organization={IEEE}
}

@article{61Verhaegen,
  title={Subspace model identification part 3. Analysis of the ordinary output-error state-space model identification algorithm},
  author={Verhaegen, M.},
  journal={International Journal of control},
  volume={58},
  number={3},
  pages={555--586},
  year={1993},
  publisher={Taylor \& Francis}
}

@INPROCEEDINGS{62Lopes, 
author={Vilela Lopes, R. and Araujo Borges, G. and Yoshiyuki Ishihara, J.}, 
booktitle={American Control Conference (ACC), 2013}, 
title={New algorithm for identification of discrete-time switched linear systems}, 
year={2013}, 
month={June}, 
pages={6219-6224}, 
keywords={MIMO systems;discrete time systems;identification;linear systems;matrix algebra;pattern classification;pattern clustering;state-space methods;time-varying systems;data classification;data clustering;discrete-time switched linear MIMO state space system identification;numerical simulation;submodel matrix representation;subspace identification techniques;Clustering algorithms;Data models;Heuristic algorithms;Markov processes;Robustness;Switches;Vectors}, 
ISSN={0743-1619},}

@INPROCEEDINGS{63Huang, 
author={Kun Huang and Wagner, A. and Yi Ma}, 
booktitle={Decision and Control, 2004. CDC. 43rd IEEE Conference on}, 
title={Identification of hybrid linear time-invariant systems via subspace embedding and segmentation (SES)}, 
year={2004}, 
month={Dec}, 
volume={3}, 
pages={3227-3234 Vol.3}, 
keywords={linear systems;observability;principal component analysis;state-space methods;time-varying systems;generalized principal component analysis;hybrid linear time-invariant systems;state-space models;subspace embedding;subspace segmentation;Biomedical informatics;Bismuth;Filtering;Linear systems;Noise robustness;Principal component analysis;System identification;Upper bound}, 
doi={10.1109/CDC.2004.1428971}, 
ISSN={0191-2216},}

@article{64Vidal,
  title={Generalized principal component analysis (GPCA)},
  author={Vidal, Rene and Ma, Yi and Sastry, Shankar},
  journal={Pattern Analysis and Machine Intelligence, IEEE Transactions on},
  volume={27},
  number={12},
  pages={1945--1959},
  year={2005},
  publisher={IEEE}
}


@INPROCEEDINGS{65Pekpe, 
author={Pekpe, K.M. and Mourot, G. and Gasso, K. and Ragot, J.}, 
booktitle={Decision and Control, 2004. CDC. 43rd IEEE Conference on}, 
title={Identification of switching systems using change detection technique in the subspace framework}, 
year={2004}, 
month={Dec}, 
volume={4}, 
pages={3720-3725 Vol.4}, 
keywords={Markov processes;parameter estimation;time-varying systems;Markov parameters;abrupt model changes;change detection technique;identification technique;local models;subspace framework;subspace method;switching systems;Control system analysis;Convergence;Delay estimation;Merging;Nonlinear control systems;Nonlinear systems;Parameter estimation;State-space methods;Switching systems;Testing}, 
doi={10.1109/CDC.2004.1429317}, 
ISSN={0191-2216},}


@inproceedings{66Bako,
  title={Identification of MIMO switched state-space models},
  author={Bako, Laurent and Le, van Luong and Lauer, Fabien and Bloch, Gerard},
  booktitle={American Control Conference (ACC), 2013},
  pages={71--76},
  year={2013},
  organization={IEEE}
}


@incollection{67Wingerden,
  title={Subspace Identification of Hammerstein--Wiener Systems Operating in Closed-loop},
  author={van Wingerden, J.W. and Verhaegen, M.},
  booktitle={Block-oriented Nonlinear System Identification},
  pages={229--239},
  year={2010},
  publisher={Springer}
}

@inproceedings{68Wingerden,
  title={Closed-loop subspace identification of Hammerstein-Wiener models},
  author={van Wingerden, J. W. and Verhaegen, M.},
  booktitle={Decision and Control, 2009 held jointly with the 2009 28th Chinese Control Conference. CDC/CCC 2009. Proceedings of the 48th IEEE Conference on},
  pages={3637--3642},
  year={2009},
  organization={IEEE}
}

@inproceedings{69Wingerden,
  title={Closed loop identification of MIMO Hammerstein models using LS-SVM},
  author={van Wingerden, J. W. and Verhaegen, M.},
  booktitle={System Identification},
  volume={15},
  number={1},
  pages={1650--1655},
  year={2009}
}

@article{70Goethals,
  title={Identification of MIMO Hammerstein models using least squares support vector machines},
  author={Goethals, Ivan and Pelckmans, Kristiaan and Suykens, Johan AK and de Moor, Bart},
  journal={Automatica},
  volume={41},
  number={7},
  pages={1263--1272},
  year={2005},
  publisher={Elsevier}
}

@article{71Goethals,
  title={Subspace identification of Hammerstein systems using least squares support vector machines},
  author={Goethals, Ivan and Pelckmans, Kristiaan and Suykens, Johan AK and de Moor, Bart},
  journal={Automatic Control, IEEE Transactions on},
  volume={50},
  number={10},
  pages={1509--1519},
  year={2005},
  publisher={IEEE}
}

@inproceedings{72Verdult,
  title={A kernel method for subspace identification of multivariable bilinear systems},
  author={Verdult, V. and Verhaegen, M.},
  booktitle={Decision and Control, 2003. Proceedings. 42nd IEEE Conference on},
  volume={4},
  pages={3972--3977},
  year={2003},
  organization={IEEE}
}

@article{73Suykens,
  title={Least squares support vector machine classifiers},
  author={Suykens, Johan AK and Vandewalle, Joos},
  journal={Neural processing letters},
  volume={9},
  number={3},
  pages={293--300},
  year={1999},
  publisher={Springer}
}

@inproceedings{74Goethals,
  title={Subspace intersection identification of Hammerstein-Wiener systems},
  author={Goethals, Ivan and Pelckmans, Kristiaan and Hoegaerts, Luc and Suykens, JAK and de Moor, BLR},
  booktitle={IEEE CONFERENCE ON DECISION AND CONTROL},
  volume={44},
  number={7},
  pages={7108},
  year={2005},
  organization={IEEE; 1998}
}

@article{75Visser,
title = "A new approach to linear regression with multivariate splines ",
journal = "Automatica ",
volume = "45",
number = "12",
pages = "2903 - 2909",
year = "2009",
note = "",
issn = "0005-1098",
doi = "http://dx.doi.org/10.1016/j.automatica.2009.09.017",
author = "C.C. de Visser and Q.P. Chu and J.A. Mulder",
keywords = "Splines",
keywords = "Parameter estimation",
keywords = "Scattered data",
keywords = "Function approximation",
keywords = "Estimators "
}

@article{76Moonen,
  title={On-and off-line identification of linear state-space models},
  author={Moonen, M. and de Moor, B. and Vandenberghe, L. and Vandewalle, J.},
  journal={International Journal of Control},
  volume={49},
  number={1},
  pages={219--232},
  year={1989},
  publisher={Taylor \& Francis}
}


@inproceedings{78Ljung,
  title={What Can Regularization Offer for Estimation of Dynamical Systems?},
  author={Ljung, L. and Chen, T.},
  booktitle={Adaptation and Learning in Control and Signal Processing},
  volume={11},
  number={1},
  pages={1--8},
  year={2013}
}

@article{79Chen,
  title= {{On the estimation of transfer functions, regularizations and Gaussian processes - Revisited}},
  author={Chen, T. and Ohlsson, H. and Ljung, L.},
  journal={Automatica},
  volume={48},
  number={8},
  pages={1525--1535},
  year={2012},
  publisher={Elsevier}
}

@article{80Schon,
  title={An explanation of the expectation maximization algorithm},
  author={Sch{\"o}n, Thomas},
  year={2009}
}

@article{82Ljung,
  title={Perspectives on system identification},
  author={Ljung, L.},
  journal={Annual Reviews in Control},
  volume={34},
  number={1},
  pages={1--12},
  year={2010},
  publisher={Elsevier}
}

@article{83Astrom,
  title={Maximum likelihood and prediction error methods},
  author={{\AA}str{\"o}m, Karl Johan},
  journal={Automatica},
  volume={16},
  number={5},
  pages={551--574},
  year={1980},
  publisher={Elsevier}
}

@article{84Gibson,
  title={Robust maximum-likelihood estimation of multivariable dynamic systems},
  author={Gibson, Stuart and Ninness, Brett},
  journal={Automatica},
  volume={41},
  number={10},
  pages={1667--1682},
  year={2005},
  publisher={Elsevier}
}

@article{85Gibson,
  title={Maximum-likelihood parameter estimation of bilinear systems},
  author={Gibson, Stuart and Wills, Adrian and Ninness, Brett},
  journal={Automatic Control, IEEE Transactions on},
  volume={50},
  number={10},
  pages={1581--1596},
  year={2005},
  publisher={IEEE}
}

@inproceedings{86Deisenroth,
 author = {Deisenroth, Marc Peter and Huber, Marco F. and Hanebeck, Uwe D.},
 title = {Analytic Moment-based Gaussian Process Filtering},
 booktitle = {Proceedings of the 26th Annual International Conference on Machine Learning},
 series = {ICML '09},
 year = {2009},
 isbn = {978-1-60558-516-1},
 location = {Montreal, Quebec, Canada},
 pages = {225--232},
 numpages = {8},
 doi = {10.1145/1553374.1553403},
 acmid = {1553403},
 publisher = {ACM},
 address = {New York, NY, USA}
} 

@inproceedings{87Turner,
  title={State-space inference and learning with Gaussian processes},
  author={Turner, Ryan D and Deisenroth, Marc P and Rasmussen, Carl E},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={868--875},
  year={2010}
}

@article{88Pillonetto,
title = "Kernel methods in system identification, machine learning and function estimation: A survey ",
journal = "Automatica ",
volume = "50",
number = "3",
pages = "657 - 682",
year = "2014",
note = "",
issn = "0005-1098",
doi = "http://dx.doi.org/10.1016/j.automatica.2014.01.001",
author = "Pillonetto, G. and Dinuzzo, F. and Chen, T. and de Nicolao, G. and Ljung, L.",
keywords = "Linear system identification",
keywords = "Prediction error methods",
keywords = "Model complexity selection",
keywords = "Bias-variance trade-off",
keywords = "Kernel-based regularization",
keywords = "Inverse problems",
keywords = "Reproducing kernel Hilbert spaces",
keywords = "Gaussian processes "
}


    @article{89Ljung,
     jstor_articletype = {research-article},
     title = {Asymptotic Properties of the Least-Squares Method for Estimating Transfer Functions and Disturbance Spectra},
     author = {Ljung, L. and Wahlberg, B.},
     journal = {Advances in Applied Probability},
     jstor_issuetitle = {},
     volume = {24},
     number = {2},
     jstor_formatteddate = {Jun., 1992},
     pages = {pp. 412-440},
    ISSN = {00018678},
     abstract = {The problem of estimating the transfer function of a linear system, together with the spectral density of an additive disturbance, is considered. The set of models used consists of linear rational transfer functions and the spectral densities are estimated from a finite-order autoregressive disturbance description. The true system and disturbance spectrum are, however, not necessarily of finite order. We investigate the properties of the estimates obtained as the number of observations tends to ∞ at the same time as the model order employed tends to ∞ . It is shown that the estimates are strongly consistent and asymptotically normal, and an expression for the asymptotic variances is also given. The variance of the transfer function estimate at a certain frequency is related to the signal/noise ratio at that frequency and the model orders used, as well as the number of observations. The variance of the noise spectral estimate relates in a similar way to the squared value of the true spectrum.},
     language = {English},
     year = {1992},
     publisher = {Applied Probability Trust},
     copyright = {Copyright © 1992 Applied Probability Trust},
    }
    
@article{90Rivals,
  title={Black-box modeling with state-space neural networks},
  author={Rivals, Isabelle and Personnaz, L{\'e}on},
  journal={Neural Adaptive Control Technology},
  volume={15},
  pages={237},
  year={1996},
  publisher={World Scientific}
}    

@article{91Akaike,
  title={Stochastic theory of minimal realization},
  author={Akaike, Hirotugu},
  journal={Automatic Control, IEEE Transactions on},
  volume={19},
  number={6},
  pages={667--674},
  year={1974},
  publisher={IEEE}
}

@inproceedings{92Pillonetto,
  title={Predictor estimation via Gaussian regression},
  author={Pillonetto, G. and Chiuso, A. and de Nicolao, G.},
  booktitle={Decision and Control, 2008. CDC 2008. 47th IEEE Conference on},
  pages={744--749},
  year={2008},
  organization={IEEE},
  month = {}
}

@article{93Pillonetto,
  title={A new kernel-based approach for linear system identification},
  author={Pillonetto, G. and de Nicolao, G.},
  journal={Automatica},
  volume={46},
  number={1},
  pages={81--93},
  year={2010},
  publisher={Elsevier}
}

@INPROCEEDINGS{94Chiuso,
author={Chiuso, A. and Pillonetto, G. and de Nicolao, G.}, 
booktitle={Decision and Control, 2008. CDC 2008. 47th IEEE Conference on}, 
title={Subspace identification using predictor estimation via Gaussian regression}, 
year={2008}, 
month={Dec}, 
pages={3299-3304}, 
}


@article{96Pillonetto,
  title={Prediction error identification of linear systems: a nonparametric Gaussian regression approach},
  author={Pillonetto, G. and Chiuso, A. and de Nicolao, G.},
  journal={Automatica},
  volume={47},
  number={2},
  pages={291--305},
  year={2011},
  publisher={Elsevier}
}

@article{97Markovsky,
  title={Overview of total least-squares methods},
  author={Markovsky, Ivan and van Huffel, Sabine},
  journal={Signal processing},
  volume={87},
  number={10},
  pages={2283--2302},
  year={2007},
  publisher={Elsevier}
}

@article{98Ibragimov,
  title={Some limit theorems for stationary processes},
  author={Ibragimov, Ildar A},
  journal={Theory of Probability \& Its Applications},
  volume={7},
  number={4},
  pages={349--382},
  year={1962},
  publisher={SIAM}
}

@article{99Withers,
  title={Central limit theorems for dependent variables. I},
  author={Withers, Christopher Stroude},
  journal={Zeitschrift f{\"u}r Wahrscheinlichkeitstheorie und verwandte Gebiete},
  volume={57},
  number={4},
  pages={509--534},
  year={1981},
  publisher={Springer}
}

@article{100Paige,
  title={Covariance matrix representation in linear filtering},
  author={Paige, Christopher C},
  journal={Special Issue of Contemporary Mathematics on Linear Algebra and its Role in Systems Theory, AMS},
  year={1985}
}

@inproceedings{101Aravkin,
  title={On the estimation of hyperparameters for empirical bayes estimators: Maximum marginal likelihood vs minimum MSE},
  author={Aravkin, Aleksandr and Burke, James V and Chiuso, Alessandro and Pillonetto, Gianluigi},
  booktitle={16th IFAC Symposium on System Identification},
  volume={16},
  number={1},
  pages={125--130},
  year={2012}
}

@inproceedings{102Carli,
  title={{On the estimation of hyperparameters for Bayesian system identification with exponentially decaying kernels.}},
  author={Carli, R. and Chen, T. and Chiuso, A. and Ljung, L. and Pillonetto, G.},
  booktitle={51st IEEE Conference on Decision and Control},
  pages={5260--5265},
  year={2012}
}

@article{103Houtzager,
  title={Predictor-based subspace identification toolbox version 0.4, 2010},
  author={Houtzager, I and van Wingerden, JW and Verhaegen, M},
  journal={URL http://www. dcsc. tudelft. nl/\~{} datadriven/pbsid}
}

@inproceedings{104Toth,
  title={Discrete time {LPV} {I/O} and state space representations, differences of behavior and pitfalls of interpolation},
  author={T{\'o}th, R. and Felici, F. and Heuberger, P. S. C. and van den Hof, P. M. J.},
  booktitle={Proc. of the European control conf},
  pages={5418--5425},
  year={2007}
}

@article{105Chen,
  title={Implementation of algorithms for tuning parameters in regularized least squares problems in system identification},
  author={Chen, T. and Ljung, L.},
  journal={Automatica},
  volume={49},
  number={7},
  pages={2213--2220},
  year={2013},
  publisher={Elsevier}
}

@inproceedings{106Carli,
  title={Efficient algorithms for large scale linear system identification using stable spline estimators},
  author={Carli, Francesca Paola and Chiuso, Alessandro and Pillonetto, Gianluigi},
  booktitle={System Identification},
  volume={16},
  number={1},
  pages={119--124},
  year={2012}
}

@inproceedings{107Chen,
  title={Rank-1 kernels for regularized system identification},
  author={Chen, Tianshi and Chiuso, Alessandro and Pillonetto, Gianluigi and Ljung, Lennart},
  booktitle={Decision and Control (CDC), 2013 IEEE 52nd Annual Conference on},
  pages={5162--5167},
  year={2013},
  organization={IEEE}
}

@inproceedings{108Pillonetto,
  title={Kernel selection in linear system identification Part I: A Gaussian process perspective},
  author={Pillonetto, G. and de Nicolao, G.},
  booktitle={Decision and Control and European Control Conference (CDC-ECC), 2011 50th IEEE Conference on},
  pages={4318--4325},
  year={2011},
  organization={IEEE}
}

@inproceedings{109Chen,
  title={Kernel selection in linear system identification part II: A classical perspective},
  author={Chen, T. and Ohlsson, H. and Goodwin, G.C. and Ljung, L.},
  booktitle={Decision and Control and European Control Conference (CDC-ECC), 2011 50th IEEE Conference on},
  pages={4326--4331},
  year={2011},
  organization={IEEE}
}

@article{113Pillonetto,
author={G. {Pillonetto} and A. {Aravkin}},
booktitle={2014 IEEE International Workshop on Machine Learning for Signal Processing (MLSP)},
title={A new kernel-based approach for identification of time-varying linear systems},
year={2014},
volume={},
number={},
pages={1-6},
doi={10.1109/MLSP.2014.6958894},
ISSN={1551-2541},
month={Sep.}
}


@article{110Bauer,
  title={Order estimation for subspace methods},
  author={Bauer, Dietmar},
  journal={Automatica},
  volume={37},
  number={10},
  pages={1561--1573},
  year={2001},
  publisher={Elsevier}
}

@ARTICLE{114Chen, 
author={Tianshi Chen and Andersen, M.S. and Ljung, L. and Chiuso, A. and Pillonetto, G.}, 
journal={Automatic Control, IEEE Transactions on}, 
title={System Identification Via Sparse Multiple Kernel-Based Regularization Using Sequential Convex Optimization Techniques}, 
year={2014}, 
month={Nov}, 
volume={59}, 
number={11}, 
pages={2933-2945}, }

@article{115Carli,
  title={Maximum Entropy Kernels for System Identification},
  author={Carli, Francesca Paola and Chen, Tianshi and Ljung, Lennart},
  journal={arXiv preprint arXiv:1411.5620},
  year={2014}
}

@inproceedings{116Golabi,
  title={{A Bayesian Approach for Estimation of Linear-Regression LPV Models}},
  author={Golabi, A. and Meskin, N. and T{\'o}th, R. and Mohammadpour, J.},
  booktitle={Decision and Control (CDC), 2014 53th IEEE Conference on},
  pages={2555-2560},
  year={2014},
  organization={IEEE}
}

@article{118Bachnas,
title = "A review on data-driven linear parameter-varying modeling approaches: A high-purity distillation column case study ",
journal = "Journal of Process Control ",
volume = "24",
number = "4",
pages = "272 - 285",
year = "2014",
note = "",
issn = "0959-1524",
author = "A.A. Bachnas and R. T\'{o}th and J.H.A. Ludlage and A. Mesbah"
}

@article{121Toth,
  title={On the state-space realization of {LPV} input-output models: Practical approaches},
  author={T{\'o}th, R. and Abbas, H.S. and Werner, H.},
  journal={Control Systems Technology, IEEE Transactions on},
  volume={20},
  number={1},
  pages={139--153},
  year={2012},
  publisher={IEEE}
}

@article{122Toth,
  title={The behavioral approach to linear parameter-varying systems},
  author={T{\'o}th, R. and Willems, J. C. and Heuberger, P. S. C. and van den Hof, P. M. J.},
  journal={Automatic Control, IEEE Transactions on},
  volume={56},
  number={11},
  pages={2499--2514},
  year={2011},
  publisher={IEEE}
}\\

@article{123Goodwin,
  title={Quantifying the error in estimated transfer functions with application to model order selection},
  author={Goodwin, G.C. and Gevers, M. and Ninness, B.},
  journal={Automatic Control, IEEE Transactions on},
  volume={37},
  number={7},
  pages={913--928},
  year={1992},
  publisher={IEEE}
}

@inproceedings{124Lovera,
  title={Identification for gain-scheduling: a balanced subspace approach},
  author={Lovera, M. and Merc{\`e}re, G.},
  booktitle={American Control Conference 2007, ACC'07},
  pages={CDROM},
  year={2007}
}

@inproceedings{125Chen,
  title={Constructive state space model induced kernels for regularized system identification⋆},
  author={Chen, Tianshi and Ljung, Lennart},
  booktitle={Proceedings of the 19th IFAC World Congress},
  year={2014}
}

@article{127Dinuzzo,
  title={Kernels for linear time invariant system identification},
  author={Dinuzzo, F.},
  journal={arXiv preprint arXiv:1203.4930},
  year={2012}
}

@article{128Aronszajn,
  title={Theory of reproducing kernels},
  author={Aronszajn, N.},
  journal={Transactions of the American mathematical society},
  pages={337--404},
  year={1950},
  publisher={JSTOR}
}

@inproceedings{129Scholkopf,
  title={A generalized representer theorem},
  author={Sch{\"o}lkopf, B. and Herbrich, R. and Smola, A. J.},
  booktitle={Computational learning theory},
  pages={416--426},
  year={2001},
  organization={Springer}
}


@incollection{132Lovera,
  title={{LPV} modelling and identification: An overview},
  author={Lovera, M. and Bergamasco, M. and Casella, F.},
  booktitle={Robust Control and Linear Parameter Varying Approaches},
  pages={3--24},
  year={2013},
  publisher={Springer}
}

@book{133Verdult,
  title={Non linear system identification: a state-space approach},
  author={Verdult, Vincent},
  year={2002},
  publisher={Twente University Press}
}

@book{134Wingerden,
  title={Control of wind turbines with'Smart'rotors: proof of concept \& {LPV} subspace identification},
  author={van Wingerden, J. W.},
  year={2008},
  publisher={TU Delft, Delft University of Technology}
}

@inproceedings{136Toth,
  title={Model structure learning: A support vector machine approach for {LPV} linear-regression models},
  author={T{\'o}th, R. and Laurain, V. and Zheng, W. X. and Poolla, K.},
  booktitle={Decision and Control and European Control Conference (CDC-ECC), 2011 50th IEEE Conference on},
  pages={3192--3197},
  year={2011},
  organization={IEEE}
}

@article{137Rasmussen,
  title={Occam's razor},
  author={Rasmussen, C. E. and Ghahramani, Z.},
  journal={Advances in neural information processing systems},
  pages={294--300},
  year={2001},
  publisher={MIT; 1998}
}

@book{138Mohammadpour,
  title={Control of linear parameter varying systems with applications},
  author={Mohammadpour, J. and Scherer, C.},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@article{139Leith,
  title={Survey of gain-scheduling analysis and design},
  author={Leith, D. J. and Leithead, W. E.},
  journal={International journal of control},
  volume={73},
  number={11},
  pages={1001--1025},
  year={2000},
  publisher={Taylor \& Francis}
}

@article{140Rugh,
title = "Research on gain scheduling ",
journal = "Automatica ",
volume = "36",
number = "10",
pages = "1401 - 1425",
year = "2000",
author = "Rugh, W. J. and Shamma, J. S."
}

@misc{141Orr,
  title={Introduction to radial basis function networks},
  author={Orr, M. J. L.},
  year={1996},
  publisher={Technical Report, Center for Cognitive Science, University of Edinburgh}
}

@article{142Golub,
author = {Golub, Gene H. and Heath, Michael and Wahba, Grace},
title = {Generalized Cross-Validation as a Method for Choosing a Good Ridge Parameter},
journal = {Technometrics},
volume = {21},
number = {2},
pages = {215-223},
year = {1979},
doi = {10.1080/00401706.1979.10489751}
}

@book{143Wahba,
  title={Spline models for observational data},
  author={Wahba, Grace},
  volume={59},
  year={1990},
  publisher={Siam}
}

@article{144Rasmussen,
  title={{Gaussian processes for machine learning (GPML) toolbox}},
  author={Rasmussen, C. E. and Nickisch, H.},
  journal={The Journal of Machine Learning Research},
  volume={11},
  pages={3011--3015},
  year={2010},
  publisher={JMLR. org}
}

@misc{145Houtzager,
  title={Predictor-based Subspace Identification Toolbox Version 0. 4},
  author={Houtzager, I. and Gebraad, P. and van Wingerden, J. W. and Verhaegen, M.},
  year={2010}
}

@article{146Stoica,
  title={On biased estimators and the unbiased Cram{\'e}r-Rao lower bound},
  author={Stoica, Petre and Moses, Randolph L},
  journal={Signal Processing},
  volume={21},
  number={4},
  pages={349--350},
  year={1990},
  publisher={Elsevier}
}

@inproceedings{147Pillonetto,
  title={Pitfalls of the Parametric Approaches Exploiting Cross-Validation for Model Order Selection},
  author={Pillonetto, Gianluigi and de Nicolao, Giuseppe},
  booktitle={System Identification},
  volume={16},
  number={1},
  pages={215--220},
  year={2012}
}

@inproceedings{148Chiuso,
  title={Regularization strategies for nonparametric system identification},
  author={Chiuso, Alessandro and Chen, Tianshi and Ljung, Lennart and Pillonetto, Gianluigi},
  booktitle={Decision and Control (CDC), 2013 IEEE 52nd Annual Conference on},
  pages={6013--6018},
  year={2013},
  organization={IEEE}
}

@inproceedings{149Aravkin,
  title={Convex vs nonconvex approaches for sparse estimation: Lasso, Multiple Kernel Learning and Hyperparameter Lasso},
  author={Aravkin, Aleksander and Burke, James V and Chiuso, Alessandro and Pillonetto, Gianluigi},
  booktitle={Decision and Control and European Control Conference (CDC-ECC), 2011 50th IEEE Conference on},
  pages={156--161},
  year={2011},
  organization={IEEE}
}

@article{150Houtzager,
  title={Recursive predictor-based subspace identification with application to the real-time closed-loop tracking of flutter},
  author={Houtzager, I. and van Wingerden, J. W. and Verhaegen, M.},
  journal={Control Systems Technology, IEEE Transactions on},
  volume={20},
  number={4},
  pages={934--949},
  year={2012},
  publisher={IEEE}
}

@article{151Lovera,
  title={Recursive subspace identification of linear and non-linear Wiener state-space models},
  author={Lovera, M. and Gustafsson, T. and Verhaegen, M.},
  journal={Automatica},
  volume={36},
  number={11},
  pages={1639--1650},
  year={2000},
  publisher={Elsevier}
}

@INPROCEEDINGS{152Huber, 
author={Huber, M.F.}, 
booktitle={Acoustics, Speech and Signal Processing (ICASSP), 2013 IEEE International Conference on}, 
title={{Recursive Gaussian process regression}}, 
year={2013}, 
month={May}, 
pages={3362-3366}, 
ISSN={1520-6149},}

@article{153Merriman,
  title={On the history of the method of least squares},
  author={Merriman, Mansfield},
  journal={The Analyst},
  pages={33--36},
  year={1877},
  publisher={JSTOR}
}

@article{154Freeth,
  title={Decoding the ancient Greek astronomical calculator known as the Antikythera Mechanism},
  author={Freeth, T. and Bitsakis, Y. and Moussas, X. and Seiradakis, J.H. and Tselikas, A. and Mangou, .H and Zafeiropoulou, M. and Hadland, R. and Bate, D. and Ramsey, A.},
  journal={Nature},
  volume={444},
  number={7119},
  pages={587--591},
  year={2006},
  publisher={Nature Publishing Group}
}

@book{155Scholkopf,
  title={Learning with kernels: Support vector machines, regularization, optimization, and beyond},
  author={Sch{\"o}lkopf, B. and Smola, A. J.},
  year={2002},
  publisher={MIT Press}
}

@article{160Jansen,
  title={Magnetically levitated planar actuator with moving magnets},
  author={Jansen, J. W. and van Lierop, C. M. M. and Lomonova, E. A. and Vandenput, A. J. A.},
  journal={IEEE Transactions on Industry Applications},
  volume={44},
  number={4},
  pages={1108--1115},
  year={2008},
  publisher={IEEE}
}

@inproceedings{161Darwish,
  title={Bayesian Identification of {LPV} Box-Jenkins Models},
  author={Darwish, M. and Cox, P. and Pillonetto, G. and T\'{o}th, R.},
  booktitle={Proceedings of the 54th IEEE Conference on Decision and Control (CDC), Osaka, Japan},
  year={2015},
  organization={IEEE}
}

@inproceedings{162Proimadis,
  title={A kernel based approach for {LPV} subspace identification},
  author={Proimadis, Ioannis and Bijl, Hildo and van Wingerden, Jan Willem},
  booktitle={Proceedings of the 1st IFAC Workshop on Linear Parameter Varying Systems, Grenoble, France},
  year={2015},
}

@article{163Golabi, 
author={A. {Golabi} and N. {Meskin} and R. {T{\'o}th} and J. {Mohammadpour}}, 
booktitle={53rd IEEE Conference on Decision and Control}, 
title={{A Bayesian approach for estimation of linear-regression LPV models}}, 
year={2014}, 
volume={}, 
number={}, 
pages={2555-2560}, 
doi={10.1109/CDC.2014.7039779}, 
ISSN={0191-2216}, 
month={Dec}
}

@article{166Akoun,
  title={{3D} analytical calculation of the forces exerted between two cuboidal magnets},
  author={Akoun, G. and Yonnet, J. P.},
  journal={Magnetics, IEEE Transactions on},
  volume={20},
  number={5},
  pages={1962--1964},
  year={1984},
  publisher={IEEE}
}

@article{167Jansen,
  title={Analytical calculation of interaction force between orthogonally magnetized permanent magnets},
  author={Jansen, J. L. G. and Paulides, J. J. H. and Lomonova, E. A. and B{\"o}l{\"o}ni, F. and Tounzi, A. and Piriou, F.},
  journal={Sensor letters},
  volume={7},
  number={3},
  pages={442--445},
  year={2009},
  publisher={American Scientific Publishers}
}

@article{168Rovers,
  title={Calculation of the static forces among the permanent magnets in a {Halbach} array},
  author={Rovers, J. M. M. and Jansen, J. W. and Lomonova, E. A. and Ronde, M. J. C.},
  journal={IEEE Transactions on Magnetics},
  volume={45},
  number={10},
  pages={4372--4375},
  year={2009},
  publisher={IEEE}
}

@article{169Rovers,
  title={Analytical calculation of the force between a rectangular coil and a cuboidal permanent magnet},
  author={Rovers, J. M. M. and Jansen, J. W. and Lomonova, E. A.},
  journal={Magnetics, IEEE Transactions on},
  volume={46},
  number={6},
  pages={1656--1659},
  year={2010},
  publisher={IEEE}
}

@article{171Jansen,
  title={Modeling of magnetically levitated planar actuators with moving magnets},
  author={Jansen, J. W. and van Lierop, C. M. M. and Lomonova, E. A. and Vandenput, A. J. A.},
  journal={Magnetics, IEEE Transactions on},
  volume={43},
  number={1},
  pages={15--25},
  year={2007},
  publisher={IEEE}
}

@article{172Compter,
  title={Electro-dynamic planar motor},
  author={Compter, J. C.},
  journal={Precision Engineering},
  volume={28},
  number={2},
  pages={171--180},
  year={2004},
  publisher={Elsevier}
}

@article{173Rovers,
  title={Analysis method of the dynamic force and torque distribution in the magnet array of a commutated magnetically levitated planar actuator},
  author={Rovers, J. M. M. and Jansen, J. W. and Compter, J. C. and Lomonova, E. A.},
  journal={IEEE Transactions on Industrial Electronics},
  volume={59},
  number={5},
  pages={2157--2166},
  year={2012},
  publisher={IEEE}
}

@article{174Jansen,
  title={Overview of analytical models for the design of linear and planar motors},
  author={Jansen, J. W. and Smeets, J. P. C. and Overboom, T. T. and Rovers, J. M. M. and Lomonova, E. A.},
  journal={IEEE Transactions on Magnetics},
  volume={50},
  number={11},
  pages={1--7},
  year={2014},
  publisher={IEEE}
}


@article{175Wassink,
  title={{LPV} control for a wafer stage: beyond the theoretical solution},
  author={Wassink, M. G. and van de Wal, M. and Scherer, C. and Bosgra, O.},
  journal={Control Engineering Practice},
  volume={13},
  number={2},
  pages={231--245},
  year={2005},
  publisher={Elsevier}
}

@article{176Butler,
  title={Position control in lithographic equipment},
  author={Butler, H.},
  journal={IEEE Control Systems Magazine},
  volume={31},
  number={5},
  pages={28--47},
  year={2011}
}

@article{177Rovers,
title = "The deformation of the moving magnet plate of a commutated magnetically levitated planar actuator ",
journal = "Mechatronics ",
volume = "23",
number = "2",
pages = "233 - 239",
year = "2013",
note = "Special Issue on Linear Drives ",
issn = "0957-4158",
doi = "http://dx.doi.org/10.1016/j.mechatronics.2012.01.011",
author = "Rovers, J.M.M. and Achterberg, J. and Ronde, M.J.C. and  Jansen, J.W. and Compter, J.C. and Lomonova, E.A. and van Lierop, C.M.M. and  van den Molengraft, M.J.G.",
}

@inproceedings{179Verkerk,
  title={Modal observer design for a flexible motion system with state dependent sensor positions},
  author={Verkerk, K. W. and Achterberg, J. and van Lierop, C. M. M. and Weiland, S.},
  booktitle={Decision and Control (CDC), 2012 IEEE 51st Annual Conference on},
  pages={4498--4504},
  year={2012},
  organization={IEEE}
}

@inproceedings{180Verkerk,
  title={State estimator synthesis for position dependent flexible systems with position independent error convergence},
  author={Verkerk, K.W. and Kasemsinsup, Y. and Butler, H. and Weiland, S.},
  booktitle={Control and Automation (MED), 2015 23th Mediterranean Conference on},
  pages={1065--1070},
  year={2015},
  organization={IEEE}
}

@MastersThesis{181Kasemsinsup,
  title={Position-dependent state observer design for a planar motor wafer stage},
  author={Kasemsinsup, Y.},
  year={2013},
  school={Department of Electrical Engineering, Control Systems Group, Eindhoven University of Tehcnology}
    }
    
@article{183Pillonetto,
  title={A new kernel-based approach for nonlinear system identification},
  author={Pillonetto, G. and Quang, M. H. and Chiuso, A.},
  journal={Automatic Control, IEEE Transactions on},
  volume={56},
  number={12},
  pages={2825--2840},
  year={2011},
  publisher={IEEE}
}


@article{184Jeltsema,
  title={Multidomain modeling of nonlinear networks and systems},
  author={Jeltsema, D. and Scherpen, J.M.A.},
  journal={IEEE Control Systems},
  volume={29},
  number={4},
  pages={28--59},
  year={2009},
  publisher={IEEE}
}

@article{185Wal,
  title={Multivariable $\mathcal{H}_\infty$/$\mu$ feedback control design for high-precision wafer stage motion},
  author={van de Wal, M. and van Baars, G. and Sperling, F. and Bosgra, O.},
  journal={Control Engineering Practice},
  volume={10},
  number={7},
  pages={739--755},
  year={2002},
  publisher={Elsevier}
}

@article{187Wal,
  title={Experimentally validated multivariable $\mu$ feedback controller design for a high-precision wafer stage},
  author={van de Wal, M. and van Baars, G. and Sperling, F. and Bosgra, O.},
  booktitle={Decision and Control, 2001. Proceedings of the 40th IEEE Conference on},
  volume={2},
  pages={1583--1588},
  year={2001},
  organization={IEEE}
}

@article{188Hughes,
  title={Space structure vibration modes: How many exist? Which ones are important?},
  author={Hughes, P.},
  journal={IEEE Control Systems Magazine},
  volume={7},
  number={1},
  pages={22--28},
  year={1987},
  publisher={IEEE}
}

@article{189Schneiders, 
author={M. G. E. Schneiders and M. J. G. van de Molengraft and M. Steinbuch}, 
booktitle={Proceedings of the 2004 American Control Conference}, 
title={Benefits of over-actuation in motion systems}, 
year={2004}, 
volume={1}, 
number={}, 
pages={505-510 vol.1}, 
keywords={motion control;vibration control;actuators;feedforward;feedback;control system synthesis;motion control system;feedback controller design;vibration control strategy;disturbance attenuation;feedforward path;Actuators;Resonance;Attenuation;Controllability;Feedback;Tuning;Adaptive control;Vibration control;Bandwidth;Resonant frequency}, 
doi={10.23919/ACC.2004.1383653}, 
ISSN={0743-1619}, 
month={June},}

@inbook{190Steinbuch,
title = "Advanced Motion Control Design",
abstract = "No abstract.",
author = "M. Steinbuch and R.J.E. Merry and M.L.G. Boerlage and M.J.C. Ronde and {Molengraft, van de}, M.J.G.",
year = "2010",
doi = "10.1201/b10382-35",
language = "English",
isbn = "978-1-4200-7360-7",
pages = "27--1/25",
booktitle = "The Control Handbook, Control System Applications, Second edition",
publisher = "CRC Press",

}


@article{191Lierop,
  title={Model-based commutation of a long-stroke magnetically levitated linear actuator},
  author={van Lierop, C. M. M. and Jansen, J. W. and Damen, A. A. H. and Lomonova, E. A. and van Den Bosch, P. P. J. and Vandenput, A. J. A.},
  journal={IEEE Transactions on Industry Applications},
  volume={45},
  number={6},
  pages={1982--1990},
  year={2009},
  publisher={IEEE}
}

@misc{192Moore,
  title={Cramming more components onto integrated circuits},
  author={Moore, G. E.},
  year={1965},
  publisher={McGraw-Hill New York, NY, USA}
}

@inproceedings{193Jong,
  title={Enabling the lithography roadmap: an immersion tool based on a Novel Stage Positioning System},
  author={de Jong, F. and van der Pasch, B. and Castenmiller, T. and Vleeming, B. and Droste, R. and van de Mast, F.},
  booktitle={SPIE Advanced Lithography},
  pages={72741S--72741S},
  year={2009},
  organization={International Society for Optics and Photonics}
}

@article{194Rovers,
title = "Real-time {3D} thermal modeling of a magnetically levitated planar actuator ",
journal = "Mechatronics ",
volume = "23",
number = "2",
pages = "240 - 246",
year = "2013",
note = "Special Issue on Linear Drives ",
issn = "0957-4158",
doi = "http://dx.doi.org/10.1016/j.mechatronics.2012.04.004",
author = "Rovers, J.M.M.  and St{\"o}ck, M.  and  Jansen, J.W. and  van Lierop, C.M.M. and Lomonova,  E.A. and Perriard, Y. "
}

@inproceedings{195Rovers,
  title={Design and measurements of the double layer planar motor},
  author={Rovers, J. M. M. and Jansen, J. W. and Lomonova, E. A.},
  booktitle={Electric Machines \& Drives Conference (IEMDC), 2013 IEEE International},
  pages={204--211},
  year={2013},
  organization={IEEE}
}

@article{196Rovers,
  title={Multiphysical analysis of moving-magnet planar motor topologies},
  author={Rovers, J. M. M. and Jansen, J. W. and Lomonova, E. A.},
  journal={Magnetics, IEEE Transactions on},
  volume={49},
  number={12},
  pages={5730--5741},
  year={2013},
  publisher={IEEE}
}

@inproceedings{197Achterberg,
  title={Performance of a six Degree-of-Freedom controlled moving-magnet planar actuator with a laser interferometer measurement setup},
  author={Achterberg, J. and Rovers, J. M. M. and van Lierop, C. M. M. and Jansen, J. W. and van den Bosch, P. P. J.},
  booktitle={Eighth international symposium on linear drives for industry applications},
  year={2011},
  address = {},
  month = {}
}


@article{198Steinbuch,
title = "Advanced Motion Control: An Industrial Perspective",
journal = "European Journal of Control",
volume = "4",
number = "4",
pages = "278 - 293",
year = "1998",
issn = "0947-3580",
doi = "https://doi.org/10.1016/S0947-3580(98)70121-9",
author = "M. Steinbuch and M.L. Norg",
keywords = "Application, Compact disk, Disturbance rejection, Drives, Hard disk, Model-based control, Motion control, Robust control",
abstract = "Industrial feedback motion controllers are tuned using manual loopshaping, according to certain design rules. This controller tuning serves as a benchmark for robust control research as applied to optical and magnetic disk drive storage systems. The design and implementation of robust controllers for the focus servo of a compact disk and the tracking servo of a hard disk mechanism is investigated. The design objective is to achieve good track-following performance in the presence of disk disturbances. H∞ robust control is used to systematically include disturbance and specification models in the standard plant framework. The control design iteration is based on disturbance identification, including implementation within the design cycle. The industrial relevance of robust control is discussed and areas for academic research in robust control are indicated, as feedback from industry."
}

@inproceedings{199Chen,
  title={{LPV} control design for precision motion systems},
  author={Chen, N. and Wen, J. T.},
  booktitle={2014 American Control Conference},
  pages={4470--4475},
  year={2014},
  organization={IEEE}
}

@inproceedings{205Kasemsinsup,
  title={Exact plant inversion of flexible motion systems with a time-varying state-to-output map},
  author={Kasemsinsup, Y. and Heertjes, M. and Butler, H. and Weiland, S.},
  booktitle={2016 European Control Conference (ECC)},
  pages={2483--2488},
  year={2016},
  organization={IEEE}
}

@INPROCEEDINGS{206Boerlage, 
title={Model-based feedforward for motion systems},
author={M. {Boerlage} and M. {Steinbuch} and P. {Lambrechts} and M. {van de Wal}}, 
booktitle={Proceedings of 2003 IEEE Conference on Control Applications, 2003. CCA 2003.}, 
year={2003}, 
volume={2}, 
number={}, 
pages={1158-1163 vol.2}
}

@article{207Clayton,
  title={A review of feedforward control approaches in nanopositioning for high-speed SPM},
  author={Clayton, G. M. and Tien, S. and Leang, K. K. and Zou, Q. and Devasia, S.},
  journal={Journal of dynamic systems, measurement, and control},
  volume={131},
  number={6},
  pages={061101},
  year={2009},
  publisher={American Society of Mechanical Engineers}
}

@article{208Lambrechts,
  title={Trajectory planning and feedforward design for electromechanical motion systems},
  author={Lambrechts, P. and Boerlage, M. and Steinbuch, M.},
  journal={Control Engineering Practice},
  volume={13},
  number={2},
  pages={145--157},
  year={2005},
  publisher={Elsevier}
}

@article{209Heertjes,
  title={{MIMO} feed-forward design in wafer scanners using a gradient approximation-based algorithm},
  author={Heertjes, M. and Hennekens, D. and Steinbuch, M.},
  journal={Control Engineering Practice},
  volume={18},
  number={5},
  pages={495--506},
  year={2010},
  publisher={Elsevier}
}

@inproceedings{211Steinbuch,
  title={Experimental modelling and {LPV} control of a motion system},
  author={Steinbuch, M. and van de Molengraft, R. and van der Voort, A.},
  booktitle={American Control Conference, 2003. Proceedings of the 2003},
  volume={2},
  pages={1374--1379},
  year={2003},
  organization={IEEE}
}

@article{212Scherer,
  title={{LPV} control and full block multipliers},
  author={Scherer, C.},
  journal={Automatica},
  volume={37},
  number={3},
  pages={361--375},
  year={2001},
  publisher={Elsevier}
}

@article{214Toth,
author={R. {T\'{o}th} and M. {van de Wal} and P. S. C. {Heuberger} and P. M. J. {van den Hof}},
booktitle={Proceedings of the 2011 American Control Conference},
title={{LPV} identification of high performance positioning devices},
year={2011},
volume={},
number={},
pages={151-158},
doi={10.1109/ACC.2011.5990902},
ISSN={2378-5861},
month={June},}

@ARTICLE{221Hoffman,
author={C. {Hoffmann} and H. {Werner}},
journal={IEEE Transactions on Control Systems Technology},
title={A Survey of Linear Parameter-Varying Control Applications Validated by Experiments or High-Fidelity Simulations},
year={2015},
volume={23},
number={2},
pages={416-433},
doi={10.1109/TCST.2014.2327584},
ISSN={1063-6536},
month={March},}


@article{224Shamma,
  title={Gain scheduling: Potential hazards and possible remedies},
  author={Shamma, J. S. and Athans, M.},
  journal={IEEE Control Systems Magazine},
  volume={12},
  number={3},
  pages={101--107},
  year={1992},
  publisher={IEEE}
}

@article{237Gahinet,
author = {Gahinet, P. and Apkarian, P.},
title = {A linear matrix inequality approach to $\mathcal{H}_{\infty}$ control},
journal = {International Journal of Robust and Nonlinear Control},
volume = {4},
number = {4},
pages = {421-448},
keywords = {State-space H∞ control, Linear matrix inequalities, Riccati inequalities, Loop shaping},
doi = {10.1002/rnc.4590040403},
year = {1994}
}


@inproceedings{238Kulcsar,
title = "On the similarity state transformation for linear parameter-varying systems",
abstract = "Abstract: Similarity state transformations between equivalent State-Space (SS) representations of discrete-time Linear Parameter-Varying (LPV) systems are investigated. Based on previous results, it is known that to characterize all equivalent LPV-SS representations, the statetransformation matrix must depend dynamically on the scheduling variable. However, preserving static dependence of a LPV-SS representation, i.e. characterizing all equivalent SS representation with static dependence, has primary importance both in control and identication. Therefore, rst, the state transformation problem is investigated from an algebraic (behavior) point of view, then conditions are developed to guarantee preservation of the static dependence in similarity state transformations. Additional geometric interpretation of the obtained results, together with computational approach to synthesize state-transformations are also developed. An illustrative example is provided to demonstrate the validity of the obtained results.",
author = "B. Kulcsar and R. Toth",
year = "2011",
language = "English",
pages = "4155--4160",
booktitle = "Proceedings of the 18th IFAC World Congress, 28 August-2 September 2011, Milano, Italy",
publisher = "International Federation of Automatic Control",
}

@unpublished{240Zhang,
  TITLE = {{On local LTI model coherence for LPV interpolation}},
  AUTHOR = {Zhang, Q. and Ljung, L. and Pintelon, R.},
  NOTE = {working paper or preprint},
  YEAR = {2018},
  MONTH = Apr,
  PDF = {https://hal.inria.fr/hal-01758337/file/coherence_hal.pdf},
  HAL_ID = {hal-01758337},
  HAL_VERSION = {v1},
}

@article{241Zhang,
title = "From structurally independent local {LTI} models to {LPV} model",
journal = "Automatica",
volume = "84",
pages = "232 - 235",
year = "2017",
issn = "0005-1098",
doi = "https://doi.org/10.1016/j.automatica.2017.06.006",
author = "Qinghua Z. and Lennart L.",
abstract = "The local approach to linear parameter varying (LPV) system identification consists in interpolating individually estimated local linear time invariant (LTI) models corresponding to fixed values of the scheduling variable. It is shown in this paper that, without any global structural assumption of the considered LPV system, individually estimated local state-space LTI models do not contain sufficient information for determining similarity transformations making them coherent. It is possible to estimate these similarity transformations from input–output data under appropriate excitation conditions."
}

@ARTICLE{242Shamma, 
author={J. S. {Shamma} and M. {Athans}}, 
journal={IEEE Transactions on Automatic Control}, 
title={Analysis of gain scheduled control for nonlinear plants}, 
year={1990}, 
volume={35}, 
number={8}, 
pages={898-907}, 
keywords={control system analysis;nonlinear systems;scheduling;stability;gain scheduled control;nonlinear plants;design;robustness;reference trajectory;stability;nonlinearities;Robust stability;Processor scheduling;Performance gain;Feedback;Design methodology;Acoustical engineering;Design engineering;Performance analysis;Stability analysis;Control systems}, 
doi={10.1109/9.58498}, 
ISSN={0018-9286}, 
month={Aug},}

@article{250Mottershead,
  title={Model updating in structural dynamics: a survey},
  author={Mottershead, J. E. and Friswell, M. I.},
  journal={Journal of sound and vibration},
  volume={167},
  number={2},
  pages={347--375},
  year={1993},
  publisher={Elsevier}
}

@article{251Dorosti,
title = "Iterative pole-zero finite element model updating using generic parameters",
journal = "Mechatronics",
volume = "55",
pages = "180 - 193",
year = "2018",
issn = "0957-4158",
doi = "https://doi.org/10.1016/j.mechatronics.2018.06.012",
author = "M. Dorosti and R.H.B. Fey and M.F. Heertjes and M.M.J. van de Wal and H. Nijmeijer",
keywords = "FE model, Model updating, System identification, Prediction and control, Generic parameters",
abstract = "Prediction and control of unmeasurable performance variables in complex large-scale systems is an important topic in systems and control. The preferred solution to this problem is to have a relatively low-order and accurate standard plant model. A reduced Finite Element (FE) dynamic model may be a good candidate for that purpose apart from the fact that its accuracy is always limited, since it never truly matches the real structure. In this paper, an iterative procedure is proposed to update the FE model using poles and zeros estimated from the measured Frequency Response Functions (FRFs). Assuming the errors in the FE stiffness and/or damping matrix to be dominant over the mass matrix, but the exact physical parameters responsible for these errors to be unknown, the eigenvalues of the (sub)structure stiffness and/or damping matrix may be updated to reduce the differences between the poles and zeros from the model and measured FRFs. The proposed procedure matches poles and zeros sequentially in an iterative manner as to realize convergence to the measured quantities. This procedure, further referred to as Iterative Pole-Zero (IPZ) model updating, facilitates the process of obtaining improved parametric models which can be used for accurate prediction and control of unmeasurable performance variables. The proposed procedure is first illustrated using a mass-spring model and then is validated via a collocated FRF measurement from an experimental beam setup."
}

@article{252Mottershead,
  title={The sensitivity method in finite element model updating: a tutorial},
  author={Mottershead, J. E. and Link, M. and Friswell, M. I.},
  journal={Mechanical systems and signal processing},
  volume={25},
  number={7},
  pages={2275--2296},
  year={2011},
  publisher={Elsevier}
}

@inproceedings{260Lofberg,
address = {Taipei, Taiwan},
author = {L{\"{o}}fberg, J.},
booktitle = {In Proceedings of the CACSD Conference},
title = {{YALMIP : A Toolbox for Modeling and Optimization in MATLAB}},
year = {2004}
}

@article{270Besselink,
  title={A comparison of model reduction techniques from structural dynamics, numerical mathematics and systems and control},
  author={Besselink, B. and Tabak, U. and Lutowska, A. and van de Wouw, N. and Nijmeijer, H. and Rixen, D. J. and Hochstenbach, M. E. and Schilders, W. H. A.},
  journal={Journal of Sound and Vibration},
  volume={332},
  number={19},
  pages={4403--4422},
  year={2013},
  publisher={Elsevier}
}


@inproceedings{271Heertjes,
author={M. {Heertjes} and D. {Hennekens} and A. {van Engelen} and M. {Steinbuch}},
booktitle={Proceedings of the 48h IEEE Conference on Decision and Control (CDC) held jointly with 2009 28th Chinese Control Conference},
title={Dynamic decoupling in motion systems using a gradient approximation-based algorithm},
year={2009}
}

@article{272Meulen,
  title={Fixed structure feedforward controller design exploiting iterative trials: Application to a wafer stage and a desktop printer},
  author={van der Meulen, Stan H and Tousain, Rob L and Bosgra, Okko H},
  journal={Journal of Dynamic Systems, Measurement, and Control},
  volume={130},
  number={5},
  pages={051006},
  year={2008},
  publisher={American Society of Mechanical Engineers}
}

@article{274Arora,
  title={Comparative study of finite element model updating methods},
  author={Arora, V.},
  journal={Journal of Vibration and Control},
  volume={17},
  number={13},
  pages={2023--2039},
  year={2011},
  publisher={Sage Publications Sage UK: London, England}
}



@article{275Dorosti,
title = "Finite Element Model Reduction and Model Updating of structures for Control",
journal = "IFAC Proceedings Volumes",
volume = "47",
number = "3",
pages = "4517 - 4522",
year = "2014",
note = "19th IFAC World Congress",
issn = "1474-6670",
doi = "https://doi.org/10.3182/20140824-6-ZA-1003.01644",
author = "Dorosti, M. and Fey, R. and Heertjes, M. and van de Wal, M. and Nijmeijer, H.",
keywords = "Model updating, model reduction, finite element model, identification, model-based control"
}

@INPROCEEDINGS{276Dorosti, 
author={M. Dorosti and F. J. M. Heck and R. H. B. Fey and M. F. Heertjes and M. M. J. van de Wal and H. Nijmeijer}, 
booktitle={2016 American Control Conference (ACC)}, 
title={Frequency Response Sensitivity model updating using generic parameters}, 
year={2016}, 
volume={}, 
number={}, 
pages={6215-6220}, 
keywords={damping;eigenvalues and eigenfunctions;elastic constants;finite element analysis;frequency response;matrix algebra;2D pinned-sliding beam system;FE dynamic models;FE model updating algorithm;FRS model;damping matrix;eigenvalues;finite element dynamic models;frequency response sensitivity model;generic parameters;high-precision system;stiffness matrix;unmeasured performance variables;Computational modeling;Damping;Eigenvalues and eigenfunctions;Mathematical model;Matrix decomposition;Semiconductor device modeling;Zinc}, 
doi={10.1109/ACC.2016.7526646}, 
ISSN={}, 
month={July},}

@article{277Balas,
  title={Active control of flexible systems},
  author={Balas, M. J.},
  journal={Journal of Optimization theory and Applications},
  volume={25},
  number={3},
  pages={415--436},
  year={1978},
  publisher={Springer}
}

@article{278Rozario,
  title={Global feedforward control of spatio-temporal mechanical systems: with application to a prototype wafer stage},
  author={de Rozario, R. and Voorhoeve, R. and Aangenent, W. and Oomen, T.},
  journal={IFAC-PapersOnLine},
  volume={50},
  number={1},
  pages={14575--14580},
  year={2017},
  publisher={Elsevier}
}

@article{280Schneiders,
  title={Introduction to an integrated design for motion systems using over-actuation},
  author={Schneiders, M.G.E. and van de Molengraft, M.J.G. and Steinbuch, M.},
  booktitle={European Control Conference (ECC), 2003},
  pages={3249--3254},
  year={2003},
  organization={IEEE}
}

@inproceedings{282Galvan, 
author={S. D. Galvan and M. Heertjes and R. Dunand}, 
booktitle={2012 American Control Conference (ACC)}, 
title={Plant enhancements in motion systems by modal control}, 
year={2012}
}

@article{283Herpen,
title = "Exploiting additional actuators and sensors for nano-positioning robust motion control",
journal = "Mechatronics",
volume = "24",
number = "6",
pages = "619 - 631",
year = "2014",
issn = "0957-4158",
doi = "https://doi.org/10.1016/j.mechatronics.2014.03.008",
author = "van Herpen, R. and Oomen, T. and Kikken, E. and van de Wal, M. and Aangenent, W. and Steinbuch, M.",
keywords = "Mechatronic systems, Performance limitations, Robust control, System identification, Input–output selection"
}

@article{285Vizer,
  title={$\mathcal{H}_\infty$-norm-based optimization for the identification of gray-box {LTI} state-space model parameters},
  author={Vizer, D. and Merc{\`e}re, G. and Prot, O. and Laroche, E.},
  journal={Systems \& Control Letters},
  volume={92},
  pages={34--41},
  year={2016},
  publisher={Elsevier}
}

@article{286Bergamasco,
  title={State space model identification: from unstructured to structured models with an $\mathcal{H}_\infty$ approach},
  author={Bergamasco, M. and Lovera, M.},
  journal={IFAC Proceedings Volumes},
  volume={46},
  number={2},
  pages={202--207},
  year={2013},
  publisher={Elsevier}
}

@article{289Marcos,
  title={Development of linear-parameter-varying models for aircraft},
  author={Marcos, A. and Balas, G. J.},
  journal={Journal of Guidance, Control, and Dynamics},
  volume={27},
  number={2},
  pages={218--228},
  year={2004}
}

@ARTICLE{300Bristow, 
author={D. A. Bristow and M. Tharayil and A. G. Alleyne}, 
journal={IEEE Control Systems}, 
title={A survey of iterative learning control}, 
year={2006}, 
volume={26}, 
number={3}, 
pages={96-114}, 
keywords={adaptive control;control system analysis;control system synthesis;feedback;feedforward;iterative methods;learning systems;robust control;design techniques;feedback control;feedforward control;iterative learning control;learning algorithms;learning transient behavior;robotics;stability;Adaptive control;Chemical industry;Control systems;Error correction;Iterative methods;Learning systems;Motion control;Muscles;Open loop systems;Radio control}, 
doi={10.1109/MCS.2006.1636313}, 
ISSN={1066-033X}, 
month={June}
}

@article{284Oomen,
  title={Connecting system identification and robust control for next-generation motion control of a wafer stage},
  author={Oomen, T. and van Herpen, R. and Quist, S. and van de Wal, M. and Bosgra, O. and Steinbuch, M.},
  journal={IEEE Transactions on Control Systems Technology},
  volume={22},
  number={1},
  pages={102--118},
  year={2014},
  publisher={IEEE}
}

@article{287Taamallah,
  title={{LPV} modelling with affine dependence: A local $\mathcal{H}_{\infty}$ approach},
  author={Taamallah, S. and Bombois, X. and T{\'o}th, R. and van den Hof, P. M. J.},
  journal={International Journal of RObust and Nonlinear Control},
  pages={1--19},
  year={2016},
  publisher={John Wiley and Sons, Ltd.},
  year={2016}
}

@INPROCEEDINGS{288Taamallah,
author={S. {Taamallah} and X. {Bombois} and P. M. J. {van den Hof}},
booktitle={52nd IEEE Conference on Decision and Control},
title={Affine {LPV} modeling: An $\mathcal{H}_{\infty}$ based approach},
year={2013},
volume={},
number={},
pages={2726-2733},
doi={10.1109/CDC.2013.6760295},
ISSN={0191-2216},
month={Dec},}

@article{301Mishra,
  title={Precision positioning of wafer scanners segmented iterative learning control for nonrepetitive disturbances [applications of control]},
  author={Mishra, S. and Coaplen, J. and Tomizuka, M.},
  journal={IEEE control systems},
  volume={27},
  number={4},
  pages={20--25},
  year={2007},
  publisher={IEEE}
}

@ARTICLE{302Bolder, 
author={J. Bolder and T. Oomen}, 
journal={IEEE Transactions on Control Systems Technology}, 
title={Rational Basis Functions in Iterative Learning Control - With Experimental Verification on a Motion System}, 
year={2015}, 
volume={23}, 
number={2}, 
pages={722-729}, 
keywords={extrapolation;iterative learning control;optimisation;ILC approaches;complex optimization problem;exogenous signals;experimental verification;extrapolation properties;iterative learning control;iterative optimization algorithm;motion system;rational basis functions;setpoint variations;single-input single-output systems;Convolution;Extrapolation;Feedforward neural networks;Finite impulse response filters;Optimization;Polynomials;Vectors;Basis functions;iterative learning control (ILC);optimal control;optimal control.}, 
doi={10.1109/TCST.2014.2327578}, 
ISSN={1063-6536}, 
month={March}
}


@article{303Butler,
title = "Magnetic disturbance compensation for a reticle stage in a lithographic tool",
journal = "Mechatronics",
volume = "23",
number = "6",
pages = "559 - 565",
year = "2013",
issn = "0957-4158",
doi = "https://doi.org/10.1016/j.mechatronics.2013.04.011",
author = "Butler, H.",
keywords = "Reticle stage, Lithography, Feedforward, Magnetic interaction"
}

@article{309Hof,
  title={Closed-loop issues in system identification},
  author={van den Hof, P. M. J.},
  journal={Annual reviews in control},
  volume={22},
  pages={173--186},
  year={1998},
  publisher={Elsevier}
}



@article{310Darwish,
title = "Prediction-error identification of {LPV} systems: A nonparametric {Gaussian} regression approach",
journal = "Automatica",
volume = "97",
pages = "92 - 103",
year = "2018",
issn = "0005-1098",
doi = "https://doi.org/10.1016/j.automatica.2018.07.032",
author = "M.A.H. Darwish and P.B. Cox and I. Proimadis and G. Pillonetto and R. T{\'o}th"
}

@inproceedings{313Callafon,
author={R. A. {de Callafon} and D. {de Roover} and P. M. J. {van den Hof}},
title={Multivariable least squares frequency domain identification using polynomial matrix fraction descriptions},
booktitle={Proceedings of 35th IEEE Conference on Decision and Control},
year={1996}
}

@article{316Voorhoeve,
  author={Voorhoeve, R. and {de Rozario}, R. and Aangenent, W. and Oomen, T.},
  title={Identifying Position-Dependent Mechanical Systems: A Modal Approach with Applications to Wafer Stage Control},
  journal={{arXiv preprint arXiv:1807.06942}},
  year={2018}
}


@ARTICLE{317Mercere,
author={G. {Merc{\`e}re} and O. {Prot} and J. A. {Ramos}},
journal={IEEE Transactions on Automatic Control},
title={Identification of Parameterized Gray-Box State-Space Systems: From a Black-Box Linear Time-Invariant Representation to a Structured One},
year={2014},
volume={59},
number={11},
pages={2873-2885},
ISSN={0018-9286},
month={Nov}
}

@inproceedings{321Vizer,
  title={A local approach framework for black-box and gray-box {LPV} system identification},
  author={Vizer, D. and Merc{\`e}re, G. and Prot, O. and Ramos, J.},
  booktitle={2013 European Control Conference (ECC)},
  pages={1916--1921},
  year={2013},
  organization={IEEE}
}

@inproceedings{322Vizer,
author={D. {Vizer} and G. {Merc{\`e}re}},
booktitle={2014 European Control Conference (ECC)},
title={$\mathcal{H}_{\infty}$-based {LPV} model identification from local experiments with a gap metric-based operating point selection},
year={2014}
}


@incollection{323Vizer,
  TITLE = {{Linear fractional LPV model identification from local experiments using an $\mathcal{H}_\infty$-based glocal approach}},
  AUTHOR = {Vizer, D. and Merc{\`e}re, G. and Laroche, E. and Prot, O.},
  BOOKTITLE = {{Control-oriented modelling and identification : theory and practice}},
  EDITOR = {M. Lovera},
  PUBLISHER = {{The Institution of Engineering and Technology}},
  PAGES = {189-213},
  YEAR = {2015},
  DOI = {10.1049/PBCE080E\_ch9 },
  HAL_ID = {hal-01313923},
  HAL_VERSION = {v1},
}

@article{325Lu,
title = "{6D} direct-drive technology for planar motion stages",
journal = "CIRP Annals",
volume = "61",
number = "1",
pages = "359 - 362",
year = "2012",
issn = "0007-8506",
doi = "https://doi.org/10.1016/j.cirp.2012.03.145",
author = "Xiaodong, L. and Usman, I. ",
keywords = "Actuator, Mechatronic, Magnetic bearing",
abstract = "Achieving 6D direct drive motion control over long planar strokes on a single mover can greatly improve machine performance. Existing solutions are either limited to small-stroke applications (a fraction of the stage size) or require a large number of coils with enormous control complexity. This paper presents a novel 6D direct drive technology for planar stages with many advantages: (1) stroke can be on the order of several meters; (2) the number of coils increases linearly with motion range; (3) no end effects or force coupling between axes; and (4) ease of control and superior force linearity."
}

@article{326Caigny,
  title={Interpolated modeling of {LPV} systems based on observability and controllability},
  author={Caigny, J and Pintelon, Rik and Camino, Juan F and Swevers, Jan},
  journal={IFAC Proceedings Volumes},
  volume={45},
  number={16},
  pages={1773--1778},
  year={2012},
  publisher={Elsevier}
}

@article{327Caigny,
  title={Interpolated modeling of {LPV} systems},
  author={de Caigny, J. and Pintelon, R. and Camino, J. F. and Swevers, J.},
  journal={IEEE Transactions on Control Systems Technology},
  volume={22},
  number={6},
  pages={2232--2246},
  year={2014},
  publisher={IEEE}
}

@article{328Schmidt,
  title={Distilling free-form natural laws from experimental data},
  author={Schmidt, M. and Lipson, H.},
  journal={science},
  volume={324},
  number={5923},
  pages={81--85},
  year={2009},
  publisher={American Association for the Advancement of Science}
}
@InProceedings{329Duvenaud,
  title = 	 {Structure Discovery in Nonparametric Regression through Compositional Kernel Search},
  author = 	 {Duvenaud, D. and Lloyd, J.R. and Grosse, R. and Tenenbaum, J. and Ghahramani, Z.},
  booktitle = 	 {Proceedings of the 30th International Conference on Machine Learning},
  pages = 	 {1166--1174},
  year = 	 {2013},
  volume = 	 {28},
  number =       {3},
  series = 	 {Proceedings of Machine Learning Research},
  address = 	 {Atlanta, Georgia, USA},
  month = 	 {17--19 Jun},
  publisher = 	 {PMLR}
}

@article{330Prot,
title = "Initialization of Gradient-based Optimization Algorithms for the Identification of Structured State-Space Models",
journal = "IFAC Proceedings Volumes",
volume = "44",
number = "1",
pages = "10782 - 10787",
year = "2011",
note = "18th IFAC World Congress",
issn = "1474-6670",
doi = "https://doi.org/10.3182/20110828-6-IT-1002.02879",
author = "Prot, O. and Merc{\`e}re, G.",
keywords = "System identification, Convex optimization, Iterative methods, Parameterization"
}


@inproceedings{331Petersson,
  author={Petersson, D. and L{\"o}fberg, J.},
  title={Optimization based {LPV}-approximation of multi-model systems},
  booktitle={2009 European Control Conference (ECC)},
  year={2009},
  pages={3172--3177},  
  organization={IEEE}
}

@inproceedings{332Xie,
	author={Xie, L.L. and Ljung, L.},
  	title={Estimate physical parameters by black box modeling},
  	booktitle={Proceedings of the 21st Chinese Control Conference},
  	year={2002}
}


@article{333Mercere,
author={Merc{\`e}re, G. and Laroche, E. and Prot, O.},
title = "Analytical Modelling and Grey-box Identification of a Flexible Arm using a Linear Parameter-varying Model",
journal = "IFAC Proceedings Volumes",
volume = "45",
number = "16",
pages = "1251 - 1256",
year = "2012",
note = "16th IFAC Symposium on System Identification",
issn = "1474-6670"
}

@inproceedings{334Paijmans,
author={B. {Paijmans} and W. {Symens} and H. {van Brussel} and J. {Swevers}},
title={A gain-scheduling-control technique for mechatronic systems with position-dependent dynamics},
booktitle={2006 American Control Conference},
year={2006}
}

@ARTICLE{335Callafon,
author={R. A. {de Callafon} and P. M. J. {van den Hof}},
journal={IEEE Transactions on Control Systems Technology},
title={Multivariable feedback relevant system identification of a wafer stepper system},
year={2001},
volume={9},
number={2},
pages={381-390},
ISSN={1063-6536},
month={March},}

@article{336Maas,
  title={Accurate FRF identification of LPV systems: nD-LPM with application to a medical X-ray system},
  author={van der Maas, R. and van der Maas, A. and Voorhoeve, R. and Oomen, T.},
  journal={IEEE Transactions on Control Systems Technology},
  volume={25},
  number={5},
  pages={1724--1735},
  year={2016},
  publisher={IEEE}
}

@article{337Voorhoeve,
  title={Non-parametric identification of multivariable systems: A local rational modeling approach with application to a vibration isolation benchmark},
  author={Voorhoeve, R. and van der Maas, A. and Oomen, T.},
  journal={Mechanical Systems and Signal Processing},
  volume={105},
  pages={129--152},
  year={2018},
  publisher={Elsevier}
}



@ARTICLE{340Dobrowiecki,
author={T. P. {Dobrowiecki} and J. {Schoukens} and P. {Guillaume}},
journal={IEEE Transactions on Instrumentation and Measurement},
title={Optimized Excitation Signals for {MIMO} Frequency Response Function Measurements},
year={2006},
volume={55},
number={6},
pages={2072-2079},
doi={10.1109/TIM.2006.887036},
ISSN={0018-9456},
month={Dec},}

@article{344Boeij,
  title={Contactless planar actuator with manipulator: A motion system without cables and physical contact between the mover and the fixed world},
  author={de Boeij, J. and Lomonova, E. and Duarte, J.},
  journal={IEEE Transactions on Industry Applications},
  volume={45},
  number={6},
  pages={1930--1938},
  year={2009},
  publisher={IEEE}
}


@ARTICLE{345Balakrishnan, 
author={V. {Balakrishnan} and L. {Vandenberghe}}, 
journal={IEEE Transactions on Automatic Control}, 
title={Semidefinite programming duality and linear time-invariant systems}, 
year={2003}, 
volume={48}, 
number={1}, 
pages={30-41}, 
keywords={eigenvalues and eigenfunctions;linear matrix inequalities;time-varying systems;linear systems;convex programming;semidefinite programming duality;linear time-invariant systems;linear matrix inequality constraints;convex optimization duality;dual optimization problems;system theoretic terms;Linear programming;Linear matrix inequalities;Application software;Control theory;Control systems;Control system synthesis;Riccati equations;Qualifications;Controllability;Constraint theory}, 
doi={10.1109/TAC.2002.806652}, 
ISSN={0018-9286}, 
month={Jan},}


@article{348Caughey,
  title={Classical normal modes in damped linear dynamic systems},
  author={O'Kelly, M. E. J. and Caughey, T. K.},
  journal={Journal of Applied Mechanics},
  volume={32},
  number={3},
  pages={583--588},
  year={1965}
}

@article{349Li,
  title={Thermal-error modeling for complex physical systems: the-state-of-arts review},
  author={Li, J.W. and Zhang, W.J. and Yang, G.S. and Tu, S.D. and Chen, X.B.},
  journal={The International Journal of Advanced Manufacturing Technology},
  volume={42},
  number={1-2},
  pages={168},
  year={2009},
  publisher={Springer}
}



@inproceedings{350Boerlage,
  title={Jerk derivative feedforward control for motion systems},
  author={Boerlage, M. and Tousain, R. and Steinbuch, M.},
  booktitle={Proceedings of the 2004 American Control Conference},
  volume={5},
  pages={4843--4848},
  year={2004},
  organization={IEEE}
}

@inproceedings{351Zou,
  title={Preview-based stable-inversion for output tracking},
  author={Zou, Q. and Devasia, S.},
  booktitle={Proceedings of the 1999 American Control Conference (Cat. No. 99CH36251)},
  volume={5},
  pages={3544--3548},
  year={1999},
  organization={IEEE}
}

@ARTICLE{352Devasia, 
author={S. {Devasia} and B. {Paden}}, 
journal={IEEE Transactions on Automatic Control}, 
title={Stable inversion for nonlinear nonminimum-phase time-varying systems}, 
year={1998}, 
volume={43}, 
number={2}, 
pages={283-288},
ISSN={0018-9286}, 
month={Feb}
}

@inproceedings{353Bloemers,
  title={Parameter-dependent feedforward strategies for motion systems},
  author={Bloemers, T.A.H. and Proimadis, I. and Kasemsinsup, Y. and T{\'o}th, R.},
  booktitle={2018 Annual American Control Conference (ACC)},
  pages={2017--2022},
  year={2018},
  organization={IEEE}
}



@article{354Bristow,
  title={A survey of iterative learning control},
  author={Bristow, D. A. and Tharayil, M. and Alleyne, A. G.},
  journal={IEEE control systems magazine},
  volume={26},
  number={3},
  pages={96--114},
  year={2006},
  publisher={IEEE}
}

@inproceedings{355Stearns,
  title={A comparative study of feedforward tuning methods for wafer scanning systems},
  author={Stearns, H. and Yu, S. and Fine, B. and Mishra, S. and Tomizuka, M.},
  booktitle={ASME 2008 Dynamic Systems and Control Conference},
  pages={669--676},
  year={2008},
  organization={American Society of Mechanical Engineers}
}

@inproceedings{356Theis,
  title={Linear parameter-varying feedforward control: A missile autopilot design},
  author={Theis, J. and Pfifer, H. and Knoblach, A. and Saupe, F. and Werner, H.},
  booktitle={AIAA Guidance, Navigation, and Control Conference},
  pages={2001},
  year={2015}
}

@article{357Mayne,
author={D. Q. {Mayne}},
journal={Proceedings of the Institution of Electrical Engineers},
title={Sequential design of linear multivariable systems},
year={1979},
volume={126},
number={6},
pages={568-572},
doi={10.1049/piee.1979.0135},
ISSN={0020-3270},
month={June}
}

@article{358Custers,
author = {C.H.H.M. Custers and J.W. Jansen and M.C. van Beurden and E.A. Lomonova},
title = {3{D} harmonic modeling of eddy currents in segmented conducting structures},
journal = {COMPEL - The international journal for computation and mathematics in electrical and electronic engineering},
volume = {38},
number = {1},
pages = {2-23},
year = {2019},
doi = {10.1108/COMPEL-02-2018-0070}
}

@INPROCEEDINGS{359Custers, 
author={C. H. H. M. {Custers} and J. W. {Jansen} and E. A. {Lomonova}}, 
booktitle={2017 IEEE International Electric Machines and Drives Conference (IEMDC)}, 
title={Static decoupling of force and torque components in a moving-magnet planar motor}, 
year={2017}, 
volume={}, 
number={}, 
pages={1-8}, 
doi={10.1109/IEMDC.2017.8002065}, 
ISSN={}, 
month={May}
}




@article{365Freeth,
  title={Decoding the ancient Greek astronomical calculator known as the Antikythera Mechanism},
  author={Freeth, T. and Bitsakis, Y. and Moussas, X. and Seiradakis, J. H. and Tselikas, A. and Mangou, H. and Zafeiropoulou, M. and Hadland, R. and Bate, D. and Ramsey, A. and others},
  journal={Nature},
  volume={444},
  number={7119},
  pages={587},
  year={2006},
  publisher={Nature Publishing Group}
}

@book{366Hobsbawm,
  title={Age of revolution: 1789-1848},
  author={Hobsbawm, E.},
  year={2010},
  publisher={Hachette UK}
}

@ARTICLE{367Kang, 
author={C. {Kang}}, 
journal={IEEE Control Systems Magazine}, 
title={{Origin of Stability Analysis: ``On Governors'' by J.C. Maxwell [Historical Perspectives]}}, 
year={2016}, 
volume={36}, 
number={5}, 
pages={77-88}, 
keywords={History;Stability criteria;Differential equations;Water clocks;Brakes}, 
doi={10.1109/MCS.2016.2584358}, 
ISSN={1066-033X}, 
month={Oct},}

@article{368Mayr,
  title={The origins of feedback control},
  author={Mayr, O.},
  journal={Scientific American},
  volume={223},
  number={4},
  pages={110--119},
  year={1970},
  publisher={JSTOR}
}

@misc{369Sawyer,
  title={Magnetic positioning device},
  author={Sawyer, B. A.},
  year={1968},
  month=apr # "~2",
  publisher={Google Patents},
  note={US Patent 3,376,578}
}

@ARTICLE{370Cho, 
author={ Cho, H.S. and Im, C. H. and Jung, H. K.}, 
journal={IEEE Transactions on Magnetics}, 
title={Magnetic field analysis of 2-D permanent magnet array for planar motor}, 
year={2001}, 
volume={37}, 
number={5}, 
pages={3762-3766}, 
keywords={magnetic fields;permanent magnet motors;magnetic flux;synchronous motors;magnetic field analysis;2D permanent magnet array;planar motor;flux density distribution;scalar magnetic potential equation;Magnetic fields;Magnetic analysis;Planar motors;Magnetic flux;Synchronous motors;Permanent magnet motors;Stators;Equations;Coils;Laboratories}, 
doi={10.1109/20.952708}, 
ISSN={0018-9464}, 
month={Sep.},}

@article{371Kim,
title = "High-precision magnetic levitation stage for photolithography",
journal = "Precision Engineering",
volume = "22",
number = "2",
pages = "66 - 77",
year = "1998",
issn = "0141-6359",
doi = "https://doi.org/10.1016/S0141-6359(98)00009-9",
author = "Kim, W.  and Trumper, D.L. ",
keywords = "precision motion control, photolithography, magnetic levitation, mechatronics",
abstract = "In this paper, we present a high-precision magnetic levitation (maglev) stage for photolithography in semiconductor manufacturing. This stage is the world’s first maglev stage that provides fine six-degree-of-freedom motion controls and realizes large (50 mm × 50 mm) planar motions with only a single magnetically levitated moving part. The key element of this stage is a linear motor capable of providing forces in both suspension and translation without contact. The advantage of such a stage is that the mechanical design is far simpler than competing conventional approaches and, thus, promises faster dynamic response and higher mechanical reliability. The stage operates with a positioning noise as low as 5 nm rms in x and y, and acceleration capabilities in excess of 1 g (10 m/s2). We demonstrate the utility of this stage for next-generation photolithography or in other high-precision motion control applications."
}

@INPROCEEDINGS{372Boerj, 
	author={J. {de Boeij} and E. {Lomonova} and J. {Duarte}},
		title={Contactless Planar Actuator with Manipulator: a Motion System without Cables and Physical Contact between the Mover and the Fixed World}, 
		 booktitle={2008 IEEE Industry Applications Society Annual Meeting}, 
	year={2008}
} 

@phdthesis{373Roover,
  title={Motion control of a wafer stage},
  author={de Roover, D.},
  school={Delft University of Technology},
  year={1997}
}

@article{374Ronde,
  title={Data-based spatial feedforward for over-actuated motion systems},
  author={Ronde, M.J.C. and Leenknegt, G.A.L. and van de Molengraft, M.J.G. and Steinbuch, M.},
  journal={Mechatronics},
  volume={24},
  number={6},
  pages={679--690},
  year={2014},
  publisher={Elsevier}
}

@article{375Halbach,
title = "Design of permanent multipole magnets with oriented rare earth cobalt material",
journal = "Nuclear Instruments and Methods",
volume = "169",
number = "1",
pages = "1 - 10",
year = "1980",
issn = "0029-554X",
doi = "https://doi.org/10.1016/0029-554X(80)90094-4",
author = "K. Halbach"
}

@article{376Ronde,
title = "Model-based spatial feedforward for over-actuated motion systems",
journal = "Mechatronics",
volume = "24",
number = "4",
pages = "307 - 317",
year = "2014",
note = "Vibration control systems",
issn = "0957-4158",
doi = "https://doi.org/10.1016/j.mechatronics.2013.09.010",
author = "M.J.C. Ronde and M.G.E. Schneiders and E.J.G.J. Kikken and M.J.G. van de Molengraft and M. Steinbuch",
}


@inproceedings{377Baggen,
author={M. {Baggen} and M. {Heertjes} and R. {Kamidi}},
title={Data-based feed-forward control in {MIMO} motion systems},
booktitle={2008 American Control Conference},
year={2008},
pages={3011-3016}
}

@book{378Kocijan,
  title={Modelling and control of dynamic systems using {Gaussian} process models},
  author={Kocijan, J.}},
  year={2016},
  publisher={Springer}
}

@article{380Tibshirani,
  title={Regression shrinkage and selection via the lasso},
  author={Tibshirani, R.},
  journal={Journal of the Royal Statistical Society: Series B (Methodological)},
  volume={58},
  number={1},
  pages={267--288},
  year={1996},
  publisher={Wiley Online Library}
}

@article{381Recht,
  title={Guaranteed minimum-rank solutions of linear matrix equations via nuclear norm minimization},
  author={Recht, B. and Fazel, M. and Parrilo, P. A.},
  journal={SIAM review},
  volume={52},
  number={3},
  pages={471--501},
  year={2010},
  publisher={SIAM}
}

@article{382Kimeldorf,
  title={Some results on Tchebycheffian spline functions},
  author={Kimeldorf, G. and Wahba, G.},
  journal={Journal of mathematical analysis and applications},
  volume={33},
  number={1},
  pages={82--95},
  year={1971},
  publisher={Elsevier}
}

@ARTICLE{383Aravkin, 
author={A. Y. {Aravkin} and B. M. {Bell} and J. V. {Burke} and G. {Pillonetto}}, 
journal={IEEE Transactions on Neural Networks and Learning Systems}, 
title={{The Connection Between Bayesian Estimation of a Gaussian Random Field and RKHS}}, 
year={2015}, 
volume={26}, 
number={7}, 
pages={1518-1524}, 
doi={10.1109/TNNLS.2014.2337939}, 
ISSN={2162-237X}, 
month={July},}


@article{384Mackay,
  title={{Introduction to Gaussian processes}},
  author={MacKay, D. J. C.},
  journal={NATO ASI Series F Computer and Systems Sciences},
  volume={168},
  pages={133--166},
  year={1998},
  publisher={Springer Verlag}
}


@article{385Tresp,
  title={{A Bayesian committee machine}},
  author={Tresp, V.},
  journal={Neural computation},
  volume={12},
  number={11},
  pages={2719--2741},
  year={2000},
  publisher={MIT Press}
}

@INBOOK{386Bottu,
author={L. {Bottou} and O. {Chapelle} and D. {DeCoste} and J. {Weston}},
title={Large-Scale Kernel Machines},
year={2007},
volume={},
number={},
pages={},
keywords={},
doi={},
ISSN={},
publisher={MIT Press},
isbn={9780262255790}
}

@article{387Quinonero,
  title={Approximation methods for Gaussian process regression},
  author={Quinonero-Candela, J. and Rasmussen, C. E. and Williams, C. K. I.},
  journal={Large-scale kernel machines},
  pages={203--224},
  year={2007},
  publisher={MIT Press}
}

@article{389Edwards,
author = {Edwards, C. and Postlethwaite, I.},
title = "Anti-windup and bumpless-transfer schemes",
journal = "Automatica",
volume = "34",
number = "2",
pages = "199 - 210",
year = "1998",
issn = "0005-1098",
doi = "https://doi.org/10.1016/S0005-1098(97)00165-9"
}


@article{390Peng,
author = {Peng, Y. and Vran\v{v}i\'{c}, D. and Hanus, R.},
year = {1996},
month = {09},
pages = {48 - 57},
title = {Antiwindup, Bumpless, and Conditioned Transfer Techniques for PID Controllers},
volume = {16},
journal = {Control Systems, IEEE},
doi = {10.1109/37.526915}
}

@article{391Kowalski,
title = "Implementation of a linear quadratic bumpless transfer method to a magnetically levitated planar actuator with moving magnets",
author = "K.K. Kowalski and J. Achterberg and {Lierop, van}, C.M.M. and {Bosch, van den}, P.P.J.",
year = "2010",
booktitle = "Proceedings of the 2010 IEEE International Conference on Control Applications (CCA 2010), part of the 2010 IEEE Multi-Conference on Systems and Control (MSC 2010), 8-10 September 2010, Yokohama, Japan"
}

@article{392Turner,
title = "Linear quadratic bumpless transfer",
journal = "Automatica",
volume = "36",
number = "8",
pages = "1089 - 1101",
year = "2000",
issn = "0005-1098",
doi = "https://doi.org/10.1016/S0005-1098(00)00021-2",
author = "Turner, M. C. and Walker, D. J.",
}

@article{393Amidror,
  title={Scattered data interpolation methods for electronic imaging systems: a survey},
  author={Amidror, I.},
  journal={Journal of electronic imaging},
  volume={11},
  pages={157--76},
  year={2002}
}


@article{394Englehart,
title = "A four-block problem for $H_{\infty}$ design: Properties and applications",
 author={Englehart, M. J. and Smith, M. C.},
journal = "Automatica",
volume = "27",
number = "5",
pages = "811 - 818",
year = "1991",
issn = "0005-1098",
doi = "https://doi.org/10.1016/0005-1098(91)90035-Z"
}

@mastersthesis{395Bloemers,
title={Nanometer accurate motion control of a magnetically levitated planar actuator},
author={
Bloemers, T.A.H.},
year={2018},
school={Eindhoven University of Technology, Department of Electrical Engineering, Control Systems Group}
}

@inproceedings{396Wortelboer, 
author={P. M. R. {Wortelboer} and O. H. {Bosgra}}, 
title={Frequency weighted closed-loop order reduction in the control design configuration}, 
booktitle={Proceedings of 1994 33rd IEEE Conference on Decision and Control}, 
year={1994}, 
}

@article{397Grosdidier,
title = "Interaction measures for systems under decentralized control",
journal = "Automatica",
volume = "22",
number = "3",
pages = "309 - 319",
year = "1986",
issn = "0005-1098",
doi = "https://doi.org/10.1016/0005-1098(86)90029-4",
author = "Grosdidier, P. and Morari, M."
}

@article{398Heertjes,
title = "Minimizing cross-talk in high-precision motion systems using data-based dynamic decoupling",
journal = "Control Engineering Practice",
volume = "19",
number = "12",
pages = "1423 - 1432",
year = "2011",
issn = "0967-0661",
doi = "https://doi.org/10.1016/j.conengprac.2011.07.016",
author = "Heertjes, M. and van Engelen, A.",
keywords = "Dynamic decoupling, Iterative schemes, Autotuning, Disturbance rejection, Industrial applications of optimal control"
}

@inproceedings{399Vaes,
author={D. {Vaes} and J. {Swevers} and P. {Sas}},
booktitle={Proceedings of the 2004 American Control Conference},
title={Optimal decoupling for {MIMO}-controller design with robust performance},
year={2004}
}

@ARTICLE{400Paattilammi,
author={J. {Paattilammi} and P. M. {Makila}},
journal={IEEE Control Systems Magazine},
title={Fragility and robustness: a case study on paper machine headbox control},
year={2000},
volume={20},
number={1},
pages={13-22},
doi={10.1109/37.823222},
ISSN={},
month={Feb}
}


@inproceedings{401Ravi,
author={R. {Ravi} and J. {Chen} and C. N. {Nett}},
booktitle={Proceedings of the 31st IEEE Conference on Decision and Control},
title={Computing nominal models for uncertain plants},
year={1992}
}

@article{402Devasia,
  title={Should model-based inverse inputs be used as feedforward under plant uncertainty?},
  author={Devasia, Santosh},
  journal={IEEE Transactions on Automatic Control},
  volume={47},
  number={11},
  pages={1865--1871},
  year={2002},
  publisher={IEEE}
}

@article{403Gelder,
  title={Nominal and robust feedforward design with time domain constraints applied to a wafer stage},
  author={de Gelder, E. and van de Wal, M. and Scherer, C. and Hol, C. and Bosgra, O.},
  journal={Journal of dynamic systems, measurement, and control},
  volume={128},
  number={2},
  pages={204--215},
  year={2006},
  publisher={American Society of Mechanical Engineers}
}

@article{404Rozario,
author={R. {de Rozario} and T. {Oomen} and M. {Steinbuch}},
booktitle={2017 American Control Conference (ACC)},
title={Iterative Learning Control and feedforward for LPV systems: Applied to a position-dependent motion system},
year={2017},
volume={},
number={},
pages={3518-3523},
month={May},}

@article{405Pintelon,
  title={Estimation of nonparametric noise and FRF models for multivariable systems—Part I: Theory},
  author={Pintelon, Rik and Schoukens, Johan and Vandersteen, Gerd and Barb{\'e}, Kurt},
  journal={Mechanical Systems and Signal Processing},
  volume={24},
  number={3},
  pages={573--595},
  year={2010},
  publisher={Elsevier}
}
@article{406Wollnack,
title = "Fixed-structure {LPV-IO} controllers: An implicit representation based approach",
journal = "Automatica",
volume = "83",
pages = "282 - 289",
year = "2017",
issn = "0005-1098",
doi = "https://doi.org/10.1016/j.automatica.2017.06.009",
author = "S. Wollnack and H.S. Abbas and R. T{\'o}th and H. Werner",
keywords = "Linear parameter-varying, Fixed-structure, Input–output"
}


@inproceedings{407Wollnack,
author={S. {Wollnack} and H. {Werner}},
booktitle={2016 American Control Conference (ACC)},
title={{LPV-IO controller design: An LMI approach}},
year={2016}
}


@article{409Schaller,
  title={Moore's law: past, present and future},
  author={Schaller, R.},
  journal={IEEE spectrum},
  volume={34},
  number={6},
  pages={52--59},
  year={1997},
  publisher={IEEE}
}

@article{410Kontaras,
title = "Continuous compliance compensation of position-dependent flexible structures",
journal = "IFAC-PapersOnLine",
volume = "49",
number = "13",
pages = "76 - 81",
year = "2016",
note = "12th IFAC Workshop on Adaptation and Learning in Control and Signal Processing ALCOSP 2016",
issn = "2405-8963",
author = "Kontaras, N. and Heertjes, M. and Zwart, H."
}

@article{411Wal,
  title={A review of methods for input/output selection},
  author={van de Wal, M. and de Jager, B.},
  journal={Automatica},
  volume={37},
  number={4},
  pages={487--510},
  year={2001},
  publisher={Elsevier}
}

@article{412Csato,
  title={Sparse on-line Gaussian processes},
  author={Csat{\'o}, L. and Opper, M.},
  journal={Neural computation},
  volume={14},
  number={3},
  pages={641--668},
  year={2002},
  publisher={MIT Press}
}

@inproceedings{413Arehart,
author={A. B. {Arehart} and W. A. {Wolovich}},
booktitle={Proceedings of 35th IEEE Conference on Decision and Control},
title={Bumpless switching controllers},
year={1996}
}

@article{414Pillonetto,
author={G. {Pillonetto} and A. {Chiuso}},
booktitle={2014 European Control Conference (ECC)},
title={Tuning complexity in kernel-based linear system identification: The robustness of the marginal likelihood estimator},
year={2014},
volume={},
number={},
pages={2386-2391},
doi={10.1109/ECC.2014.6862629},
ISSN={null},
month={June}
}

@inproceedings{415Rasmussen,
  author={Rasmussen, C. E. and Ghahramani, Z.},
  title={Occam's razor},
  booktitle={Advances in neural information processing systems},
  year={2001},
  pages={294--300}
}

@article{416Maxwell,
  title={{I. On governors}},
  author={Maxwell, James Clerk},
  journal={Proceedings of the Royal Society of London},
  number={16},
  pages={270--283},
  year={1868},
  publisher={The Royal Society London},
  address = {}
}

@article{417Schmidt,
  title={Ultra-precision engineering in lithographic exposure equipment for the semiconductor industry},
  author={Schmidt, Robert-H Munnig},
  journal={Philosophical Transactions of the Royal Society A: Mathematical, Physical and Engineering Sciences},
  volume={370},
  number={1973},
  pages={3950--3972},
  year={2012},
  publisher={The Royal Society Publishing}
}

@inproceedings{418Custers,
  title={Active Compensation of the Deformation of a Magnetically Levitated Mover of a Planar Motor},
  author={Custers, CHHM and Proimadis, Ioannis and Jansen, JW and Butler, Hans and Toth, Roland and Lomonova, EA and van den Hof, PMJ},
  booktitle={2019 IEEE International Electric Machines \& Drives Conference (IEMDC)},
  pages={854--861},
  year={2019},
  organization={IEEE}
}

@article{419Lierop,
  title={Commutation of a magnetically levitated planar actuator with moving-magnets},
  author={Jansen, J.W. and Lomonova, E.A. and Damen, A.A.H. and van den Bosch, P.P.J. and Vandenput, A.J.A.},
  journal={IEEJ Transactions on Industry Applications},
  volume={128},
  number={12},
  pages={1333--1338},
  year={2008},
  publisher={The Institute of Electrical Engineers of Japan}
}

